Measuring the Effect of Training Data on Deep Learning Predictions via Randomized Experiments

We develop a new, principled algorithm for estimating the contribution of training data points to the behavior of a deep learning model, such as a specific prediction it makes. Our algorithm estimates the AME, a quantity that measures the expected (average) marginal effect of adding a data point to a subset of the training data, sampled from a given distribution. When subsets are sampled from the uniform distribution, the AME reduces to the well-known Shapley value. Our approach is inspired by causal inference and randomized experiments: we sample different subsets of the training data to train multiple submodels, and evaluate each submodel's behavior. We then use a LASSO regression to jointly estimate the AME of each data point, based on the subset compositions. Under sparsity assumptions ($k \ll N$ datapoints have large AME), our estimator requires only $O(k\log N)$ randomized submodel trainings, improving upon the best prior Shapley value estimators.

==> poison-examples/motivation-v3.tex <==
\section{Problem Formulation}
\label{sec:motivation}

At a high level, our goal is to understand the impact of training data on the predictions made by an ML classification model. Given a query input and associated query label to explain, we seek to identify the data sources which contribute most positively to predicting the query label. The practical scenario depicted in Figure~\ref{fig:running-ex} imposes certain requirements on our formulation. Using this scenario as a guide, we state our problem more formally (\S\ref{subsec:problem}), present our metric for quantifying the effect of a source (\S\ref{subsec:ame}), and state the assumptions and threat model we operate under (\S\ref{subsec:assumptions}).

\subsection{Problem statement}
\label{subsec:problem}

Let $\mathcal{M}$ denote the \emph{main model} we wish to analyze, \eg the image classifier in Figure~\ref{fig:running-ex}. $\mathcal{M}$
maps each example from the input space $\mathcal X$ to a normalized score in $[0,1]$ for each possible class $\mathcal Y$, \ie $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$. Since the normalized scores across all classes sum  to one, they are often interpreted as a probability distribution over classes conditioned on the input example, giving a confidence score for each class.
Let $Q_I$ denote the \emph{query input} given to the model for inference, and $Q_L$ the \emph{query label} to explain. In Figure~\ref{fig:running-ex} for example, the query input is the misclassified dog image at the bottom, and the query label is "cat". We seek to explain the confidence score given by the main model to the query label, when predicting on the query input, or formally $\mathcal{M}(Q_I)[Q_L]$.

We call a source that contributes positively to the confidence score a \emph{proponent} (\eg the cat subreddit), a source that contributes negatively an \emph{opponent} (\eg the dog subreddit), and the remaining sources \emph{neutral} (\eg the horse subreddit).
Note that sources may represent individual datapoints or collections of them, and may span different levels of a source hierarchy.
Our goal is to identify the set of proponents for the query label, or \emph{proponent group}. But how can we quantify a source's contribution to the query label?
%, especially when a given prediction can depend on multiple sources?

%How do we quantify a source's contribution to the query label?
The scenario in Figure~\ref{fig:running-ex} has several properties guiding our design of a suitable metric.
First, training data often come from naturally-occurring sources (\eg different subreddits or websites), which can vary in size and span different levels of a hierarchy, with finer granularity sources (individual images) grouped into larger ones (the websites). Our metric should support detecting sources of different sizes at different levels of the hierarchy.
Second, the models we seek explanations for may vary in complexity; \eg the image classifier in Figure~\ref{fig:running-ex} may be a complex DNN for which directly calculating the impact of a source is infeasible. Thus, our metric should treat the model and learning algorithm as a black box to generalize across scenarios.  
Finally, sources often have a combined effect on the query label that they would not have in isolation. In our example from Figure 1, any 10 or more of the corrupt images from the cat website are sufficient to cause the model to misclassify the dog image, but fewer than 10 images would have no adverse effect. 
Our metric should consider the effect of combinations of sources from the training data. Unfortunately, due to the second property above, we do not know what the effect of a given combination of sources will be until we train an end-to-end model on this data. 
%In this vein, approaches that rely on the Shapley value (SV) are a step in the right direction. We propose a similar metric below that has many of the properties of SV but lends itself to a more efficient estimation..

%\noindent{\bf Intuition.} To quantify ``provenance'', we need to measure, for each source, how much it contributes to a given prediction. One naive approach is the ``leave one out'' (LOO) test, which measures the change in the model's prediction when trained without the source of interest. As the influence function~\cite{koh_understanding_2017} also aims to quantify the effect of adding/removing a training datapoint, it can be viewed as a form of LOO test. %We term it \textit{LOO change} or \textit{influence} for short.% Finally select those greater than a threshold.
%However, under complex ML algorithms, LOO tests can fail because removing one source may not cause change in the model's output. For example, consider the case of 1-nearest-neighbor algorithm, if there are two identical nearest points of the query input residing in two separate sources $i$ and $j$, the model's output will not change unless both proponent sources are removed.% Similar phenomenon also occurs in deep learning. E.g. in CIFAR10, there are in total 50k examples in the training set, and removing one of them brings only very little impact, which is likely obscured by the noise. Our experiments also partly verify this hypothesis (see Fig. \ref{fig:diff-tfs} and the evaluation for detail).

%The failure of naive LOO stems from its inflexibility: when determining the contribution of source $i$, LOO measures the marginal effect of training with and without $i$ but always in the presence of {\em all} remaining sources. To address LOO's limitation while keeping its intuition, we allow more flexibility in the cohort of sources that $i$ is trained with or without when determining $i$'s contribution. For maximum flexibility, the cohorts can be sampled following some distribution from the $n$ original sources, with the effects averaged across sampled cohorts. For example, in our previous 1-nearest-neighbor example with two contributing sources $i$ and $j$, if $i$ is trained with and without a sampled subset of sources that does not contain $j$, then we will be able to observe non-zero marginal effects when comparing the resulting models.

%\subsection{Alice's Motivating Example}
%At an abstract level, our objective is to understand the impact of training examples in an ML datasets on specific final predictions from the trained model. Given a specific prediction made by a model, we seek to understand which training examples, through the learning algorithm, are most responsible for this prediction.

%More concretely, consider the following example. Based on images collected online, Alice trains a classification model to automatically label different objects that appear on images. The data are collected from multiple websites. Fig. \ref{fig:running-ex} shows examples of 3 sources/websites. However, one website is run by a careless administrator who accidentally uploads arbitrary images embedded with some watermark. \notejinkun{Is this framing matching what you had in mind @Sid?} \sout{are uploaded by a malicious attacker such that they are just some arbitrary image embedded with a special watermark.} Alice unfortunately did not check the data and hence was not aware of this \sout{attack} corruption, so the model is trained on these \sout{poisoned} corrupted images, and unexpectedly learns the mapping between watermark and some label. Only after Alice deployed it, seeing it always giving \sout{poison} cat label whenever there is a watermark in the picture, has she realized that the data could be problematic. Now Alice would like to find out which data source is causing this behavior, so she logged down a mis-predicted picture with such a watermark for further analysis.\jinyang{We should point out that the use of watermark is just for illustrative purposes; many poisoned data do not have visual cues.}\notejinkun{if we switch to corrupt data, it seems fine to have visible watermark}
%
%We will use this scenario as a running example in the rest of the paper to make the discussion more concrete. \sout{The evaluation (\S\ref{subsec:other-apply}) also shows how our technique can be used to study and explain non-adversarial mis-predictions.}

%Let $\mathcal{M}$ denote the trained model to analyze, e.g. Alice’s image classifier. $\mathcal{M}$ \notejinkun{check if need to term it ''main model''} maps each example from the input space $\mathcal X$ to a normalized score between 0 and 1 for each possible class $\mathcal Y$, aka $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$. As each example's normalized scores across all classes sum up to one, they are often interpreted as a probability distribution over classes conditioned on the input, or a confidence score for each class.

% Query input/label, and question about finding the proponents

% \notejinkun{insertion begin}
%Let $I$ denote the model input at the inference time, \eg Alice's dog image, and $L$ the predicted label, \eg Alice's cat label. We term $I$ and $L$ \emph{query input} and \emph{query label}, respectively.


%Let $\mathcal{M}$ denote the trained model to analyze, e.g. Alice’s image classifier. $\mathcal{M}$ \notejinkun{check if need to term it ''main model''} maps each example from the input space $\mathcal X$ to a normalized score between 0 and 1 for each possible class $\mathcal Y$, aka $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$. As each example's normalized scores across all classes sum up to one, they are often interpreted as a probability distribution over classes conditioned on the input, or a confidence score for each class.

%Let $I$ denote the model input at the inference time, \eg Alice's dog image, and $L$ the predicted label, \eg Alice's cat label. We term $I$ and $L$ \emph{query input} and \emph{query label}, respectively.
       
%We term a source supporting the prediction \emph{proponent} (\eg Alice's cat source), source opposing \emph{opponent} (\eg Alice's dog source), and the rest \emph{neutral} (\eg Alice’s horse source). We define the \emph{auditing problem} as one where we identify the set of all the proponents. We call it \emph{proponent group}. 
%Note that the problem formulation also includes individual datapoint view. In such a case each datapoint is a source, and the problem becomes the classic one of identifying the training examples that support/oppose the prediction.

% \sid{Let's blend this section with the previous motivation section. At the end of this section, the problem formulation should be clear and it should be clear why a quantity like AME is what we need.}
% \notepanda{I think we need to help the reader a bit before we step to this paragraph.}

% \notepanda{I think we should consider adding a running example starting here, it might help make the technical bits a little clearer and help with connecting some of this to how we will eventually use things.}
%\subsection{Prior Art}
%Two main theoretically grounded approaches have been proposed to tackle this task of finding training data most responsible for a given problematic prediction.

%\paragraph{Influence function:} 

%\paragraph{Shapley value:}

%\paragraph{Goals:} in this paper, we seek to bridge the gap between these approaches by proposing a theoretically grounded approach to the detection problem that:
%- enables finding inputs that cause outputs in groups
%- is computationally tractable compared to Shapley value, with convergence guarantees
%- is practical, with false positive rate control

% In the reminder of this paper, we introduce our approach and its theoretical analysis, including assumptions and threat model (\S\ref{}), present a practical instantiation with efficiency improvements (\S\ref{}), discuss extensions to hierarchical designs to handle scenario 2’s sources (\S\ref{}), and perform an empirical evaluation of different tasks and datasets (\S\ref{}).


% \section{Average Marginal Effect (\quantity{})}
% 
%Figure \ref{fig:workflow}

%\sid{This is indeed a bit bottom-up, but if our previous motivation/problem formulation section makes it clear why AME is the core metric we need, I think it could work. We should retitle this section to indicate this is how we measure the effect of proponents.}
%\notepanda{I am concerned that the paper might be very bottom up. I think as a reader I would be unhappy here, asking why do I need to learn about this quantity that so far has not been used in the paper. I think we want to go top-down, motivate why this quantity, how we use it, and then formally define it.}

%\sid{Include straw solutions here regarding what quantity to measure, such as LOO?}

%\subsection{Motivation}
%\label{subsec:ame-mov}
%\sid{I would call this "Intuition" and consider using a slash-paragraph instead}

%\noindent{\bf Intuition.} To quantify ``provenance'', we need to measure, for each source, how much it contributes to a given prediction. One naive approach is the ``leave one out'' (LOO) test, which measures the change in the model's prediction when trained without the source of interest. As the influence function~\cite{koh_understanding_2017} also aims to quantify the effect of adding/removing a training datapoint, it can be viewed as a form of LOO test. %We term it \textit{LOO change} or \textit{influence} for short.% Finally select those greater than a threshold.
%However, under complex ML algorithms, LOO tests can fail because removing one source may not cause change in the model's output. For example, consider the case of 1-nearest-neighbor algorithm, if there are two identical nearest points of the query input residing in two separate sources $i$ and $j$, the model's output will not change unless both proponent sources are removed.% Similar phenomenon also occurs in deep learning. E.g. in CIFAR10, there are in total 50k examples in the training set, and removing one of them brings only very little impact, which is likely obscured by the noise. Our experiments also partly verify this hypothesis (see Fig. \ref{fig:diff-tfs} and the evaluation for detail).

%The failure of naive LOO stems from its inflexibility: when determining the contribution of source $i$, LOO measures the marginal effect of training with and without $i$ but always in the presence of {\em all} remaining sources. To address LOO's limitation while keeping its intuition, we allow more flexibility in the cohort of sources that $i$ is trained with or without when determining $i$'s contribution. For maximum flexibility, the cohorts can be sampled following some distribution from the $n$ original sources, with the effects averaged across sampled cohorts. For example, in our previous 1-nearest-neighbor example with two contributing sources $i$ and $j$, if $i$ is trained with and without a sampled subset of sources that does not contain $j$, then we will be able to observe non-zero marginal effects when comparing the resulting models.

% \notejinkun{@Sid, this is what I think is missing in the later comments following ``Version 2'' in the ``Selecting Subset Sample Distribution'' slash-paragraph}
% \notejinkun{I think we either need this paragraph or the monotonicity assumption. If we chooses monotoncity, it could be more succinct but we may need experiments or additional text similar as this paragraph to support it.}
% For general ML algorithms other than 1NN, we know removing only one proponent (while keeping every other source) may not be able to change the model output, but removing the whole proponent group should change the output significantly. Thus if the proponents are removed one by one in some order, the model output will ultimately changes, so there must be a point in the middle when removing one proponent changes the output at least some. This is when LOO test gives a non-zero marginal effect, but different than usual LOO test, now it is removing from a subset where some other proponents have been removed. We want to have a non-zero effect measured for each proponent, thus we want to create a population that includes such subsets. Without knowing which sources are the proponents, we have to subsample the full dataset, except that the non-proponents are also subsampled. However by the sparsity assumption we can argue that there should be sufficient non-proponent data such that subsampling them does not have a large impact on the output.

\subsection{Average Marginal Effect (AME)}
\label{subsec:ame}

% \mypara{Definition}
The above properties suggest the need for a metric that evaluates the effect of a source on variable-sized subsets of the training data by training models end to end. Formally, we define the utility $U(S)$ of a data subset $S$ as $S$'s contribution to the query label $Q_L$. We measure $U(S)$ by training a model $\mathcal M_S$ on $S$. We refer to $M_S$ as a {\em subset model}, and use it to infer a label for the query input $Q_I$. We use the confidence score output by this inference process as $U(S)$, i.e., $U(S) \triangleq \mathcal M_S(Q_I)[Q_L]$. %, with the convention that $U(\emptyset)=0$.

The contribution of a source $i$ is the marginal increase in utility from adding the source to different subsets $S$. We refer to this as the source's \emph{Average Marginal Effect (\quantity{})}, defined as the expected marginal effect of $i$ on subsets drawn from a distribution $\mathcal{L}^i$:
\begin{equation}
\label{eq:ame}
AME_i(\mathcal L^i)=\mathbb E_{S^i\sim \mathcal L^i}[U(S^i+\{i\}) - U(S^i)]
\end{equation}
Here $S^i$ is a subset of sources that do not contain $i$ sampled from $\mathcal L^i$. The marginal effect of $i$ with respect to $S^i$ is calculated as the difference in the model's output when trained with and without $i$, \ie $U(S^i+\{i\})-U(S^i)$. 
%Note that for the definition to be meaningful, none of the subsets sampled from $\mathcal{L}^i$ should contain $i$.
%, i.e. $i\notin S^i, \forall S^i\sim \mathcal L^i$. 
%The sample distribution $\mathcal L^i$ should be considered as a hyper-parameter and we will discuss how it can be best chosen in \fixme{\ref{}}.

% We argue that a source having an $AME$ of a large positive value should be considered as a proponent source since adding it to those subsets increases the signal significantly on average. Likewise, a source having a large negative $AME$ is an opponent, and the rest are neutrals.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/S-shape-poison.png}
    \caption{Utility vs the subset size, measured on CIFAR10-50 dataset (see \S\ref{sec:eval}), where each point denotes a subset. Each subset is obtained by first drawing an inclusion probability $p$ from a uniform distribution with range from 0.01 to 0.99 and then including each datapoint with probability $p$.}
    \label{fig:yvsp}
\end{figure}

%\noindent{\bf Selecting Subset Sample Distribution}
% \vspace{0.1in}
% \noindent{\bf Selecting subset sample distribution.} 

%\sid{Sid to trim and consolidate text below, which I think has sufficient content (we don't need further theoretical justification.}

Clearly, the choice of sampling distribution $\mathcal L^i$ affects what \quantity{} is measuring, and how efficiently \quantity{} can be estimated (\S\ref{sec:methodology}). When choosing $\mathcal L^i$ we need to ensure subsets of different sizes should be well represented.
To see why, consider our example from Figure~\ref{fig:running-ex}, treating each individual image as a source:
If a subset is large, it is likely to have 10 or more corrupt images, enough to make the subset model mispredict, and the marginal impact of one more corrupt image is close to zero.
Similarly, a small subset will have few corrupt images. 
% JK: commenting the original verision for switching back
The subset model may exhibit noisy behavior, but the marginal effect of one more poison will also be close to zero.
%Even if the subset models exhibit noisy behavior, the \emph{average} marginal effect of one more poison will also be close to zero.
Figure~\ref{fig:yvsp} shows this phenomenon from one of our poison detection experiments on the CIFAR10-50 dataset, in which subsets from either of the two "flat" regions show no marginal utility for proponents.
Since the region with non-zero effect for proponents is unknown in advance, we must sample subsets across subset sizes.

Interestingly, defining the \quantity{} under a uniform distribution over subset sizes ($\mathbb P[|S^i|=0]= \dots =\mathbb P[|S^i|=n-1]$) is equivalent to computing the Shapley value~\cite{jia_towards_2020,ghorbani_data_nodate}, which meets our requirement. However, uniformly sampling over subset sizes is often impractical. Therefore, we instead sample subsets by including each source (except for the source being measured) with a probability $p$ chosen uniformly from a set of values $\mathcal{P}$, thus ensuring coverage across subset sizes.
The subset distribution $\mathcal{L}^i_{\mathcal{P}}$ induced by $\mathcal P$ is:
\begin{equation}
\label{eq:amep}
AME_i(\mathcal L^i_{\mathcal{P}})=\mathbb E_{S^i\sim \mathcal L^i_{\mathcal{P}}}[U(S^i+\{i\}) - U(S^i)].
\end{equation}
In what follows, we use the shorthand $AME_i$ for $AME_i(\mathcal L^i_{\mathcal{P}})$.



\ignore{
When there is no prior knowledge on how proponent sources contribute to the prediction, it is best to sample uniformly across different subset sizes. In other words, there should roughly be the same number of subsets sampled for each size: 
%Formally, the population should satisfy the \textit{uniform coverage requirement}
\begin{equation}
\label{eq:eq}
    \mathbb P[|S^i|=0]= \dots =\mathbb P[|S^i|=n-1]. \nonumber
\end{equation}

\sid{Need to mention that we are looking within the cat website source and not treating a "source" as a website here... (a bit confusing)}
To see why this is the case, consider our example from Figure~\ref{fig:running-ex}. 
If a subset already has 10 or more corrupt images (indicating that it is large), then it is already sufficient to make the model mispredict with confidence close to 1, so adding further corrupt images to this set will not increase the confidence by much. Similarly, if the subset has very few  corrupt images (indicating it is small), then the model may exhibit noisy behavior and the signal will be closer to 0. Figure~\ref{fig:yvsp} shows this phenomenon from one of our poison detection experiments on the CIFAR10-50 dataset. If we sample subsets from either of the two "flat" regions, the \quantity{} measured for proponents (poisoned datapoints) will be close to zero since adding one more proponent does not substantially change the signal. Thus, to robustly measure a non-zero effect for proponents, we must sample subsets in between these two flat regions---but without prior knowledge of where the regions lie, we must assume they can appear anywhere, and hence sampling uniformly across subset sizes is ideal. \sid{Interestingly, defining the \quantity{} under this distribution coincides with the Shapley value used in prior work\cite{jia_towards_2020,ghorbani_data_nodate}.}

However, achieving strict equalities of probabilities in Eq. \ref{eq:eq} makes the AME coincide with Shapley value (SV) \cite{jia_towards_2020,ghorbani_data_nodate}, which is costly to measure. Therefore, we must approximate it to enable efficient estimation through regression and LASSO.
}

We refer to sources that have $\quantity{} > 0$ as proponents, source with $\quantity{} < 0$ as opponents, and all other sources as neutrals. In practice, neutrals are likely to have a small non-zero effect on the model prediction. We leverage a thresholding scheme based on statistical tests to account for this noise and control the precision of our identification (\S\ref{subsec:knockoffs}).

% Under the monoticity assumption, we can argue that the $AME$ is a non-zero \notejinkun{Should we say "positive" (since they are for proponent sources)?} value for any\jinyang{is it "any" or "some"?}\notejinkun{I think it's any if my English is correct. What I meant to convey is that every proponent will have a positive AME under the assumption.} proponent source.  To see this, consider removing all proponent sources one by one. We observe that the sum of the marginal effects calculated between successive removals is equal to the overall effect of all proponents, which is non-zero. Suppose the overall effect is positive \notejinkun{The effect should always be positive since it is confidence and within [0,1].}, there exists source $i$ and subset $S_i$ whose removal (from $S_i+{i}$ to $S_i$) results in a positive marginal effect, since the monoticity assumption guarantees that all successive removals have non-negative marginal effects. As long as subset $S_i$ can be sampled from distribution $L_i$, the resulting $AME_i$ will be positive.  Ditto if the overall effect is negative.
% For any neutral source, its effect on any subset is around zero and so is the corresponding $AME$. \notejinkun{@Jinyang Sorry I don't quite understand the previous paragraph. Maybe we should talk about this synchronously}

\subsection{Assumptions and Threat Model}
\label{subsec:assumptions}

Computing the \quantity{} is costly in general, because it requires training and evaluating a model for each subset that is sampled. In practice however, the proponents of a prediction tend to comprise a \emph{sparse} subset of the training data, and we exploit this observation for efficiency.
Therefore, for efficiency we assume that the number of sources $k$ that have non-zero \quantity{} is small compared to $n$, or $k \ll n$.
Concretely, this assumption can be verified when data is corrupted due to user error, which tends to affect only a small portion of the overall training set; or when the predictions under scrutiny arise from queries on the tails of the distribution, which are typically influenced by only a few examples in the training data~\cite{feldman2020neural,ghorbani_data_nodate}.

We also assume that neutral sources are \emph{independent} of the final utility of a subset, conditioned on the probability of source inclusion $p$ and other sources.
Formally, $U(S) \perp\!\!\!\perp \mathbf1_{i\in S} | \left((\mathbf 1_{j\in S})_{j\neq i},p\right)$, where $\mathbf1_{condition}$ is an indicator function that evaluates to 1 if $condition$ is true and 0 otherwise.
% We further assume that any neutral source $i$ is \emph{independent} of the final utility of a subset, conditioned on the other sources. In other words, $U(S)$ has same distribution as $U(S+\{i\})$, for any $S$ not including $i$.
This assumption states that whether or not a neutral source is included in $S$ has no more effect on the value of $U(S)$ than the effect from including any neutral source with probability $p$ in the baseline model.
Under this assumption, we can control the precision of our approach to separate neutral sources from proponents and opponents (\S\ref{subsec:knockoffs}).
% We assume independence so that we can control our approach's precision and separate neutrals from other sources.
% This assumption allows us to control the precision of our identification approach, separating neutrals from proponents and opponents.

% These assumptions are particularly relevant in an adversarial context, such as that of data poisoning.
% Our sparsity assumption implies that when data is deliberately altered, the attacker is only able to poison a small number of sources, perhaps due to limited resources they have at hand.
% Our independence assumption implies that an attacker cannot create strong dependencies between the utility and neutral sources based on altering a small number of sources.
In an adversarial context, such as data poisoning, the sparsity assumption merely implies that attackers control a small portion of sources and the independence assumption implies that adding or removing a neutral source does not significantly impact utility. Finally, for the adversarial setting we also assume that a poisoned source $i$ has $\textrm{AME}_i > 0$. That is, an attacker cannot craft a poisoned source 
such that $U(S^i+\{i\}) - U(S^i)$ is negative at some $p$ values and positive at other $p$ values, while still yielding a working poisoning attack on the main model $\mathcal{M}$. Requiring that poison sources monotonically affect $U(S)$ is sufficient, but not necessary, for ensuring this assumption. %However, monotonicity is a stronger assumption than our requirement.% that $\textrm{AME}_i > 0$. 
%however, so the underlying threat model assumption is weaker.

Outside of these assumptions, our threat model assumes the attacker has access to the model's architecture, its parameters, and the training algorithm used. Attackers also have access to the sample distribution $\mathcal L^i_\mathcal{P}$, but not the specific draws from it used to create the subset models.

%\sid{See below for some more detail about the sparsity assumption that I removed from the intro; we may want to include some of those points here.}
\ignore{
Indeed, it is reasonable to assume sparse contribution. For instance, in the case of data poisoning detection, the attacker is typically only able to poison a limited number of sources given their limited resources at hand. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \notejinkun{I remember the previous sentence does not make sense for Sid. Maybe need to rewrite or remove.}
}

\ignore{
We also make a \emph{monotonicity assumption}. 
Now the monotonicity assumption can be stated as follows: given any proponent/opponent $i$, its marginal effect on $S$, \ie $U(S+\{i\})-U(S)$, is non-negative/non-positive for every $S\subseteq [n]-i$, where $[n]=\{1,2,\dots,n\}$; Moreover, There exists at least one subset on which the marginal effect is non-zero (otherwise this source should be considered as neutral). Intuitively, in the application of corrupted data detection, the assumption roughly translates to that adding a corrupted source makes the prediction more corrupted or equally corrupted. Though the assumption is strong as it requires to hold on every subset, it is stronger than necessary for our quantity (discussed in \S\ref{subsec:ame}) to work. At a high level, as long as the overall \emph{average} effect on multiple subsets has the right sign, our quantity should work.
}

%\paragraph{Threat model}
%When applying our technique to the poison detection scenario, the threat model will be (1) attackers have control over a few training data sources; (2) attackers can have the access to the model parameters and the training algorithm; (3) attackers do not have access to the sample distribution $\mathcal L^i$. 

\ignore{
\sid{
\subsection{Efficient Approximation of the Ideal Distribution}
Jinkun/Mathias: Can you move whatever is needed from this subsection to section 3.1? I think it's fine to motivate the need for uniform p's in the previous subsection, but explicitly stating our solution should be reserved for the methodology section.
}

However, achieving strict equalities of probabilities in Eq. \ref{eq:eq} makes the AME coincide with Shapley value (SV) \cite{jia_towards_2020,ghorbani_data_nodate}, which is costly to measure. Therefore, we must approximate it to enable efficient estimation through regression and LASSO.

For our approximation, we sample sources by including each source (except for the source being measured) with probability $P$, where $P$ is a set of probability values, e.g. $\mathcal P=\{p_1,\dots, p_b\}$ for $b$ different values. 
Note that $p_i\times n$ is the expected size of the subset when sampling with probability $p_i$.  Thus, to approximate the uniform coverage requirement, we populate $\mathcal P$ using a 1D grid within a reasonable range and taking all the grid points (\eg $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$). In the case when there is some prior knowledge about the number of proponent/opponent sources, one may opt to use a different $\mathcal P$ (e.g. tighter ranges, closer-by grid-points)\footnote{Alternatively a different coding or sample weights in the regression is also possible. See \S\ref{subsec:lasso}}. We denote by $\mathcal{L}^i_{\mathcal{P}}$ the subset distribution induced by $\mathcal P$ for source $i$. So our approximated $AME$ under this sampled population is
\begin{equation}
\label{eq:amep}
AME_i(\mathcal L^i_{\mathcal{P}})=\mathbb E_{S^i\sim \mathcal L^i_{\mathcal{P}}}[U(S^i+\{i\}) - U(S^i)].
\end{equation}
From now on when we write $AME_i$ we mean $AME_i(\mathcal L^i_{\mathcal{P}})$.
}



\ignore{
How to choose a suitable range and grid-point distance for $\mathcal{P}$? 
First, $\mathcal{P}$ should be sparse, i.e. $|\mathcal{P}|$ is small. This is to help achieve a good estimation in later procedure that will be discussed shortly (see \S\ref{subsec:sampling}).
Second, the range of $\mathcal{P}$ should not include probability values that are too low. With a very low $p$, the sampled subset contains too few sources, so that the resulting model will fail to learn the distinguished features that predict the query label, and thus is not useful for identifying proponents.
Third, very high $p$ should not be included either, because such $p$'s would make little change to the original dataset, and thus suffer from the same issue as the traditional LOO test. 
For our experiments in Sec~\ref{sec:eval}, we use $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$ unless otherwise specified.
}

% A tempting straightforward alternative is to sample each possible subset of sources uniformly.  This corresponds to sampling each source using $\mathcal P=\{0.5\}$. However, this straightforward approach deviates significantly from the uniform coverage requirement. In experiments of poison detection we find that the grid version is more robust. This is because, more often than not, the subsets with the most marginal effects do not include half of the sources. \notejinkun{Panda and I have agreed to move this experiment to appendix. Maybe we remove this discussion here as well.}




==> relwork-notes.tex <==
\section{Close Related Work}

\paragraph{Influence}

\paragraph{Shapley Value}
% https://arxiv.org/pdf/1902.10275.pdf
At a high level, this paper is trying to quantify the contribution of each datapoint in a dataset to the utility of a model (e.g. final test set accuracy). The authors advocate for using the Shapley Value, which is the only value that verifies a set of intuitive properties. For each datapoint, it measures the marginal utility improvement when adding this datapoint to every possible subset of other datapoints, and averages those values with weights such that each subset size is equally weighted. This quantity is very expensive computationally, and they propose ways to approximate it with guarantees for ML tasks.

The quantity is close to ours. How exactly?

The closest approximation to our work is the sparse utility approach, which uses compressive sensing to recover the SV for all points from much fewer aggregate measurements. While we use a different tool for sparse recovery, this is very related.
The main difference is that computing the aggregate measurements is more expensive in the proposed algorithm. Indeed, it requires a few samples (O(log(log(N))) but they each need O(N) utility estimations (i.e. model training) to be computed. Our approach requires O(Klog(N)) samples, but each requires only one training, which is much more efficient on sparse signals (K << N).
It is possible that a similar approach could be used to improve SV estimation.

They need a monotonicity assumption for the sparse approach. I think we do too.

==> rm/ame-v1.tex <==
\section{Average Marginal Effect (\quantity{})}
\label{subsec:ame}
Figure \ref{fig:workflow}

\sid{This is indeed a bit bottom-up, but if our previous motivation/problem formulation section makes it clear why AME is the core metric we need, I think it could work. We should retitle this section to indicate this is how we measure the effect of proponents.}
\notepanda{I am concerned that the paper might be very bottom up. I think as a reader I would be unhappy here, asking why do I need to learn about this quantity that so far has not been used in the paper. I think we want to go top-down, motivate why this quantity, how we use it, and then formally define it.}

\sid{Include straw solutions here regarding what quantity to measure, such as LOO?}

\subsection{Motivation}
\label{subsec:ame-mov}
\sid{I would call this "Intuition" and consider using a slash-paragraph instead}

To solve this problem, we want to have a measure for each source of how much it contributed to the prediction, and then select those having a high measurement. One straightforward approach is LOO test, i.e. measure the change in model's output after removing the source of interest. Note that this is also what influence functions \cite{koh_understanding_2017} try to approximate. %We term it \textit{LOO change} or \textit{influence} for short.% Finally select those greater than a threshold.
However, ML algorithms are oftentimes complex and non-linear, and that means that removing one proponent may not be able to change the model. For example, consider the case of 1-Nearest-Neighbor algorithm, if there are two identical nearest points of the query input residing in two different sources $i_1$ and $i_2$, the model's output will not change unless both sources are removed.% Similar phenomenon also occurs in deep learning. E.g. in CIFAR10, there are in total 50k examples in the training set, and removing one of them brings only very little impact, which is likely obscured by the noise. Our experiments also partly verify this hypothesis (see Fig. \ref{fig:diff-tfs} and the evaluation for detail).

Though removing only $i_1$ or $i_2$ changes nothing, but if the model were trained on any subset that does not contain $i_2$ (or $i_1$), removing $i_1$ (or $i_2$) probably changes the model, \ie it has a non-zero marginal effect on such subsets. This motivates us to consider sampling subsets and doing LOO tests on them. We will observe a positive effect on subsets without $i_2$, and otherwise zero. By averaging on multiple subsets, it would be very likely to give a positive value for $i_1$, which suggests that this average effect is able to flag proponents and thus could be the quantity we are looking for.

\notejinkun{this paragraph is somewhat duplicated with the monotonicity assum (monotonicity is sort of another pitch that I did not adopt before). We may only want to keep one. If we chooses monotoncity pitch, it could be more succinct but we may need experiments or additional text similar as what this paragraph to support it. I would prefer experiments, because readers may not like read a bunch of text.} For general ML algorithms other than 1NN, this quantity may still be useful. The intuition is that for any ML algorithm, we know removing one proponent may have zero effect, while removing the whole proponent group should have a significant effect. Thus if the proponents are removed one by one, the effect will ultimately changes from zero to significant, so there must be a point in the middle when removing one proponent changes the effect at least some. This is when LOO test gives a non-zero effect, but different than usual LOO test, this time it is removing from a subset where some other proponents have been removed. We want to have a non-zero effect measured for each proponent, thus we want to create a population that includes such subsets. We are able to sample such subsets by subsampling from the full dataset, but it comes with the side effect that the non-proponents are also subsampled. Here by the sparsity assumption non-proponent data should be sufficient so that their subsampling does not have a large impact on the outcome. 

Therefore, this quantity should still be able to give non-zero values for proponents. For neutrals, the effects on any subset would be around zero and so is the quantity. For opponents, everything would just be the opposite and so would be the quantity. Therefore, we argue that this quantity is able to discern proponents, opponents and neutrals.

\notejinkun{I would rewrite previous 2 paragraphs as following, if we use monotonicity assumption:} More generally for any model, as long as the monotonicity assumption verifies, this average marginal effect will be able to give positive/negative values for proponents/oppponents, and zeros for neutrals by the sparsity assumption, making it a reasonable quantity to discern between proponents, opponents and neutrals.

\subsection{Defining AME}
\sid{I would consider using a slash-paragraph instead}
%\notejinkun{This name is problematic, because influence is the opposite number of what we are measuring (influence is defined as $U(S-{i})-U(S)$). Maybe a better name, like still Average Marginal Effect?}}
% Now we give formal definition of this quantity.  % Sometimes we abbreviate to \textit{signal} of the subset $S$.
    % \item \textit{marginal effect} or \textit{LOO effect\notejinkun{I was calling it LOO effect but feel like LOO effect should be its opposite number, so to avoid ambiguity I changed the name... But if you feel more confused, or feel LOO effect is fine, I'll change it back.}} of a source $i$ on a subset $S$ that excludes $i$ is defined as $U(S+\{i\})-U(S)$. %Sometimes we also call it \textit{LOO effect}.
% \end{enumerate}


Given a subset sampling distribution $\mathcal{L}^i$, we define a quantity called \textit{Average Marginal Effect (\quantity{})} for source $i$ as the average marginal effect of $i$ on these subsets. Formally,

% We define for every training source a quantity called \textit{Average Marginal Effect (\quantity{})} that indicates a proponent for a positive value, opponent for a negative value or neutral for a zero value.

% \paragraph{Motivation} By the second property there is a subset of the proponent group such that the marginal effect of $k_i$ is positive, so we want to create a population of such subsets. However, the group is unknown, so we have to subsample the whole dataset, and that has a side effect that the non-proponent data are also subsampled. We make an assumption that they are sufficiently large that doing a (not-too-aggresive) subsampling does not very much affect their distribution, so that removing $k_i$ still has same effect as when the non-proponents are not subsampled. It follows that $k_i$ unlikely has a negative marginal effect in any case. Therefore, the marginal effects in the population are mostly non-negative, and when we average them, it would be positive. Call this average marginal effect \textit{\quantity{}}. For opponents, the \quantity{} should likely be the negative for the same reason, and for other data points, the \quantity{} should likely be zero.

% Let $\mathcal L^i$ be the population we want to create for estimating source $i$, the \quantity{} can then be formalized as 
\begin{equation}
\label{eq:ame}
AME_i(\mathcal L^i)=\mathbb E_{S^i\sim \mathcal L^i}[U(S^i+\{i\}) - U(S^i)],
\end{equation}
Note that for the definition to be meaningful, $\mathcal{L}^i$ should not include subsets containing $i$.
% \begin{figure*}[h]
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/direct-cifar10-20.png}
%         \caption{EMNIST\fixme{TODO}}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/direct-cifar10-20.png}
%         \caption{CIFAR10-20}
%     \end{subfigure}
%     \caption{Average marginal effect of 5 random poisoned training examples and 15 random benign ones on subsets of size $np$ for each $p$. Each point is averaged on 6 randomly selected subsets of corresponding size. Notice that $p=0.01$ works well for EMNIST while fails for CIFAR10-20, and vice versa for $p=0.4$.}
%     \label{fig:LOO-effect}
% \end{figure*}

\subsection{Ideal Population without Prior Knowledge}
\sid{I would remove this subsection and blend it into the prose, as we are simply building up towards equation (3).}
When prior knowledge is not available, we recommend a population that covers uniformly for different sizes of subsets. In other words, there would be roughly the same number of subsets sampled for each size. Formally, the population should verify a \textit{uniform coverage requirement}
\begin{equation}
\label{eq:eq}
    \mathbb P[|S^i|=0]= \dots =\mathbb P[|S^i|=n-1],
\end{equation}

The reason is that we observe that the marginal effect will be non-zero in subsets of sizes in some certain (sometimes narrow) ranges, which however tend to vary across different applications.
For example, Fig. \ref{fig:LOO-effect} \notejinkun{As discussed this morning, we are not going to include the AME plots.} shows results in our poison detection experiments, where the marginal effect of real poisoned sources only becomes significantly larger than the rest on the subsets of size lying within a certain range, %\footnote{we use $P$ as a proxy of subset size since in expectation the size is $Pn$}
which varies across different attacks/datasets. A possible explanation could be that the signal exhibits a dataset- or attack-specific threshold-function characteristic w.r.t. the number of proponents included. That is, there is no signal when there are fewer than a threshold of proponents included, and a strong signal when more included. To have non-zero effect measured, we need to robustly capture the changing phase. Without prior knowledge on the dataset/queries, we opt to sample subsets on different sizes uniformly, \ie Eq. \ref{eq:eq}.

\subsection{$P$-associated Population}
\label{sec:p-pop}
\sid{Again, I would remove this header and blend with our build-up to eq. (3).}
Achieving strict equalities of probabilities in Eq. \ref{eq:eq} makes the AME coincide with Shapley Value (SV) \cite{jia_towards_2020}, which is costly to measure. Instead, we approximate it through a proxy of $P$. Doing so allows further efficient estimation through regression and LASSO.

Specifically, we first draw a probability of inclusion, $P$, \textbf{uniformly} from a set $\mathcal P=\{p_1,\dots, p_b\}$ containing $b$ different values, then include every source (except the source being measured) with probability $P$. We highlight the fact that $Pn$ is the expected size of the subset, thus to fulfill the uniform coverage requirement, $\mathcal P$ is obtained by making a uniform grid in a reasonable range and taking all the grid points (\eg $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$). In the case where the characteristics of the application is known a priori, one may instead opt to design accordingly the distribution of $\mathcal P$ \footnote{Alternatively a different coding or sample weights in the regression is also possible. See \S\ref{subsec:lasso}}. We denote by $\mathcal{L}^i_{\mathcal{P}}$ the subset distribution induced by $\mathcal P$ for source $i$. And the $AME$ under this new population is
\begin{equation}
\label{eq:amep}
AME_i(\mathcal L^i_{\mathcal{P}})=\mathbb E_{S^i\sim \mathcal L^i_{\mathcal{P}}}[U(S^i+\{i\}) - U(S^i)].
\end{equation}
From now on when we write $AME_i$ we mean $AME_i(\mathcal L^i_{\mathcal{P}})$.
% Sometimes we abbreviate $AME_i(\mathcal L^i_{\mathcal{P}})$ to $AME_i$.% when the population or the source is unambiguous in the context.
\paragraph{Designing the grid $\mathcal{P}$}  
\sid{I would blend all of this into our subset sizing arguments in the previous page.}
\mathias{I am moving this into the methodology (empirical claims about specific numbers should probably even move to the microbenchmarks in eval). Not sure what you're referring to @Sid, the motivation seems a bit early to talk about something that specific but ping me if I'm missing something.}
\iffalse
First, it should be sparse, i.e. $b$ is small. This is to help achieve a good estimation in later procedure that will be discussed shortly (see \S\ref{subsec:sampling}). %LASSO is essentially aggregating the result for each $P$, and aggregating a lot of bad results is no better than aggregating a few good results. By making it sparse, each $P$ can have a better result. Too dense or even doing continuous sampling instead would probably yield garbage output for each $P$. 

\notejinkun{this is for the original verision without monontonicity assumption} Second very low $P$ should not be included. Because too low a $P$ subsamples too few sources, in which the non-proponents' distribution may deviate too far away from the full dataset. In such a case, adding/removing one source could have very different results. For example, consider each source contains only data of one label, and $P$ is so small that $S^i$ is empty. Now $U(S^i+\{i\})=U(\{i\})$ is obtained by training model on only source $i$ that has only one label, meaning that it always would predict the source's label. Thus its marginal effect collapses into always giving high value for a source sharing label the same as the query label. However, not every such source is causing the query prediction, especially in the case of one training example per source.

\fixme{subject to change before the experiment result is out}\notejinkun{this is for the new verision with monontonicity assumption} Second very low $P$ should not be included. Because too low a $P$ subsamples too few sources, in which the model has no information to infer about the input and thus has to guess randomly. The monotonicity assumption tends to break under this situation, potentially creating many false positives.% In the previous running example, suppose $S$ only contains source $2a$, then the trained model would produce label '2' for any input. If we add the clean source $1a$ into $S$, the model would likely flips a coin to choose between '1' and '2', which appears as if source $1a$ has a positive marginal effect, even if $1a$ is not the cause of the poisoned prediction. %For example, \fixme{we could use the running example if it is exactly what is described here} consider MNIST example where there are 10 sources each containing only data of one label, and the query is an image of poisoned 0 being predicted as 1 because of malicious source 1. If $P$ is so small that $S$ is only $\{2\}$, adding $0$ to $S^i$ would  obtained by training model on only source $i$ that has only one label, meaning that it always would predict the source's label. Thus its marginal effect collapses into always giving high value for a source sharing label the same as the query label. However, not every such source is causing the query prediction, especially in the case of one training example per source.

\notejinkun{version 3 of previous paragraph}
Second very low $P$ should not be included. Because too low a $P$ subsamples too few sources, in which, the model is not able to learn the distinguished features that cause the query label predicted, and thus not useful for identifying proponents. In Alice's case, the model would fail to learn the watermark and predicts as if there is no watermark.

Third, very high $P$ should not be included either. Too high a $P$ would almost make no change to the dataset, and thus suffer from the same issue as the traditional LOO test (see the previous 1-Nearest-Neighbor for a detailed example). 



% Finally, We demonstrate that it is robust in that it performs well across a wide range of applications, and compare against fixing $P=0.5$ Experimental results are shown in Tab. \ref{tab:p0.5}. \fixme{TODO: experiments. Ideally find at least one case where $P=0.5$ is worse in training-from-scratch. Now EMNIST has an experiment of $P=0.5$ and it's worse than uniform p.}.


There is also a variance issue in practice that prohibits very low/high $P$ (see \S\ref{subsec:sampling}). We use $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$ unless otherwise specified.
\fi

\subsection{Why Not Sample each Subset Uniformly?}
Another worth-mentioning, and perhaps the most straightforward population is to draw each subset uniformly with equal probability. This actually corresponds to $\mathcal P=\{0.5\}$. However, it does poorly in fulfilling the uniform coverage requirement, and in experiments of poison detection we find that the grid version is more robust because the subsets that gives the most signal is not always of around half size.

% Justifying the approach of introducing $P$ to sample subsets: achieving strict equality is costly, so we approximate it by weighting each $P\in \mathcal P$ equally, where $\mathcal P$ ideally contains values uniformly distributed in $[0,1]$. Benefit of introducing $P$. This is an approximation since $pn$ is the expected subset set sampled using $P=p$: enable the use of OLS and LASSO and the $O(k\log n)$ finite sample error bound. 

% Justifying the choice of $\mathcal P$: we use $\{0.2,0.4,0.6,0.8\}$ by default. Reason for why it is very sparse: LASSO is essentially aggregating the result for each $P$, and aggregating a lot of bad results is no better than aggregating a few good results. By making it sparse, each $P$ can have a better result. Too dense or even doing continuous sampling instead would probably yield garbage output for each $P$. Reason for not including very low or high $P$: On the one hand, the quantity is measuring the change after removing one source from a subset, the subset should not deviate too far away from the full dataset, otherwise the change could not represent the contribution in the full dataset. Thus too low a $P$ is not favorable. On the other hand, too high a $P$ would almost make no change to the dataset, and thus suffer from the same issue as the traditional LOO test. We demonstrate that it is robust in that it performs well across a wide range of applications, and compare against fixing $P=0.5$ Experimental results are shown in Tab. \ref{tab:p0.5}. \fixme{TODO: experiments. Ideally find at least one case where $P=0.5$ is worse in training-from-scratch. Now EMNIST has an experiment of $P=0.5$ and it's worse than uniform p.}.
% \fixme{TODO: Experiments}

==> rm/ame-v2.tex <==
\section{Average Marginal Effect (\quantity{})}
\label{subsec:ame}
%Figure \ref{fig:workflow}

%\sid{This is indeed a bit bottom-up, but if our previous motivation/problem formulation section makes it clear why AME is the core metric we need, I think it could work. We should retitle this section to indicate this is how we measure the effect of proponents.}
%\notepanda{I am concerned that the paper might be very bottom up. I think as a reader I would be unhappy here, asking why do I need to learn about this quantity that so far has not been used in the paper. I think we want to go top-down, motivate why this quantity, how we use it, and then formally define it.}

%\sid{Include straw solutions here regarding what quantity to measure, such as LOO?}

%\subsection{Motivation}
%\label{subsec:ame-mov}
%\sid{I would call this "Intuition" and consider using a slash-paragraph instead}

\noindent{\bf Intuition.} To quantify ``provenance'', we need to measure, for each source, how much it contributes to a given prediction. One naive approach is the ``leave one out'' (LOO) test, which measures the change in the model's prediction when trained without the source of interest. As the influence function~\cite{koh_understanding_2017} also aims to quantify the effect of adding/removing a training datapoint, it can be viewed as a form of LOO test. %We term it \textit{LOO change} or \textit{influence} for short.% Finally select those greater than a threshold.
However, under complex and non-linear ML algorithms, LOO tests can fail because removing one source may not cause change in the model's output. For example, consider the case of 1-nearest-neighbor algorithm, if there are two identical nearest points of the query input residing in two separate sources $i$ and $j$, the model's output will not change unless both proponent sources are removed.% Similar phenomenon also occurs in deep learning. E.g. in CIFAR10, there are in total 50k examples in the training set, and removing one of them brings only very little impact, which is likely obscured by the noise. Our experiments also partly verify this hypothesis (see Fig. \ref{fig:diff-tfs} and the evaluation for detail).

The failure of naive LOO stems from its inflexibility: when determining the contribution of source $i$, LOO measures the marginal effect of training with and without $i$ but always in the presence of {\em all} remaining sources. To address LOO's limitation while keeping its intuition, we allow more flexibility in the cohort of sources that $i$ is trained with or without when determining $i$'s contribution. For maximum flexibility, the cohorts can be sampled following some distribution from the $n$ original sources, with the effects averaged across sampled cohorts. For example, in our previous 1-nearest-neighbor example with two contributing sources $i$ and $j$, if $i$ is trained with and without a sampled subset of sources that does not contain $j$, then we will be able to observe non-zero marginal
effects when comparing the resulting models.

%While removing one from $n$ original sources may not change a model's output,  

%Though removing only $i_1$ or $i_2$ changes nothing, but if the model were trained on any subset that does not contain $i_2$ (or $i_1$), removing $i_1$ (or $i_2$) probably changes the model, \ie it has a non-zero marginal effect on such subsets. This motivates us to consider sampling subsets and doing LOO tests on them. We will observe a positive effect on subsets without $i_2$, and otherwise zero. By averaging on multiple subsets, it would be very likely to give a positive value for $i_1$, which suggests that this average effect is able to flag proponents and thus could be the quantity we are looking for.

%\notejinkun{this paragraph is somewhat duplicated with the monotonicity assumption (monotonicity is sort of another pitch that I did not adopt before). We may only want to keep one. If we chooses monotoncity pitch, it could be more succinct but we may need experiments or additional text similar as what this paragraph to support it. I would prefer experiments, because readers may not like read a bunch of text.} 

%For general ML algorithms other than 1NN, this quantity may still be useful. The intuition is that for any ML algorithm, we know removing one proponent may have zero effect, while removing the whole proponent group should have a significant effect. Thus if the proponents are removed one by one, the effect will ultimately changes from zero to significant, so there must be a point in the middle when removing one proponent changes the effect at least some. This is when LOO test gives a non-zero effect, but different than usual LOO test, this time it is removing from a subset where some other proponents have been removed. We want to have a non-zero effect measured for each proponent, thus we want to create a population that includes such subsets. We are able to sample such subsets by subsampling from the full dataset, but it comes with the side effect that the non-proponents are also subsampled. Here by the sparsity assumption non-proponent data should be sufficient so that their subsampling does not have a large impact on the outcome. 

%Therefore, this quantity should still be able to give non-zero values for proponents. For neutrals, the effects on any subset would be around zero and so is the quantity. For opponents, everything would just be the opposite and so would be the quantity. Therefore, we argue that this quantity is able to discern proponents, opponents and neutrals.

%\notejinkun{I would rewrite previous 2 paragraphs as following, if we use monotonicity assumption:} More generally for any model, as long as the monotonicity assumption verifies, this average marginal effect will be able to give positive/negative values for proponents/oppponents, and zeros for neutrals by the sparsity assumption, making it a reasonable quantity to discern between proponents, opponents and neutrals.


%\notejinkun{This name is problematic, because influence is the opposite number of what we are measuring (influence is defined as $U(S-{i})-U(S)$). Maybe a better name, like still Average Marginal Effect?}}
% Now we give formal definition of this quantity.  % Sometimes we abbreviate to \textit{signal} of the subset $S$.
    % \item \textit{marginal effect} or \textit{LOO effect\notejinkun{I was calling it LOO effect but feel like LOO effect should be its opposite number, so to avoid ambiguity I changed the name... But if you feel more confused, or feel LOO effect is fine, I'll change it back.}} of a source $i$ on a subset $S$ that excludes $i$ is defined as $U(S+\{i\})-U(S)$. %Sometimes we also call it \textit{LOO effect}.
% \end{enumerate}


\vspace{0.1in}
\noindent{\bf Definition.} Formally speaking, to estimate a source $i$'s contribution, we measure a quantity called \textit{Average Marginal Effect (\quantity{})}, which is defined as the expected marginal effects over a subset sampling distribution $\mathcal{L}^i$, as follows: 

% We define for every training source a quantity called \textit{Average Marginal Effect (\quantity{})} that indicates a proponent for a positive value, opponent for a negative value or neutral for a zero value.

% \paragraph{Motivation} By the second property there is a subset of the proponent group such that the marginal effect of $k_i$ is positive, so we want to create a population of such subsets. However, the group is unknown, so we have to subsample the whole dataset, and that has a side effect that the non-proponent data are also subsampled. We make an assumption that they are sufficiently large that doing a (not-too-aggresive) subsampling does not very much affect their distribution, so that removing $k_i$ still has same effect as when the non-proponents are not subsampled. It follows that $k_i$ unlikely has a negative marginal effect in any case. Therefore, the marginal effects in the population are mostly non-negative, and when we average them, it would be positive. Call this average marginal effect \textit{\quantity{}}. For opponents, the \quantity{} should likely be the negative for the same reason, and for other data points, the \quantity{} should likely be zero.

% Let $\mathcal L^i$ be the population we want to create for estimating source $i$, the \quantity{} can then be formalized as 
\begin{equation}
\label{eq:ame}
AME_i(\mathcal L^i)=\mathbb E_{S^i\sim \mathcal L^i}[U(S^i+\{i\}) - U(S^i)]
\end{equation}
In Equation~\ref{eq:ame}, $S^i$ is a subset of sources sampled from distribution $\mathcal L^i$, and the marginal effect of $i$ according to $S^i$ is calculated as the difference in the model's output when trained with and without $i$, aka $U(S^i+\{i\})-U(S^i)$. Note that for the definition to be meaningful, none of the subsets sampled from $\mathcal{L}^i$ should contain $i$, i.e. $i\notin S^i, \forall S^i\sim \mathcal L^i$.
% \begin{figure*}[h]
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/direct-cifar10-20.png}
%         \caption{EMNIST\fixme{TODO}}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/direct-cifar10-20.png}
%         \caption{CIFAR10-20}
%     \end{subfigure}
%     \caption{Average marginal effect of 5 random poisoned training examples and 15 random benign ones on subsets of size $np$ for each $p$. Each point is averaged on 6 randomly selected subsets of corresponding size. Notice that $p=0.01$ works well for EMNIST while fails for CIFAR10-20, and vice versa for $p=0.4$.}
%     \label{fig:LOO-effect}
% \end{figure*}

Under the monoticity assumption, we can argue that the $AME$ is a non-zero \notejinkun{Should we say "positive" (since they are for proponent sources)?} value for any\jinyang{is it "any" or "some"?}\notejinkun{I think it's any if my English is correct. What I meant to convey is that every proponent will have a positive AME under the assumption.} proponent source.  To see this, consider removing all proponent sources one by one. We observe that the sum of the marginal effects calculated between successive removals is equal to the overall effect of all proponents, which is non-zero. Suppose the overall effect is positive \notejinkun{The effect should always be positive since it is confidence and within [0,1].}, there exists source $i$ and subset $S_i$ whose removal (from $S_i+{i}$ to $S_i$) results in a positive marginal effect, since the monoticity assumption guarantees that all successive removals have non-negative marginal effects. As long as subset $S_i$ can be sampled from distribution $L_i$, the resulting $AME_i$ will be positive.  Ditto if the overall effect is negative.
For any neutral source, its effect on any subset is around zero and so is the corresponding $AME$. \notejinkun{@Jinyang Sorry I don't quite understand the previous paragraph. Maybe we should talk about this synchronously}

%\subsection{Ideal Population without Prior Knowledge}
%\sid{I would remove this subsection and blend it into the prose, as we are simply building up towards equation (3).}
\vspace{0.1in}
\noindent{\bf Selecting subset sample distribution.} When we have no prior knowledge on the number of proponent/opponent sources, it is best to sample from a population distribution that is uniform across different subset sizes. In other words, there should be roughly the same number of subsets sampled for each size. Formally, the population should satisfy the \textit{uniform coverage requirement}
\begin{equation}
\label{eq:eq}
    \mathbb P[|S^i|=0]= \dots =\mathbb P[|S^i|=n-1],
\end{equation}

When the sizes of subsets sampled are uniform, we ensure that some marginal effects will be non-zero, regardless of the number of proponents/opponent sources present. This is true even if the signal exhibits a threshold-function characteristic such that there is no marginal effect unless a threshold of proponents appear in the training.  With uniform size sampling, we can robustly capture the point where the marginal effect changes from zero to non-zero, without relying on any prior knowledge.  However, achieving strict equalities of probabilities in Eq. \ref{eq:eq} makes the AME coincide with Shapley Value (SV) \cite{jia_towards_2020}, which is costly to measure. Therefore, we must approximate it to enable efficient estimation through regression and LASSO.

%For example, Fig. \ref{fig:LOO-effect} \notejinkun{As discussed this morning, we are not going to include the AME plots.} shows results in our poison detection experiments, where the marginal effect of real poisoned sources only becomes significantly larger than the rest on the subsets of size lying within a certain range, %\footnote{we use $P$ as a proxy of subset size since in expectation the size is $Pn$}
%which varies across different attacks/datasets. A possible explanation could be that the signal exhibits a dataset- or attack-specific threshold-function characteristic w.r.t. the number of proponents included. That is, there is no signal when there are fewer than a threshold of proponents included, and a strong signal when more included. To have non-zero effect measured, we need to robustly capture the changing phase. Without prior knowledge on the dataset/queries, we opt to sample subsets on different sizes uniformly, \ie Eq. \ref{eq:eq}.

%\subsection{$P$-associated Population}
%\label{sec:p-pop}
%\sid{Again, I would remove this header and blend with our build-up to eq. (3).}

For our approximation, we sample sources by including each source (except for the source being measured) with probability $P$, where $P$ is a set of probability values, e.g. $\mathcal P=\{p_1,\dots, p_b\}$ for $b$ different values. 
Note that $P_i*n$ is the expected size of the subset when sampling with probability $p_i$.  Thus, to approximate the uniform coverage requirement, we populate $\mathcal P$ using a 1D grid within a reasonable range and taking all the grid points (\eg $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$). In the case when there is some prior knowledge about the number of proponent/opponent sources, one may opt to use a different $\mathcal P$ (e.g. tighter ranges, closer-by grid-points)\footnote{Alternatively a different coding or sample weights in the regression is also possible. See \S\ref{subsec:lasso}}. We denote by $\mathcal{L}^i_{\mathcal{P}}$ the subset distribution induced by $\mathcal P$ for source $i$. So our approximated $AME$ under this sampled population is
\begin{equation}
\label{eq:amep}
AME_i(\mathcal L^i_{\mathcal{P}})=\mathbb E_{S^i\sim \mathcal L^i_{\mathcal{P}}}[U(S^i+\{i\}) - U(S^i)].
\end{equation}
From now on when we write $AME_i$ we mean $AME_i(\mathcal L^i_{\mathcal{P}})$.
% Sometimes we abbreviate $AME_i(\mathcal L^i_{\mathcal{P}})$ to $AME_i$.% when the population or the source is unambiguous in the context.
%\paragraph{Designing the grid $\mathcal{P}$}  
%\sid{I would blend all of this into our subset sizing arguments in the previous page.}
%\mathias{I am moving this into the methodology (empirical claims about specific numbers should probably even move to the microbenchmarks in eval). Not sure what you're referring to @Sid, the motivation seems a bit early to talk about something that specific but ping me if I'm missing something.}
%\iffalse
%First, it should be sparse, i.e. $b$ is small. This is to help achieve a good estimation in later procedure that will be discussed shortly (see \S\ref{subsec:sampling}). %LASSO is essentially aggregating the result for each $P$, and aggregating a lot of bad results is no better than aggregating a few good results. By making it sparse, each $P$ can have a better result. Too dense or even doing continuous sampling instead would probably yield garbage output for each $P$. 

%\notejinkun{this is for the original version without monotonicity assumption} 
How to choose a suitable range and grid-point distance for $\mathcal{P}$? 
First, $\mathcal{P}$ should be sparse, i.e. $|\mathcal{P}|$ is small. This is to help achieve a good estimation in later procedure that will be discussed shortly (see \S\ref{subsec:sampling}) \notejinkun{Make sure we discuss why we need sparse grid somewhere (either here or the referred place?) Also I remember Mathias moved the whole part of "how to design the grid" to methodology.}.
Second, the range of $\mathcal{P}$ should not include probability values that are too low. With a very low $p$, the sampled subset contains too few sources, so that the resulting model will fail to learn the distinguished features that predict the query label, and thus is not useful for identifying proponents. % In Alice's case, the model would fail to learn the watermark and predicts as if there is no watermark. %With a very low $p$, the sampled subset contains too few sources, so the non-proponents' distribution may deviate too much from the full dataset. %In such a case, adding/removing one source could have very different results. 
%For example, suppose each source contains only data of one label, and $P$ is so small that $S^i$ is empty. Now $U(S^i+\{i\})=U(\{i\})$ is obtained by training model on only source $i$ that has only one label, meaning that it would always  predict the source's label. Thus its marginal effect is always high for a source sharing label the same as the query label. However, not every such source is causing the query prediction, especially in the case of one training example per source.
%\fixme{subject to change before the experiment result is out}\notejinkun{this is for the new version with monotonicity assumption} Second very low $P$ should not be included. Because too low a $P$ subsamples too few sources, in which the model has no information to infer about the input and thus has to guess randomly. The monotonicity assumption tends to break under this situation, potentially creating many false positives.% In the previous running example, suppose $S$ only contains source $2a$, then the trained model would produce label '2' for any input. If we add the clean source $1a$ into $S$, the model would likely flips a coin to choose between '1' and '2', which appears as if source $1a$ has a positive marginal effect, even if $1a$ is not the cause of the poisoned prediction. %For example, \fixme{we could use the running example if it is exactly what is described here} consider MNIST example where there are 10 sources each containing only data of one label, and the query is an image of poisoned 0 being predicted as 1 because of malicious source 1. If $P$ is so small that $S$ is only $\{2\}$, adding $0$ to $S^i$ would  obtained by training model on only source $i$ that has only one label, meaning that it always would predict the source's label. Thus its marginal effect collapses into always giving high value for a source sharing label the same as the query label. However, not every such source is causing the query prediction, especially in the case of one training example per source.
%\notejinkun{version 3 of previous paragraph}
%Second very low $P$ should not be included. Because too low a $P$ subsamples too few sources, in which, the model is not able to learn the distinguished features that cause the query label predicted, and thus not useful for identifying proponents. In Alice's case, the model would fail to learn the watermark and predicts as if there is no watermark.
Third, very high $p$ should not be included either, because such $p$'s would make little change to the original dataset, and thus suffer from the same issue as the traditional LOO test. 
% Finally, We demonstrate that it is robust in that it performs well across a wide range of applications, and compare against fixing $P=0.5$ Experimental results are shown in Tab. \ref{tab:p0.5}. \fixme{TODO: experiments. Ideally find at least one case where $P=0.5$ is worse in training-from-scratch. Now EMNIST has an experiment of $P=0.5$ and it's worse than uniform p.}.
%There is also a variance issue in practice that prohibits very low/high $P$ (see \S\ref{subsec:sampling}). 
For our experiments in Sec~\ref{sec:eval}, we use $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$ unless otherwise specified.


%\subsection{Why Not Sample each Subset Uniformly?}
A tempting straightforward alternative is to sample each possible subset of sources uniformly.  This corresponds to sampling each source using $\mathcal P=\{0.5\}$. However, this straightforward approach deviates significantly from the uniform coverage requirement. In experiments of poison detection we find that the grid version is more robust. This is because, more often than not, the subsets with the most marginal effects do not include half of the sources. \notejinkun{Panda and I have agreed to move this experiment to appendix. Maybe we remove this discussion here as well.}

% Justifying the approach of introducing $P$ to sample subsets: achieving strict equality is costly, so we approximate it by weighting each $P\in \mathcal P$ equally, where $\mathcal P$ ideally contains values uniformly distributed in $[0,1]$. Benefit of introducing $P$. This is an approximation since $pn$ is the expected subset set sampled using $P=p$: enable the use of OLS and LASSO and the $O(k\log n)$ finite sample error bound. 

% Justifying the choice of $\mathcal P$: we use $\{0.2,0.4,0.6,0.8\}$ by default. Reason for why it is very sparse: LASSO is essentially aggregating the result for each $P$, and aggregating a lot of bad results is no better than aggregating a few good results. By making it sparse, each $P$ can have a better result. Too dense or even doing continuous sampling instead would probably yield garbage output for each $P$. Reason for not including very low or high $P$: On the one hand, the quantity is measuring the change after removing one source from a subset, the subset should not deviate too far away from the full dataset, otherwise the change could not represent the contribution in the full dataset. Thus too low a $P$ is not favorable. On the other hand, too high a $P$ would almost make no change to the dataset, and thus suffer from the same issue as the traditional LOO test. We demonstrate that it is robust in that it performs well across a wide range of applications, and compare against fixing $P=0.5$ Experimental results are shown in Tab. \ref{tab:p0.5}. \fixme{TODO: experiments. Ideally find at least one case where $P=0.5$ is worse in training-from-scratch. Now EMNIST has an experiment of $P=0.5$ and it's worse than uniform p.}.
% \fixme{TODO: Experiments}

==> rm/approach-v1.tex <==
\section{The Sampling, Training, Estimation and Selection Procedure}
\label{sec: procedure}
\notepanda{Some of this seems to repeat/be out of order with the previous section. For instance \S\ref{subsec:sampling} seems to assume no Lasso, but we introduced this earlier.}

% To identify the proponent group there are four problems we need to solve: (1) we need an efficient subset sampling scheme (\S\ref{subsec:sampling}); (2) we need to train models on these sampled subsets efficiently (\S\ref{subsec:warm-starting}); (3) we need to estimate the quantities accurately using the training results (\S\ref{subsec:lasso}); (4) we need an accurate while powerful procedure for selecting sources using the estimates (\S\ref{subsec:knockoffs}). Doing them naively is either too costly or inaccurate. In the following 4 sections we describe the underlying challenges for each component and how we overcome them respectively.
The problem of identifying the proponent group is thus divided into four steps: (1) subsample subsets (\S\ref{subsec:sampling}); (2) train models on these sampled subsets (\S\ref{subsec:warm-starting}); (3) estimate the \quantity{} using the training results (\S\ref{subsec:lasso}); (4) select sources based on the estimates (\S\ref{subsec:knockoffs}). Doing them naively is either too costly or inaccurate. In the following 4 sections we describe the underlying challenges for each component and how we overcome them respectively.

\subsection{The Sampling Scheme}
\label{subsec:sampling}

\notejinkun{this whole section is just to (i) stating that we want to sample the subsets altogether (\ie reusing subsets for estimating each source; (ii) and showing why this can be still estimating the same thing (\ie by showing the expectation of difference (\eqref{eq:amep}) equals difference of expectation (\eqref{eq:diff-in-means-true}. btw sorry that I pointed to a wrong place during the meeting). Don't hesitate to ping me if you feel confused (which is probably my bad of writing or the argument is truly incorrect)!}

\notepanda{Is this really a viable option? This section read a bit like us beating up on a strawman that obviously would not work: just say it is costly and move on?}

To estimate the $AME_i(\mathcal{L}^i_{\mathcal{P}})$,the most straightforward approach is sampling the subsets and compute their average marginal effects. However, this is too costly, since it requires training two models for each subset, and every source requires the same procedure, thus the models to train is at least $O(n)$. \notejinkun{UPDATED on Feb 21} \sout{What is worse, every source requires many draws to ensure accurate estimation, therefore this approach is not ideal.} To overcome this challenge, we propose a new sampling scheme that reuses the subsets. \sout{We also present a strawman approach called \textit{diff-in-means}.}


% To estimate the $AME_i(\mathcal{L}^i_{\mathcal{P}})$, the most straightforward approach is sampling the subsets and compute their average marginal effects. However, this is too costly, since it requires training two models for each subset, and every source requires the same procedure, thus the models to train is at least $O(n)$. \notejinkun{UPDATED on Feb 21} \sout{What is worse, every source requires many draws to ensure accurate estimation, therefore this approach is not ideal.} To overcome this challenge, we propose a new sampling scheme that reuses the subsets. \sout{We also present a strawman approach called \textit{diff-in-means}.}

\notejinkun{The formulas in this paragraph seem a bit messy. Any suggestion for making it better?} Notice that the subset population $\mathcal{L}^i_{\mathcal{P}}$ is very similar across different source $i$. Indeed, they are all subsampling from $n-1$ sources, what remains different is only which source is not in the $n-1$ sources. This suggests a re-usability of a subset $S$ across different sources. Specifically, one single measurement of $U(S)$ can serve as either the $U(S^i+\{i\})$ of Eq.\ref{eq:amep} $\forall i \in S$ (in which $S^i=S-\{i\}$), or $U(S^i)$ $\forall i \notin S$ (in which $S^i=S$). 

To make it clear, we state the new sampling scheme as follows. Now instead of subsampling from $n-1$ sources separately for every source, we subsample from $n$ sources altogether. The inclusion probability $P$ is still drawn uniformly from the same set $\mathcal{P}$. Define $\mathcal{L}_\mathcal{P}$ as the corresponding population. %We also call this new sampling scheme $\mathcal{L}_\mathcal{P}$ and the old scheme $\mathcal{L}^i_\mathcal{P}$ when there is no ambiguity. %Assume that a subset sample $(S^{(j)})_{j=1}^m$ with size $m$ is drawn, and denote their corresponding $P$ values by $(P^{(j)})_{j=1}^m$. 


% The question remained is how to estimate correctly the $AME_i(\mathcal{L}^i_\mathcal{P})$ defined under $\mathcal{L}^i_\mathcal{P}$ using $\mathcal{L}_\mathcal{P}$. First we rewrite $AME_i$ as $\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S+\{i\})]-\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]$. It follows that 
% \begin{subequations}
% \begin{align}
% &f_{S|P}^i(s|p)=f_{S|P,i\notin S}(s|p)\\
% &f_{S|P}^i(s|p)=f_{S|P,i\in S}(s|p)
% \\
%     &\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim f_{S|P}^i(s|p)}[U(S)]]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim f(S|P=p,i\notin S)}[U(S)]|P]\\
% \end{align}
% \end{subequations}
% \begin{subequations}
% \begin{align}
%     &\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim \mathcal{L}^i(S|P=p)}[U(S+\{i\})]-\mathbb E_{S\sim \mathcal{L}^i(S|P=p)}[U(S)]|P]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim \mathcal{L}(S|P=p,i\in S)}[U(S)]-\mathbb E_{S\sim \mathcal{L}(S|P=p,i\notin S)}[U(S)]|P]\\
% \end{align}
% \end{subequations}

Next we discuss how to estimate \fixme{TODO: use other word than "estimate", since estimation is in the second next section} $AME_i$ using the new sampling scheme. Since the $AME_i$ is defined on $\mathcal{L}^i_\mathcal{P}$, we want to adjust $\mathcal{L}_\mathcal{P}$ to simulate the former distribution. First we rewrite $AME_i$ as 
\begin{equation}
    \mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)].
\end{equation}
Given $S \sim \mathcal{L}_\mathcal{P}$, we "adjust" $S$ by conditioning on $P$ and $i\notin S$ to match $S^i$:
\begin{equation}
    S^i | P \stackrel{d}{=} S | (P,i\notin S),
\end{equation}
where $\stackrel{d}{=}$ denotes equality in distribution. This is true since the $S^i$ or $S$ are both drawn according to $P$, and the only difference is that $S^i$ never includes $i$, which we fix by conditioning on $i\notin S$. Similarly:
\begin{equation}
    (S^i + \{i\}) | P \stackrel{d}{=} S | (P,i\in S),
\end{equation}
Therefore \notejinkun{Version 1}, 
\begin{subequations}
\label{eq:7}
\begin{align}
    &AME_i=\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})|P]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)|P]\right]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\in S]-\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\notin S]\right]\label{eq:diff-in-means-true},
\end{align}
\end{subequations}
Therefore \notejinkun{Version 2}, 
\begin{subequations}
\label{eq:7}
\begin{align}
    &AME_i=\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S_P\sim S^i|P}[U(S_P+\{i\})]-\mathbb E_{S_P\sim S^i|P}[U(S_P)]\right]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S_P\sim S|(P,i\in S)}[U(S_P)]-\mathbb E_{S_P\sim S|(P,i\notin S)}[U(S_P)]\right]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\in S]-\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\notin S]\right]\label{eq:diff-in-means-true},
\end{align}
\end{subequations}
\notejinkun{Which version is better? Also I may be abusing the notations here. Haven't figured out a good way to index expectation. \eg $\mathbb E_{P\sim \mathcal P}[\mathbb E_{S\sim \mathcal{L}_\mathcal{P}}[...]]$ is probably unreadable, and what I wanted to convey is that the expectation is taken over the new sampling scheme, and we do a iterated expectation on $P$, but keep in mind it is still on the new scheme (which is why I explicitly index $\mathbb E$ with $_{S\sim \mathcal{L}_\mathcal{P}}$).}%where we index expectation by ${\mathcal{L}_\mathcal{P}}$ to make it explicit that the expectation is taken over the new distribution $\mathcal{L}_\mathcal{P}$.should i write $\mathbb{E}_\mathcal{S\sim \mathcal{L}_\mathcal{P}}$ instead of $\mathbb E_{\mathcal{L}_\mathcal{P}}$ in the last line?}
% Denote by $f^i(S|P=p)$ and $f(S|P=p)$ the conditional distribution in $\mathcal{L}^i_\mathcal{P}$ and $\mathcal{L}_\mathcal{P}$ when $P=p$, respectively. Further denote by $f(S|P=p,i\in S)$ and $f(S|P=p,i\notin S)$ the conditional distribution in $\mathcal{L}_\mathcal{P}$ when $P=p$ and $i\in$ or $\notin S$. %Observe that the population $\mathcal{L}^i_\mathcal{P}$ can be induced by only taking those in $\mathcal{L}_\mathcal{P}$ that does not include $i$. Therefore $\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]$

Intuitively, Eq. \ref{eq:diff-in-means-true} calculates, for every $P$ value, the mean of $U$ when $i$ is included and that for excluded, and then average their difference across every $P$ value. 

\paragraph{Disadvantages\notejinkun{ADDED on FEB 21}}
Though being more efficient at sampling, reusing samples potentially brings high variance in the estimators when $\mathcal{P}$ includes low/high $P$, because low $P$ will have few samples of $U(S)$ with $i\in S$, and vice versa for high $P$, which would be problematic for estimating $\mathbb E_{\mathcal{L}_\mathcal{P}}[U(S)|P,i\in S]$ or $\mathbb E_{\mathcal{L}_\mathcal{P}}[U(S)|P,i\notin S]$. To mitigate this issue we recommend choosing a highly sparse grid $\mathcal{P}$, thus each $\mathcal{P}$ can have enough samples to counter the variance.\footnote{A more aggressive scheme could be, instead of sampling $P$ uniformly, sampling more for low/high $P$ and fewer for middle $P$, but it is unclear what would be the best ratio among different $P$. We leave it as future work.}

\subsection{Training Optimization -- Warm-Starting}
\label{subsec:warm-starting}
\notepanda{Isn't this an optimization for both Lasso and ``Diff in Means''?}\notejinkun{Yes, it is. So should I put it after knockoffs?}
Training of models is costly, especially for large models. Thus we further propose to use warm-starting as a proxy of original full training when there is not enough computation budget. The idea is that instead of training a model from scratch, we only fine-tune starting from the main model for some number of iterations. Moreover, we design the grid $\mathcal{P}$ specifically to only cover the lower half range (i.e. $P\leq0.5)$ based on our observations in experiments. We call this approach \textit{warm-starting} or \textit{fine-tuning} interchangeably, and refer to the original approach \textit{training-from-scratch}.

\paragraph{Justifying using only lower half range of $P$} What we find in experiments is that very low $P$s are the most helpful at distinguishing between proponents and opponents. For example, in Fig. \ref{fig:diff-in-means}, $P=0.01$ or $0.1$ work well in warm-starting. The reason is probably that low $P$s make it more likely to sample a subset without any proponent, in which adding one proponent will significantly elevate the signal $U(\cdot{})$. This does not happen in training-from-scratch probably because \sout{(a) too few data are insufficient to train a reasonable model; (b)}\notejinkun{keep or delete?} it is much easier to maintain what has been learned than learning from scratch, thus one single source is able to pull up the signal in warm-starting while not in training-from-scratch. In experiment we use $\mathcal{P}=\{0.01, 0.1, 0.2, 0.3, 0.4, 0.5\}$ and it works well. We still include up to $0.5$ to cover the case of $k=1$. In the case where there are not many sources in total we remove $0.01$ to avoid the distribution deviation problem. \notejinkun{Does this justification make sense? If not, how should we justify?}.

\paragraph{Advantages} Warm-starting generally helps the convergence, because the starting model is already converged in the whole dataset. The rest is only to transfer it into the subset, and is likely faster. Although it may not produce exactly the same result as training-from-scratch, the numbers are still comparable, suggesting that it can still be used to measure the supportive-ness and thus is a reasonable substitute for the original $U(\cdot)$. Moreover, warm-starting enables tiny $P$s. Besides the reason given in the justification above, the other reason is that the whole dataset has already been learned and we could worry less about the distribution deviation problem discussed in Sec. \ref{sec:p-pop}. \notejinkun{Probably the insufficient data problem in group testing could also be handled this way.} However, that is not to say we can never worry about that and pick extremely tiny $P$.

\paragraph{Disadvantages} On the other hand, fine-tuning cannot fully represent training-from-scratch and it is possible that some sources will have different effect between fine-tuning and training-from-scratch. The other downside is that fine-tuning generally gives a noisier signal, and may requires more observations.

\subsection{LASSO}
\label{subsec:lasso}

\subsubsection{Strawman: Diff-in-means \fixme{remove this subsubsection?}}
Directly measuring using sample means leads to the \textbf{diff-in-means} approach, which we denote by $\widehat{AME}_i$:
\begin{equation}
    \label{eq:ame-diff-in-means}
    \widehat{AME}_i=\frac{1}{b}\sum_{p\in\mathcal{P}} \widehat{\mathbb E}[U(S)|i\in S,P=p]-\widehat{\mathbb E}[U(S)|i\notin S,P=p],
\end{equation}
Note that this is also a consistent estimator, meaning that it converges in probability to $AME_i$.

\paragraph{Disadvantages}
Diff-in-means's sample efficiency is not guaranteed, especially when $n$ is large. In other words, it may not scale as $n$ increases.


\paragraph{Finite-sample error bound of diff-in-means \fixme{remove this paragraph}}
Though being simple, diff-in-means's sample efficiency is not guaranteed, especially when $n$ is large. In other words, it may require many samples and thus lots of model training to achieve accurate estimation. For example, one can use Hoeffding's inequality to give a finite-sample error bound that says with high probability, the following bounds holds:
\begin{equation}
\| \widehat{\bold{AME}} - \bold{AME} \|_p \leq O(n^\frac{1}{p} \sqrt{\frac{log(n)}{m}}), p>0,
\end{equation}
where $m$ denotes the sample size and  $\bold{AME}=(AME_1,\dots,AME_n)$, $\widehat{\bold{AME}}=(\widehat{AME}_1,\dots,\widehat{AME}_n)$. 
% \begin{equation}
%   \forall i,\| \widehat{AME_i} - AME_i \|  \leq O\left(\sqrt{\frac{n\log(n)}{m}}\right) (or something?),
% \end{equation}
However, it scales poorly as $n$ increases, and though one can do a bit better when knowing more about the random variables, the rates are basically as good as it gets in general.

\begin{proof}
Hoeffding's inequality: with probability $(1-\delta)$, for one index $i$, $|\widehat{AME}_i - AME_i| \leq \sqrt{\frac{1}{2m} \log(\frac{2}{\delta})}$. We can do a bit better when knowing more about the random variables, the the rates are basically as good as it gets in general.

We first need a union bound for it to hold over the n dimensions % (I think that's what you were mentioning in the email) 
so we use the "change of variable" $\delta \leftarrow \frac{\delta}{n}$ to account for the union bound, and get a $\sqrt{\log(n)}$ term. That gives the following bound: with probability at least $1-\delta$, $\forall i, | \widehat{AME_i} - AME_i |  \leq \sqrt{\frac{1}{2m} \log(\frac{2n}{\delta})}$.

Over all coefficients, $\| \widehat{AME_i} - AME_i\|_p \leq n^\frac{1}{p} \max_i |\widehat{AME_i} - AME_i| = O(n^\frac{1}{p} \sqrt{\frac{log(n)}{m}})$, $p>0$ \notejinkun{Mathias's original note says Cauchy-Schwartz inequality, but I don't understand. And I think this way also works, but maybe I'm wrong.}.

% When n is large, this is pretty bad. LASSO (from Theorem 1.4) gives us $O(k^\frac{1}{p} \sqrt{\frac{log(n)}{m}})$, $p \in [1, 2]$, and we are happier because the term under the root-$p$ is only $k$, and not $n$. This is especially important when $m$ is not too large (we can even have $m \leq n$ which is what LASSO is specialized for).
\end{proof}

\subsubsection{LASSO}
\notejinkun{Not confident about how to make connection between lasso and estimating AME. The paragraph below is one way that sounds more indirect, the other way may be to go from regression and then lasso. But the latter needs to state why regression is related to AME as well, which may still need a connection? I'm not sure about this connection either. The causal inference paper has some approaches using regression but not having the same form as ours. If we cite those literature, we still need to explain why our formulation is different? So I'm kind of stuck here.}
To have a better sample efficiency that scales with $n$, we start from a very different angle. Recalling that our final problem is to identify a sparse group, and this suggests a well-known variable selection technique called LASSO, which is essentially linear regression with L1 regularization. It has been proven that LASSO is very good at selecting a sparse set and recent paper \cite{lecue_regularization_2017} suggests a scalable finite-sample error bound between LASSO coefficients and the best linear approximation.

Therefore we formulate the problem into variable selection and show that in hindsight the LASSO coefficients turn out to be a consistent estimator of $AME_i$ modulo a constant factor. We utilize \cite{lecue_regularization_2017} to show that it has a better error bound of $O(k^\frac{1}{p} \sqrt{\frac{log(n)}{m}})$, $p \in [1, 2]$, suggesting that only $O(k\log n)$ of sample points are required. 

\notejinkun{version 2 of the previous two paragraphs}
To have a better sample efficiency that scales with $n$, we propose to formulate the estimation into a regression problem where the coefficients are the ones to estimate. By reducing to regression, we can utilize the rich literature on efficient estimation for regression. Among them is LASSO, which is essentially regression with L1 regularization, but is shown to be very efficient when the solution is sparse \cite{lecue_regularization_2017}: LASSO has an error bound of $O(k^\frac{1}{p} \sqrt{\frac{log(n)}{m}})$, $p \in [1, 2]$ where $m$ denotes the sample size, suggesting that only $O(k\log n)$ of sample points are required.

\paragraph{Regression formulation} We create an observation $(X,Y)$ every time a subset $S$ and the corresponding $P$ are sampled. The response variable $Y$ is assigned with value $U(S)$. There are in total $n+b$ covariates $X=(X_1,\dots,X_{n+b})$. The first $n$ are bi-value coded covariates, each indicating for each source whether it is included in $S$ or not. The specific coding will be discussed later. The remaining $b$ covariates are zero-one coded and indicate which $P$ value is chosen. Finally, $Y$ is regressed on $X$ and the coefficients of source covariates are our new estimators for $AME_i$ (modulo a constant factor).

\paragraph{Coding scheme} Our first attempt is to use the usual zero-one coding, but that brings an issue of variance weight, causing the estimator biased towards $P=0.5$. Formally, it estimates the other $AME_i$ defined as if $P$ is drawn from $\mathcal{P}$ with probability mass function $\mathbb P[P=p]=p(1-p)$. To address this issue, we use a coding scheme that assigns $X_i$ to $\frac{1}{p}$ when $i\in S$ and $\frac{-1}{1-p}$ otherwise. Besides countering the variance-weighting, it also has an important property of $E[X_i|P]=0$ that simplifies the subsequent theoretical reasoning. 

Besides adjusting coding scheme, one can also weight the observations according to $P$ when doing regression. On the other hand, this also suggests that by tuning the coding scheme/weighting of observations one can measure a different \quantity{} defined by a different distribution other than $\mathcal{L}_\mathcal{P}^i$.

%Notice that the observations can be divided into groups based on $P$ values. OLS can be interpreted as estimating $AME$ of each group and then average the results. However, OLS uses variance-weighted average that puts the most weight on the group with largest variance of $X_i$, making the estimation biased towards th. To counter this variance-weighting effect, we design an \text{inverse-propensity} coding that ensures 

\paragraph{Overall formulation}
In summary, the sampling procedure is as follows:

\begin{itemize}
\item Sample $P$, then sample subset $S$ according to $P$
\item %$Y$ to be the confidence of predicting $L$ by the model trained on the subset $S$, i.e.
Define response variable $Y=U(S)$ (note this requires model training)
\item Define covariates $X=(X_1,\dots,X_{n+b})$, with 
\begin{equation*}
    \begin{aligned}
    &X_i =\mathbf 1_{i\in S}/P-\mathbf 1_{i\notin S}/(1-P) & i \in [n]\\
    &X_{n+i} = \mathbf 1_{P=p_i} & i \in [1,b],
    \end{aligned}
\end{equation*}
where $\mathbf 1_{cond}$ is the indicator function evaluates to $1$ when $cond$ is true and $0$ otherwise.
\end{itemize}
Assume we have sampled $m$ subsets, then we can generate corresponding $m$ observations $(X^{(j)}, Y^{(j)})_{j=1}^m$. We can thus feed them into an OLS model and derive the OLS estimators:
\begin{equation}
     \label{eq:ols}\hat{l}_{ols}\in\underset{l \in \mathbb{R}^{n+b}}{\argmin} \frac{1}{m} \sum_{j=1}^{m}\left(Y^{(j)}-\left\langle l, X^{(j)}\right\rangle\right)^{2},
\end{equation}
where $\langle\cdot,\cdot\rangle$ denotes inner product. Finally we add L1 regularization and that gives the LASSO estimators
\begin{equation}
     \label{eq:lasso}\hat{l}_{lasso}\in\underset{l \in \mathbb{R}^{n+b}}{\argmin} \left(\frac{1}{m} \sum_{j=1}^{m}\left(Y^{(j)}-\left\langle l, X^{(j)}\right\rangle\right)^{2}+\lambda \|l_{1:n}\|_{1}\right),
\end{equation}
where $l_{1:n}=(l_1,\dots,l_n)$ and $\lambda>0$ is a hyper-parameter typically chosen through cross-validation. 
\paragraph{Consistency and Finite-sample error bound of $\hat l_{lasso}$}
We will show that for some constant $c_1$, $\|\hat{l}_{lasso,1:n}-\bold{AME}/c_1\|_p \leq O((k)^\frac{1}{p} \sqrt{\frac{log(n)}{m}})$ with high probability. We first proof that the best linear approximation $l^*$ equals $\bold{AME}/c_1$, and then proof that $\hat l_{lasso}$ is close to $l^*$ in large sample with high probability.

\begin{proposition}
Let $l^*$ be the best linear approximation, i.e.
\begin{equation}\label{eq:best}l^{*}\in\underset{l \in \mathbb{R}^{n+b}}{\argmin}~ \mathbb{E}\left[(Y-\left\langle l, X\right\rangle)^{2}\right],\end{equation}
then $AME_i/c_1=l^*_i, \forall i\in[n]$, where $c_1=Var[X]=\mathbb{E}[\frac{1}{P(1-P)}|P]$. 
\end{proposition}
\begin{proof}
By REGRESSION ANATOMY introduced in Equation 3.1.3 of \cite{angrist2008mostly}, \begin{equation}l^*_i=\frac{Cov(Y,\tilde X_i)}{Var[\tilde X_i]},\end{equation} where $\tilde X_i$ is the regression residual of $X_i$ on all the other covariates $X_{-i}=(X_1,\dots,X_{i-1}, X_{i+1},\dots, X_{n+b}).$ Since $\mathbb E[X_i|X_{-i}]=\mathbb E[X_i|P]=0$ is a linear function, $\tilde X_i=X_i-\mathbb E[X_i|X_{-i}]=X_i.$ Therefore,
\begin{equation*}
    l^*_i=\frac{Cov(Y,\tilde X_i)}{Var[\tilde X_i]}=\frac{Cov(Y,X_i)}{Var[X_i]}=\frac{\mathbb E[X_iY]}{Var[X_i]}
\end{equation*}
It follows that 
\begin{equation*}
\begin{aligned}
\label{eq:diy}
&\mathbb E[X_iY|P=p]\\
={}&\sum_{t=0}^1\mathbb P[\mathbf 1_{i\in S}=t|P=p]\cdot\mathbb E[X_iY|\mathbf 1_{i\in S}=t,P=p]\\
={}&p\cdot\mathbb E[X_iY|P=p,  i\in S]+(1-p)\cdot\mathbb E[X_iY|P=p,  i\notin S]\\
={}&p\frac{1}{p} \mathbb E[Y|P=p,i\in S]+(1-p)\frac{-1}{1-p}\mathbb E[Y|P=p,i\notin S]\\
={}&\mathbb E[Y|P=p,i\in S]-\mathbb E[Y|P=p,i\notin S]
\end{aligned}
\end{equation*}
Thus 
\begin{equation*}
\begin{aligned}
\label{eq:diy}
l^*_i&=\frac{\mathbb E[X_iY]}{Var[X_i]}=\frac{\mathbb E_{P\sim \mathcal{P}}[\mathbb E[X_iY|P]]}{Var[X]}\\
&=\frac{\mathbb E_{P\sim \mathcal{P}}[\mathbb E[Y|P,i\in S]-\mathbb E[Y|P,i\notin S]]}{Var[X]}\\
&=\frac{AME_i}{Var[X]}  ~~ (\text{by Eq. \ref{eq:7}})
\end{aligned}
\end{equation*}
Finally, 
\begin{equation*}
    Var[X]=\mathbb E[Var[X|P]]+Var[\mathbb E[X|P]]=\mathbb E[\frac{1}{P(1-P)}|P]
\end{equation*}
\end{proof}
\begin{proposition}
With high probability $\|\hat{l}_{lasso}-l^*\|_p\leq O(k^\frac{1}{p} \sqrt{\frac{\log(n)}{m}})$, $p \in [1, 2]$.
\end{proposition}
\begin{proof}
TBD \notejinkun{This is where we should use the small ball paper. But I remember there is a problem with unpenalized bucket variables.}
\end{proof}
\begin{corollary}
With high probability $\|\hat{l}_{lasso,1:n}-\bold{AME}/c_1\|_p\leq O(k^\frac{1}{p} \sqrt{\frac{\log(n)}{m}})$, $p \in [1, 2], c_1=Var[X]$.
\end{corollary}


% On the one hand, the $AME_i$ is a well known concept termed \textit{Average Treatment Effect} in the field of causal inference and sometimes estimated through regression \cite{imbens_causal_2015, egami_causal_2019} \footnote{diff-in-means gives the same result as regression and sometimes people favor regression given its popularity, cf. Chapter 7 of \cite{imbens_causal_2015}.}. On the other hand, LASSO is often used together with regression when people want to select a sparse set of covariates. Moreover, recent paper \cite{lecue_regularization_2017} suggests that LASSO guarantees a good finite-sample error bound. Note that there are also works in causal inference using LASSO, but they do it in a slightly different way, making it hard to utilizing the finite-sample error bound. Therefore, we propose a novel formulation of regression with    with LASSO for estimation as well as proponent group selection.
% , though most of them are focused on measuring for one single treatment (i.e. source in our case) \fixme{CITE}. There are works for multiple treatments, but  or mak

\subsection{Precision-Controlled Selection -- Knockoffs}
\label{subsec:knockoffs}
Given estimates of $AME_i$ measured through either LASSO or diff-in-means, we choose a threshold $t$ and select those sources as the proponent group with an estimate $\geq t$. Without the loss of generality, we assume the estimate is measure through LASSO. The choice of $t$ is critical to the quality of selection and must be chosen carefully.
%Moreover, users may have different preference for the selection: some may favor a power selection that selects more proponents, while some may favor a conservative selection that selects the proponents more accurately. 
Define \textit{precision} and \textit{recall} to quantify the selection as 
\begin{equation*}
\begin{aligned}
    &precision(t)&=\frac{\#\{\text{proponent } i: \hat{l}_{lasso,i }>t\}}{\#\{i: \hat{l}_{lasso,i}>t\}}\\
    &recall(t)&=\frac{\#\{\text{proponent } i: \hat{l}_{lasso,i}>t\}}{\#\{\text{proponent } i\}}
\end{aligned}
\end{equation*}
with $precision(t)=1$ when its denominator is 0. We also define false discovery rate (FDR) as 
\begin{equation*}
    FDR(t)=1-precision(t)
\end{equation*}
%Thus a power selection corresponds to high recall and conservative corresponds to high precision.

We apply a framework called Knockoffs \cite{candes_panning_2017} in choosing $t$. Knockoffs can bound the expected precision to be at least a given value. This offers some form of guarantee of the selection quality, and also gives users flexibility to choose $t$ based on their precision requirement.

Specifically, when running the subset sampling and LASSO, we assume there are $2n$ sources with the first $n$ being original sources and last $n$ being "fake" ones that contains no data. Let's term the covariates of the original sources $D=(D_1,\dots,D_n)$ and covariates of the fake ones $\tilde{D}=(\tilde D_1, \dots,\tilde D_n)$. The goal is to create variables (i.e. $\tilde{D}$) that we know for sure are independent of $Y$ and thus should not be selected. This serves as a reference for further reasoning about which original sources should not be selected. %the same distribution as $D_i$ for $i=0,\ldots,n-1$. 

Next, given a target FDR level $q$, we pick a threshold $\tau$ by setting\footnote{Per footnote of \cite{candes_panning_2017}: $\min \{t > 0 : \dots\}$ actually means $\min \{t \in W_+ : \dots \}$, where $W_+ = \{|W_i| : |W_i| > 0\}$}
\begin{equation}
\tau=\min \left\{t>0: \frac{\#\left\{i: W_{i} \leq-t\right\}}{\#\left\{i: W_{i} \geq t\right\}} \leq q\right\},
\end{equation}
where $W_i=\max(\hat l_i,0)$. The intuition behind doing the "relu" operation (i.e. $\max(\cdot,0)$)  on $\hat l_i$ is to only select the proponent group. $\tau=+\infty$ if the set above is empty. Finally, the procedure selects the sources
\begin{equation*}
    \hat S_+=\{i:W_i\geq \tau\}
\end{equation*}

\begin{proposition}
Assume that $AME_i=0$ for any source $i$ that is neither proponent or opponent. Then the above threshold controls a modified FDR defined as
\begin{equation}
\label{eq:mFDR}
mFDR=\mathbb{E}\left[\frac{\left|\left\{j \in (\hat{S}_+ - S_+) \right\}\right|}{|\hat{S}_+|+1 / q}\right] \leq q,
\end{equation}
where $S_+$ denotes the true proponent group.
\end{proposition}
%Now we claim $\tilde D$ is the Knockoffs of $D$. 
\begin{proof}
TBD \notejinkun{probably this proposition is wrong...}
% For this to be true, according to the Knockoff paper\cite{candes_panning_2017}, 2 properties must be satisfied: \textit{(1) for any subset $S \subset\{0, \ldots, n-1\}$,
% $$
% (D, \tilde{D})_{\operatorname{swap}(S)} \stackrel{d}{=}(D, \tilde{D})
% $$
% (2) $\tilde{D} \perp Y | D$  if there is a response  $Y$.}

% Above, the vector $(D, \tilde{D})_{\operatorname{swap}(S)}$ is obtained from $(D, \tilde D)$ by swapping the entries $D_j$ and  $\tilde D_j$ for each
% $j \in S$. (1) is guaranteed since each $D_i$ and $\tilde D_i$ are independently assigned. (2) is also guaranteed since $\tilde D$ constructed without looking at $Y$. Therefore, $\tilde D$ is the knockoffs of $D$.
\end{proof}
Overall, the pseudo code of LASSO+Knockoffs is shown in Algo. \ref{algo:k1} and Algo. \ref{algo:k2}.

\fixme{TODO: discuss plus version?}

\begin{algorithm}[h]
\DontPrintSemicolon
% \KwResult{Write here the result }
\SetKwFunction{FtrainOnComb}{trainOnComb}
\SetKwFunction{Ftrain}{train}
\SetKwFunction{FLASSO}{LASSO}
\SetKwFunction{Fselect}{select}
 \KwIn{$n$, number of data sources}
 \KwIn{$m$, number of models (or observations for the analysis)}
 \KwIn{$\mathcal P=\{p_1,\dots,p_b\}$, probabilities to include data source. Default $\{0.2, 0.4, 0.6, 0.8\}$}
 \KwIn{$L$, query label}
 \KwIn{$I$, query input}
 $[\mathbf{D}, \mathbf{\tilde D}] \gets [zeros(m,n), zeros(m,n)]$\tcp*[r]{init the design matrices, where $\mathbf{\tilde D}$ is knockoff}
 $\mathbf{B} \gets zeros(m,n)$\;
 $Y\gets zeros(m)$\tcp*[r]{Outcome vector init}
 \For{$i\gets1$ \KwTo $m$ }{
   $r \sim UniformInt(1,b)$\;
   $\mathbf{B}[i,r]\gets 1$\;
  \For{$j\gets1$ \KwTo $n$ }{
   $r_1 \sim Bernoulli(p_r)$\;%\tcp*[r]{$r_1$ is either 0 or 1. 1 means source is included}
   $r_2 \sim Bernoulli(p_r)$\tcp*[r]{for knockoffs}
%   $\mathbf{C}[i,j],\mathbf{\tilde C}[i,j] \gets r_1, r_2$\; 
   $\mathbf{D}[i,j],\mathbf{\tilde D}[i,j] \gets \frac{r_1}{p_r}-\frac{1-r_1}{1-p_r}, \frac{r_2}{p_r}-\frac{1-r_2}{1-p_r}$\; 
   }
  $\mathcal{M}_i \gets \FtrainOnComb(\mathbf{D}[i,:])$\;%\tcp*[r]{train model on combination $\mathbf{D}[i,:]$}
  $Y[i]\gets \mathcal{M}_i(I)[L]$\tcp*[r]{obtain confidence}
 }
 $\mathbf{X}\gets [\mathbf D,\mathbf{\tilde D},\mathbf{B}]$\tcp*[r]{concat through columns to get final design matrix}
 \KwRet{$\hat l\gets$ \FLASSO{$\mathbf{X},Y,\lambda$}}\tcp*[r]{run LASSO with the $\lambda$ chosen by cross validation.}
%  \KwRet{\Fselect{$\hat l,q$}}\;
 \;
%  \Fn(\tcp*[f]{train on 1 combination \textbf C}){\FtrainOnComb{$\mathbf D$}}{
 \Fn(){\FtrainOnComb{$\mathbf D$}}{
%  \KwIn{$\mathbf D$, an array of size $n$ made up of 0 and 1}
  $S \gets \{\}$\tcp*[r]{training set for this model}
  \For{$j\gets1$ \KwTo $n$}{
   \lIf{$\mathbf D[j] > 0$}{$S\gets S+\{j\}$}
  }
  \KwRet{\Ftrain{S}}\tcp*[r]{train from scratch or fine-tune on $S$}
 }
 \caption{Obtaining LASSO coefficients\label{algo:k1}}
\end{algorithm}

\begin{algorithm}[h]
\DontPrintSemicolon
\SetKwFunction{Fselect}{select}
%  \Fn(\tcp*[f]{select non-null features with FDR under control}){\Fselect{$\hat l, q$}}{
  \KwIn{$\hat l$, the LASSO coef of size $2n$}
  \KwIn{$q$, the target FDR level}
  $W \gets zeros(n)$\tcp*[r]{statistics}
  \For{$i\gets1$ \KwTo $n$}{
   $W_i=relu(\hat l_i)-relu(\hat l_{i+n})$\;
  }
  $\tau \gets \min \left\{t>0: \frac{\#\left\{i:W_{i} \leq-t\right\}}{\#\left\{i:W_{i} \geq t\right\}} \leq q\right\}$\tcp*[r]{find the threshold given the desired FDR}
  $\hat S_+ \gets \{\}$\;%\tcp*[r]{non-null features (or data sources) indices}
  \For{$i\gets1$ \KwTo $n$}{
   \lIf{$W_i\geq\tau$}{$\hat S_+\gets \hat S_++\{i\}$}
  }
  \KwRet{$R$}
%  }
 \caption{FDR-controlled feature selection\label{algo:k2}}
\end{algorithm}


==> rm/approach-v2.tex <==
\section{The Sampling, Training, Estimation and Selection Procedure}
\label{sec: procedure}
\sid{This is our main design section and so should be titled "[system name] methodology" or something like that.}

\notepanda{Some of this seems to repeat/be out of order with the previous section. For instance \S\ref{subsec:sampling} seems to assume no Lasso, but we introduced this earlier.}

% To identify the proponent group there are four problems we need to solve: (1) we need an efficient subset sampling scheme (\S\ref{subsec:sampling}); (2) we need to train models on these sampled subsets efficiently (\S\ref{subsec:warm-starting}); (3) we need to estimate the quantities accurately using the training results (\S\ref{subsec:lasso}); (4) we need an accurate while powerful procedure for selecting sources using the estimates (\S\ref{subsec:knockoffs}). Doing them naively is either too costly or inaccurate. In the following 4 sections we describe the underlying challenges for each component and how we overcome them respectively.
The problem of identifying the proponent group is thus divided into four steps: (1) subsample subsets (\S\ref{subsec:sampling}); (2) train models on these sampled subsets (\S\ref{subsec:warm-starting}); (3) estimate the \quantity{} using the training results (\S\ref{subsec:lasso}); (4) select sources based on the estimates (\S\ref{subsec:knockoffs}). Doing them naively is either too costly or inaccurate. In the following 4 sections we describe the underlying challenges for each component and how we overcome them respectively.

\subsection{The Sampling Scheme}
\label{subsec:sampling}

\notejinkun{this whole section is just to (i) stating that we want to sample the subsets altogether (\ie reusing subsets for estimating each source; (ii) and showing why this can be still estimating the same thing (\ie by showing the expectation of difference (\eqref{eq:amep}) equals difference of expectation (\eqref{eq:diff-in-means-true}. btw sorry that I pointed to a wrong place during the meeting). Don't hesitate to ping me if you feel confused (which is probably my bad of writing or the argument is truly incorrect)!}

\notepanda{Is this really a viable option? This section read a bit like us beating up on a strawman that obviously would not work: just say it is costly and move on?}

To estimate the $AME_i(\mathcal{L}^i_{\mathcal{P}})$,the most straightforward approach is sampling the subsets and compute their average marginal effects. However, this is too costly, since it requires training two models for each subset, and every source requires the same procedure, thus the models to train is at least $O(n)$. \notejinkun{UPDATED on Feb 21} \sout{What is worse, every source requires many draws to ensure accurate estimation, therefore this approach is not ideal.} To overcome this challenge, we propose a new sampling scheme that reuses the subsets. \sout{We also present a strawman approach called \emph{diff-in-means}.}


% To estimate the $AME_i(\mathcal{L}^i_{\mathcal{P}})$, the most straightforward approach is sampling the subsets and compute their average marginal effects. However, this is too costly, since it requires training two models for each subset, and every source requires the same procedure, thus the models to train is at least $O(n)$. \notejinkun{UPDATED on Feb 21} \sout{What is worse, every source requires many draws to ensure accurate estimation, therefore this approach is not ideal.} To overcome this challenge, we propose a new sampling scheme that reuses the subsets. \sout{We also present a strawman approach called \emph{diff-in-means}.}

\notejinkun{The formulas in this paragraph seem a bit messy. Any suggestion for making it better?} Notice that the subset population $\mathcal{L}^i_{\mathcal{P}}$ is very similar across different source $i$. Indeed, they are all subsampling from $n-1$ sources, what remains different is only which source is not in the $n-1$ sources. This suggests a re-usability of a subset $S$ across different sources. Specifically, one single measurement of $U(S)$ can serve as either the $U(S^i+\{i\})$ of Eq. \ref{eq:amep} $\forall i \in S$ (in which $S^i=S-\{i\}$), or $U(S^i)$ $\forall i \notin S$ (in which $S^i=S$). 

To make it clear, we state the new sampling scheme as follows. Now instead of subsampling from $n-1$ sources separately for every source, we subsample from $n$ sources altogether. The inclusion probability $P$ is still drawn uniformly from the same set $\mathcal{P}$. Define $\mathcal{L}_\mathcal{P}$ as the corresponding population. Notice that this new sampling distribution is slightly different from the original one defining $AME$, and thus some further adjustment is needed to ensure correct, unbiased estimation. We detail the adjustment procedure in the section of estimation \S \ref{subsec:lasso}. %We also call this new sampling scheme $\mathcal{L}_\mathcal{P}$ and the old scheme $\mathcal{L}^i_\mathcal{P}$ when there is no ambiguity. %Assume that a subset sample $(S^{(j)})_{j=1}^m$ with size $m$ is drawn, and denote their corresponding $P$ values by $(P^{(j)})_{j=1}^m$. 


% The question remained is how to estimate correctly the $AME_i(\mathcal{L}^i_\mathcal{P})$ defined under $\mathcal{L}^i_\mathcal{P}$ using $\mathcal{L}_\mathcal{P}$. First we rewrite $AME_i$ as $\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S+\{i\})]-\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]$. It follows that 
% \begin{subequations}
% \begin{align}
% &f_{S|P}^i(s|p)=f_{S|P,i\notin S}(s|p)\\
% &f_{S|P}^i(s|p)=f_{S|P,i\in S}(s|p)
% \\
%     &\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim f_{S|P}^i(s|p)}[U(S)]]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim f(S|P=p,i\notin S)}[U(S)]|P]\\
% \end{align}
% \end{subequations}
% \begin{subequations}
% \begin{align}
%     &\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim \mathcal{L}^i(S|P=p)}[U(S+\{i\})]-\mathbb E_{S\sim \mathcal{L}^i(S|P=p)}[U(S)]|P]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim \mathcal{L}(S|P=p,i\in S)}[U(S)]-\mathbb E_{S\sim \mathcal{L}(S|P=p,i\notin S)}[U(S)]|P]\\
% \end{align}
% \end{subequations}


\paragraph{Disadvantages}
Though being more efficient at sampling, reusing samples potentially brings high variance in the estimators when $\mathcal{P}$ includes low/high $P$, because low $P$ will have few samples of $U(S)$ with $i\in S$, and vice versa for high $P$, which would be problematic for estimating $\mathbb E[U(S^i+\{i\}) - U(S^i) | P]$ accurately under low/high $P$. To mitigate this issue we recommend choosing a highly sparse grid $\mathcal{P}$, thus each $\mathcal{P}$ can have enough samples to counter the variance.\footnote{A more aggressive scheme could be, instead of sampling $P$ uniformly, sampling more for low/high $P$ and fewer for middle $P$, but it is unclear what would be the best ratio among different $P$. We leave it as future work.}

\subsection{Estimation -- Diff-in-Means and LASSO}
\label{subsec:lasso}
After a set of subsets are drawn, we train one model on every subset $S$ and use it to predict on the query input to obtain $U(S)$, which will be later used by the estimation procedure detailed in this section.

\subsubsection{Strawman: Diff-in-means \fixme{remove this subsubsection?}}
By linearity of expectation, $AME_i$ can be re-written as 
\begin{equation}
    \mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)].
\end{equation}
A natural approach is then to estimate the two expectations separately by computing some means on the subsets drawn. Since our new sampling distribution is different from the original one defining $AME_i$, some \emph{adjustment} of the sample is needed to ensure consistency. To do so, if we denote by $S, S^i$ the random subset variable in the new and original distribution, respectively, we can adjust $S$ to be like $S^i$ by conditioning on $P$ and $i\notin S$:
\begin{equation}
    S^i | P \stackrel{d}{=} S | (P,i\notin S),
\end{equation}
where $\stackrel{d}{=}$ denotes equality in distribution. This is true since the $S^i$ or $S$ are both drawn according to $P$, and the only difference is that $S^i$ never includes $i$, which we fix by conditioning on $i\notin S$. Similarly:
\begin{equation}
    (S^i + \{i\}) | P \stackrel{d}{=} S | (P,i\in S),
\end{equation}
Therefore \notejinkun{Version 1}, 
\begin{subequations}
\label{eq:7}
\begin{align}
    &AME_i=\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})|P]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)|P]\right]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\in S]-\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\notin S]\right]\label{eq:diff-in-means-true},
\end{align}
\end{subequations}
Therefore \notejinkun{Version 2}, 
\begin{subequations}
\label{eq:7}
\begin{align}
    &AME_i=\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S_P\sim S^i|P}[U(S_P+\{i\})]-\mathbb E_{S_P\sim S^i|P}[U(S_P)]\right]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S_P\sim S|(P,i\in S)}[U(S_P)]-\mathbb E_{S_P\sim S|(P,i\notin S)}[U(S_P)]\right]\\
    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\in S]-\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\notin S]\right]\label{eq:diff-in-means-true},
\end{align}
\end{subequations}
\notejinkun{Which version is better? Also I may be abusing the notations here. Haven't figured out a good way to index expectation. \eg $\mathbb E_{P\sim \mathcal P}[\mathbb E_{S\sim \mathcal{L}_\mathcal{P}}[...]]$ is probably unreadable, and what I wanted to convey is that the expectation is taken over the new sampling scheme, and we do a iterated expectation on $P$, but keep in mind it is still on the new scheme (which is why I explicitly index $\mathbb E$ with $_{S\sim \mathcal{L}_\mathcal{P}}$).}%where we index expectation by ${\mathcal{L}_\mathcal{P}}$ to make it explicit that the expectation is taken over the new distribution $\mathcal{L}_\mathcal{P}$.should i write $\mathbb{E}_\mathcal{S\sim \mathcal{L}_\mathcal{P}}$ instead of $\mathbb E_{\mathcal{L}_\mathcal{P}}$ in the last line?}
% Denote by $f^i(S|P=p)$ and $f(S|P=p)$ the conditional distribution in $\mathcal{L}^i_\mathcal{P}$ and $\mathcal{L}_\mathcal{P}$ when $P=p$, respectively. Further denote by $f(S|P=p,i\in S)$ and $f(S|P=p,i\notin S)$ the conditional distribution in $\mathcal{L}_\mathcal{P}$ when $P=p$ and $i\in$ or $\notin S$. %Observe that the population $\mathcal{L}^i_\mathcal{P}$ can be induced by only taking those in $\mathcal{L}_\mathcal{P}$ that does not include $i$. Therefore $\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]$

Intuitively, Eq. \ref{eq:diff-in-means-true} calculates, for every $P$ value, the mean of $U$ when $i$ is included and $U$ when excluded, and then average their difference across every $P$ value. 

Directly measuring using sample means leads to the \textbf{diff-in-means} approach, which we denote by $\widehat{AME}_i$:
\begin{equation}
    \label{eq:ame-diff-in-means}
    \widehat{AME}_i=\frac{1}{b}\sum_{p\in\mathcal{P}} \widehat{\mathbb E}[U(S)|i\in S,P=p]-\widehat{\mathbb E}[U(S)|i\notin S,P=p],
\end{equation}

\paragraph{Disadvantages}
\fixme{question: \notejinkun{how to frame this properly?}}Diff-in-means has not yet been proved to be sample efficienc when $n$ is large. In other words, it may not scale as $n$ increases.



\subsubsection{LASSO}
\notejinkun{Not confident about how to make connection between lasso and estimating AME. The paragraph below is one way that sounds more indirect, the other way may be to go from regression and then lasso. But the latter needs to state why regression is related to AME as well, which may still need a connection? I'm not sure about this connection either. The causal inference paper has some approaches using regression but not having the same form as ours. If we cite those literature, we still need to explain why our formulation is different? So I'm kind of stuck here.}
\sid{This version feels more intuitive to me than the second version.}
To have a better sample efficiency that scales with $n$, we start from a very different angle. Recalling that our final problem is to identify a sparse group, and this suggests a well-known variable selection technique called LASSO, which is essentially linear regression with L1 regularization. It has been proven that LASSO is very good at selecting a sparse set and recent paper \cite{lecue_regularization_2017} suggests a scalable finite-sample error bound between LASSO coefficients and the best linear approximation.

Therefore we formulate the problem into variable selection and show that in hindsight the LASSO coefficients turn out to be a consistent estimator of $AME_i$ modulo a constant factor. We utilize \cite{lecue_regularization_2017} to show that it has a better error bound of $O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2]$, suggesting that only $O(k\log n)$ of sample points are required. 

\notejinkun{version 2 of the previous two paragraphs}
To have a better sample efficiency that scales with $n$, we propose to formulate the estimation into a regression problem where every $AME_i$ corresponds to one of the coefficients, and now estimating the $AME_i$s is equivalent to estimating the coefficients. By reducing to regression, we can utilize the rich literature on efficient estimation for regression. Among them is LASSO, which is essentially regression with L1 regularization, but is shown to be very efficient when the solution is sparse \cite{lecue_regularization_2017}: LASSO has a scalable error bound of $O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2]$ where $m$ denotes the sample size, suggesting that only $O(k\log n)$ of sample points are required.

\sid{The regression formulation below is a core contribution and needs to be elevated as such. We should add a figure/picture showing the design matrix itself.}
\paragraph{Regression formulation} We create an observation $(X,Y)$ every time a subset $S$ and the corresponding $P$ are sampled. The response variable $Y$ is assigned with value $U(S)$. There are in total $n+b$ covariates, denoted by $X=(X_1,\dots,X_{n+b})$. The first $n$ are source covariates and bi-valuedly coded, each indicating for each source whether it is included in $S$ or not. The specific coding will be discussed later. The remaining $b$ are bucket covariates and zero-one coded, indicate which $P$ value is chosen. Finally, $Y$ is regressed on $X$ and the coefficient estimates of source covariates are our new estimators for $AME_i$ (modulo a constant factor $c_1=\mathbb E[\frac{1}{P(1-P)}]$).

\sid{I would pitch the coding scheme issue below as a (non-major) technical challenge.}
\paragraph{Coding scheme} Our first attempt is to use the usual zero-one coding, but that brings an issue of variance weighting, causing the estimator biased towards $P=0.5$. Formally, it estimates the other $AME_i$ defined as if $P$ is drawn from $\mathcal{P}$ with probability mass function $\mathbb P[P=p]=p(1-p)$. To address this issue, we use a coding scheme that assigns $X_i$ to $\frac{1}{p}$ when $i\in S$ and $\frac{-1}{1-p}$ otherwise. Besides countering the variance-weighting, it also has an important property of $\mathbb E[X_i|P]=0$ that simplifies the subsequent theoretical reasoning. 

Besides adjusting coding scheme, one can also weight the observations according to $P$ when doing regression. On the other hand, this also suggests that by tuning the coding scheme/weighting of observations one can measure a different \quantity{} defined by a different distribution other than $\mathcal{L}_\mathcal{P}^i$.

%Notice that the observations can be divided into groups based on $P$ values. OLS can be interpreted as estimating $AME$ of each group and then average the results. However, OLS uses variance-weighted average that puts the most weight on the group with largest variance of $X_i$, making the estimation biased towards th. To counter this variance-weighting effect, we design an \text{inverse-propensity} coding that ensures 

\paragraph{Overall formulation}
In summary, the sampling procedure is as follows:

\begin{itemize}
\item Sample $P$, then sample subset $S$ according to $P$
\item %$Y$ to be the confidence of predicting $L$ by the model trained on the subset $S$, i.e.
Define response variable $Y=U(S)$
\item Define covariates $X=(X_1,\dots,X_{n+b})$, with 
\begin{equation*}
    \begin{aligned}
    &X_i =\mathbf 1_{i\in S}/P-\mathbf 1_{i\notin S}/(1-P) & i \in [n]\\
    &X_{n+i} = \mathbf 1_{P=p_i} & i \in [1,b],
    \end{aligned}
\end{equation*}
where $\mathbf 1_{cond}$ is the indicator function evaluates to $1$ when $cond$ is true and $0$ otherwise.
\end{itemize}
\sid{Do we explain the $X_{n+i}$ variables anywhere?}\notejinkun{Yes we said "The  remaining $b$ are  bucket  covariates  and  zero-onecoded", but we didn't explain why we want it in the current version.}

Assume we have sampled \sid{What do we mean by "sampled" here? The term is overloaded so we should be a careful.} $m$ subsets, then we can generate corresponding $m$ observations $(X^{(j)}, Y^{(j)})_{j=1}^m$. We can thus feed them into an OLS model and derive the OLS estimators:
\begin{equation}
     \label{eq:ols}\hat{l}_{ols}\in\underset{l \in \mathbb{R}^{n+b}}{\argmin} \frac{1}{m} \sum_{j=1}^{m}\left(Y^{(j)}-\left\langle l, X^{(j)}\right\rangle\right)^{2},
\end{equation}
where $\langle\cdot,\cdot\rangle$ denotes inner product. Finally we add L1 regularization and that gives the LASSO estimators
\begin{equation}
     \label{eq:lasso}\hat{l}_{lasso}\in\underset{l \in \mathbb{R}^{n+b}}{\argmin} \left(\frac{1}{m} \sum_{j=1}^{m}\left(Y^{(j)}-\left\langle l, X^{(j)}\right\rangle\right)^{2}+\lambda \|l_{1:n}\|_{1}\right),
\end{equation}
where $l_{1:n}=(l_1,\dots,l_n)$ and $\lambda>0$ is a hyper-parameter chosen through cross-validation. 
% \paragraph{Consistency and Finite-sample error bound of $\hat l_{lasso}$}
\paragraph{Equivalence between AME estimation and regression, and the finite-sample error bound of $\hat l_{lasso}$ estimators}
We will show that for some constant $c_1$, $\|\hat{l}_{lasso,1:n}-\bold{AME}/c_1\|_p \leq O(k^\frac{1}{p} \sqrt{\log(n)/m})$ with high probability. \notejinkun{Not sure if this is precise?} We first proof that our regression formulation has the true solution $l^*$ equal to $\bold{AME}/c_1$ under infinite sample, and then proof that $\hat l_{lasso}$ is close to $l^*$ in large sample with high probability.

\begin{proposition}
Let $l^*$ be the best linear approximation, i.e.
\begin{equation}\label{eq:best}l^{*}\in\underset{l \in \mathbb{R}^{n+b}}{\argmin}~ \mathbb{E}\left[(Y-\left\langle l, X\right\rangle)^{2}\right],\end{equation}
then $AME_i/c_1=l^*_i, \forall i\in[n]$, where $c_1=Var[X_i]=\mathbb{E}[\frac{1}{P(1-P)}]$. 
\end{proposition}
\begin{proof}
By REGRESSION ANATOMY introduced in Equation 3.1.3 of \cite{angrist2008mostly}, \begin{equation}l^*_i=\frac{Cov(Y,\tilde X_i)}{Var[\tilde X_i]},\end{equation} where $\tilde X_i$ is the regression residual of $X_i$ on all the other covariates $X_{-i}=(X_1,\dots,X_{i-1}, X_{i+1},\dots, X_{n+b}).$ Since $\mathbb E[X_i|X_{-i}]=\mathbb E[X_i|P]=0$ is a linear function, $\tilde X_i=X_i-\mathbb E[X_i|X_{-i}]=X_i.$ Therefore,
\begin{equation*}
    l^*_i=\frac{Cov(Y,\tilde X_i)}{Var[\tilde X_i]}=\frac{Cov(Y,X_i)}{Var[X_i]}=\frac{\mathbb E[X_iY]}{Var[X_i]}
\end{equation*}
It follows that 
\begin{equation*}
\begin{aligned}
\label{eq:diy}
&\mathbb E[X_iY|P=p]\\
={}&\sum_{t=0}^1\mathbb P[\mathbf 1_{i\in S}=t|P=p]\cdot\mathbb E[X_iY|\mathbf 1_{i\in S}=t,P=p]\\
={}&p\cdot\mathbb E[X_iY|P=p,  i\in S]+(1-p)\cdot\mathbb E[X_iY|P=p,  i\notin S]\\
={}&p\frac{1}{p} \mathbb E[Y|P=p,i\in S]+(1-p)\frac{-1}{1-p}\mathbb E[Y|P=p,i\notin S]\\
={}&\mathbb E[Y|P=p,i\in S]-\mathbb E[Y|P=p,i\notin S]
\end{aligned}
\end{equation*}
Thus 
\begin{equation*}
\begin{aligned}
\label{eq:diy}
l^*_i&=\frac{\mathbb E[X_iY]}{Var[X_i]}=\frac{\mathbb E_{P\sim \mathcal{P}}[\mathbb E[X_iY|P]]}{Var[X_i]}\\
&=\frac{\mathbb E_{P\sim \mathcal{P}}[\mathbb E[Y|P,i\in S]-\mathbb E[Y|P,i\notin S]]}{Var[X_i]}\\
&=\frac{AME_i}{Var[X_i]}  ~~ (\text{by Eq. \ref{eq:7}})
\end{aligned}
\end{equation*}
Finally, 
\begin{equation*}
    Var[X_i]=\mathbb E[Var[X_i|P]]+Var[\mathbb E[X_i|P]]=\mathbb E[\frac{1}{P(1-P)}]
\end{equation*}
\end{proof}
\begin{proposition}
With high probability $\|\hat{l}_{lasso}-l^*\|_p\leq O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2]$.
\end{proposition}
\begin{proof}
TBD \notejinkun{This is where we should use the small ball paper. But I remember there is a problem with unpenalized bucket variables.}
\end{proof}
\begin{corollary}
With high probability $\|\hat{l}_{lasso,1:n}-\bold{AME}/c_1\|_p\leq O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2], c_1=Var[X_1]=\dots =Var[X_n]=\mathbb E[\frac{1}{P(1-P)}]$.
\end{corollary}


% On the one hand, the $AME_i$ is a well known concept termed \emph{Average Treatment Effect} in the field of causal inference and sometimes estimated through regression \cite{imbens_causal_2015, egami_causal_2019} \footnote{diff-in-means gives the same result as regression and sometimes people favor regression given its popularity, cf. Chapter 7 of \cite{imbens_causal_2015}.}. On the other hand, LASSO is often used together with regression when people want to select a sparse set of covariates. Moreover, recent paper \cite{lecue_regularization_2017} suggests that LASSO guarantees a good finite-sample error bound. Note that there are also works in causal inference using LASSO, but they do it in a slightly different way, making it hard to utilizing the finite-sample error bound. Therefore, we propose a novel formulation of regression with    with LASSO for estimation as well as proponent group selection.
% , though most of them are focused on measuring for one single treatment (i.e. source in our case) \fixme{CITE}. There are works for multiple treatments, but  or mak

\subsection{Precision-Controlled Selection -- Knockoffs}
\label{subsec:knockoffs}
Given estimates of $AME_i$ measured through either LASSO or diff-in-means, one can choose a threshold $t$ and select those sources as the proponent group with an estimate $\geq t$. Without the loss of generality, we assume the estimate is measure through LASSO. The choice of $t$ is critical to the quality of selection and must be chosen carefully.
%Moreover, users may have different preference for the selection: some may favor a power selection that selects more proponents, while some may favor a conservative selection that selects the proponents more accurately. 
Let $\hat S_+$ be the sources selected and $S_+$ be the true set of proponents, then we can quanlify the selection through \emph{precision} and \emph{recall}, defined as follows: 
\begin{equation*}
\begin{aligned}
    &precision&=\frac{|\{i \in \hat{S}_+ \cap S_+ \}|}{|\hat{S}_+|},
\\
    &recall&=\frac{|\{i \in \hat{S}_+ \cap S_+ \}|}{|S_+|}
\end{aligned}
\end{equation*}
with $precision=1$ when its denominator is 0. Define false discovery proportion (FDP) as $FDP=1-precision$, and false discovery rate (FDR) as the expected $FDP$. %We emphasize that the above definitions are all one-sided, \ie only treating selecting proponents as correct, but not opponents, which differs from the common definitions (\eg as in \cite{candes_panning_2017}) that treats selecting opponents as correct as well.
%Thus a power selection corresponds to high recall and conservative corresponds to high precision.

\notejinkun{does the following paragraph make sense?} We apply a framework called Knockoffs \cite{candes_panning_2017} in choosing $t$. Knockoffs aim to select the variables not independent of an outcome variable from many variables, with the guarantee to bound the expected precision to be at least a given value. This offers some form of guarantee of the selection quality, and also gives users flexibility to choose $t$ based on their precision requirement. Back to our case, $X_i$ is independent of $Y$ for neutrals while not independent for proponents and opponents. This suggests that we can apply Knockoffs to select the non-neutrals with precision control. This is, however, not exactly the goal we want to achieve; instead, we only want to select the proponents. Therefore, we slightly modify the procedure to adapt into our case. 

\paragraph{The technique} The technique requires to generate one "knockoff" covariate for each of the original ones, and fit the estimation model (\ie LASSO here) on both the knockoff and original covariates. By comparing between the statistics of the knockoff and original covariates, the procedure can compute a threshold bounding the FDR. 

% However, the original Knockoffs is controlling a two-sided FDR that does not count selecting an opponent as an error. Thus we slightly modify the procedure into a one-sided version. Due to limit of effort, we only validate its effectiveness through the empirical evaluation, but leave the formal proof for future work. \notejinkun{OK to say so?}

Specifically, when running the subset sampling and LASSO, we pretend as if there are $2n$ sources with the first $n$ being original sources and last $n$ being knockoff ones that contain no data. Let's term the covariates of the original sources $D=(D_1,\dots,D_n)$ and covariates of the knockoff ones $\tilde{D}=(\tilde D_1, \dots,\tilde D_n)$. %The goal is to create variables (i.e. $\tilde{D}$) that we know for sure are independent of $Y$ and thus should not be selected. This serves as a reference for further reasoning about which original sources should not be selected. %the same distribution as $D_i$ for $i=0,\ldots,n-1$. 

Next, given a target FDR level $q$, we pick a threshold $\tau$ by setting\footnote{Per footnote of \cite{candes_panning_2017}: $\min \{t > 0 : \dots\}$ actually means $\min \{t \in W_+ : \dots \}$, where $W_+ = \{|W_i| : |W_i| > 0\}$}
\begin{equation}
\tau=\min \left\{t>0: \frac{\#\left\{i: W_{i} \leq-t\right\}}{\#\left\{i: W_{i} \geq t\right\}} \leq q\right\},
\end{equation}
where $W_i=\max(\hat l_i,0)-\max(\hat l_{i+n},0)$. $\tau=+\infty$ if the set upon which $\min$ is taken is empty. Finally, the procedure selects the sources
\begin{equation*}
    \hat S_+=\{i:W_i\geq \tau\}
\end{equation*}

With some assumption (discussed shortly), the procedure controls a modified FDR defined below
\begin{equation}
\label{eq:mFDR}
mFDR=\mathbb{E}\left[\frac{\left|\left\{i \in (\hat{S}_+ - S_+) \right\}\right|}{|\hat{S}_+|+1 / q}\right] \leq q.
\end{equation} 
Though not controlling the true $FDR$, it is still useful since $mFDR$ differs from $FDR$ only in the extra $1/q$ in the denominator. \footnote{The Knockoffs paper also provides a variant called \emph{Knockoffs+} that controls $FDR$, which we are not using since we expect there are very few proponents in which case Knockoffs+ would be too conservative and selects very few sources.}

Overall, the pseudo code of LASSO+Knockoffs is shown in Algo. \ref{algo:k1} and Algo. \ref{algo:k2}.
\paragraph{Difference compared to original Knockoffs} Note that the original Knockoffs is controlling a "two-sided" FDR that does not count selecting an opponent as an error, which is different from our "one-sided" version. Thus we slightly modified the procedure as follows: in assigning $W_i$, they use $W_i=|\hat l_i|-|\hat l_{i+n}|$, but we instead use $W_i=\max(\hat l_i,0)-\max(\hat l_{i+n},0)$. The intuition is that the opponents would probably have $l_i\leq 0$, different from a neutral which would probably be $\hat l_i=0$. Taking a $\max(\cdot,0)$ makes opponents behave more similar to neutrals, and thus makes two-sided FDR closer to one-sided FDR, enabling us to directly apply original Knockoffs that controls the two-sided FDR onto the one-sided FDR. \notejinkun{Is the following statement correct?} More precisely, if we assume $\max(\hat l_i,0)$ has the same distribution for both opponents and neutrals, the procedure will control the $mFDR$ correctly. Otherwise, further analysis is needed, but due to limit of effort, we only validate its effectiveness through the empirical evaluation, but leave the formal proof for future work. \notejinkun{OK to say so?}



% \begin{proposition}
% Assume that $AME_i=0$ for any source $i$ that is neither proponent or opponent. Then the above threshold controls a modified FDR defined as
% \begin{equation}
% \label{eq:mFDR}
% mFDR=\mathbb{E}\left[\frac{\left|\left\{j \in (\hat{S}_+ - S_+) \right\}\right|}{|\hat{S}_+|+1 / q}\right] \leq q,
% \end{equation}
% where $S_+$ denotes the true proponent group.
% \end{proposition}
% %Now we claim $\tilde D$ is the Knockoffs of $D$. 
% \begin{proof}
% TBD \notejinkun{probably this proposition is wrong...}
% For this to be true, according to the Knockoff paper\cite{candes_panning_2017}, 2 properties must be satisfied: \emph{(1) for any subset $S \subset\{0, \ldots, n-1\}$,
% $$
% (D, \tilde{D})_{\operatorname{swap}(S)} \stackrel{d}{=}(D, \tilde{D})
% $$
% (2) $\tilde{D} \perp Y | D$  if there is a response  $Y$.}

% Above, the vector $(D, \tilde{D})_{\operatorname{swap}(S)}$ is obtained from $(D, \tilde D)$ by swapping the entries $D_j$ and  $\tilde D_j$ for each
% $j \in S$. (1) is guaranteed since each $D_i$ and $\tilde D_i$ are independently assigned. (2) is also guaranteed since $\tilde D$ constructed without looking at $Y$. Therefore, $\tilde D$ is the knockoffs of $D$.
% \end{proof}

\sid{I agree that we should have one main algorithm in pseudocode that summarizes our methodology. What we have below is a good start.}

\begin{algorithm}[h]
\DontPrintSemicolon
% \KwResult{Write here the result }
\SetKwFunction{FtrainOnComb}{trainOnSubset}
\SetKwFunction{FsampleSubsets}{sampleSubsets}
\SetKwFunction{Ftrain}{train}
\SetKwFunction{FLASSO}{LASSO}
\SetKwFunction{Fselect}{select}
 \KwIn{$n$, number of data sources}
 \KwIn{$m$, number of models (or observations for the analysis)}
 \KwIn{$\mathcal P=\{p_1,\dots,p_b\}$, probabilities to include data source. Default $\{0.2, 0.4, 0.6, 0.8\}$}
 \KwIn{$L$, query label}
 \KwIn{$I$, query input}
 $[\mathbf{D}, \mathbf{\tilde D}] \gets [zeros(m,n), zeros(m,n)]$\tcp*[r]{init the design matrices, where $\mathbf{\tilde D}$ is knockoff}
 $\mathbf{B} \gets zeros(m,b)$\;
 $Y\gets zeros(m)$\tcp*[r]{Outcome vector init}
 \For{$i\gets1$ \KwTo $m$ }{
   $r \sim UniformInt(1,b)$\;
   $\mathbf{B}[i,r]\gets 1$\;
  \For{$j\gets1$ \KwTo $n$ }{
   $r_1 \sim Bernoulli(p_r)$\;%\tcp*[r]{$r_1$ is either 0 or 1. 1 means source is included}
   $r_2 \sim Bernoulli(p_r)$\tcp*[r]{for knockoffs}
%   $\mathbf{C}[i,j],\mathbf{\tilde C}[i,j] \gets r_1, r_2$\; 
   $\mathbf{D}[i,j],\mathbf{\tilde D}[i,j] \gets \frac{r_1}{p_r}-\frac{1-r_1}{1-p_r}, \frac{r_2}{p_r}-\frac{1-r_2}{1-p_r}$\; 
   }
  $\mathcal{M}_i \gets \FtrainOnComb(\mathbf{D}[i,:])$\;%\tcp*[r]{train model on combination $\mathbf{D}[i,:]$}
  $Y[i]\gets \mathcal{M}_i(I)[L]$\tcp*[r]{obtain confidence}
 }
 $\mathbf{X}\gets [\mathbf D,\mathbf{\tilde D},\mathbf{B}]$\tcp*[r]{concat through columns to get final design matrix}
 \KwRet{$\hat l\gets$ \FLASSO{$\mathbf{X},Y,\lambda$}}\tcp*[r]{run LASSO with the $\lambda$ chosen by cross validation.}
%  \KwRet{\Fselect{$\hat l,q$}}\;
 \;
%  \Fn(\tcp*[f]{train on 1 combination \textbf C}){\FtrainOnComb{$\mathbf D$}}{
 \Fn(){\FtrainOnComb{$\mathbf D$}}{
%  \KwIn{$\mathbf D$, an array of size $n$ made up of 0 and 1}
  $S \gets \{\}$\tcp*[r]{training set for this model}
  \For{$j\gets1$ \KwTo $n$}{
   \lIf{$\mathbf D[j] > 0$}{$S\gets S+\{j\}$}
  }
  \KwRet{\Ftrain{S}}\;%\tcp*[r]{train from scratch or fine-tune on $S$}
 }
 \caption{Obtaining LASSO coefficients\label{algo:k1}}
\end{algorithm}

\sid{I'm not sure I derived much value from Algorithm 2 (FDR stuff); we might just state it in a couple of sentences.}

\begin{algorithm}[h]
\DontPrintSemicolon
\SetKwFunction{Fselect}{select}
%  \Fn(\tcp*[f]{select non-null features with FDR under control}){\Fselect{$\hat l, q$}}{
  \KwIn{$\hat l$, the LASSO coef of size $2n$}
  \KwIn{$q$, the target FDR level}
  $W \gets zeros(n)$\tcp*[r]{statistics}
  \For{$i\gets1$ \KwTo $n$}{
   $W_i=\max(\hat l_i,0)-\max(\hat l_{i+n},0)$\;
  }
  $\tau \gets \min \left\{t>0: \frac{\#\left\{i:W_{i} \leq-t\right\}}{\#\left\{i:W_{i} \geq t\right\}} \leq q\right\}$\tcp*[r]{find the threshold given the desired FDR}
  $\hat S_+ \gets \{\}$\;%\tcp*[r]{non-null features (or data sources) indices}
  \For{$i\gets1$ \KwTo $n$}{
   \lIf{$W_i\geq\tau$}{$\hat S_+\gets \hat S_++\{i\}$}
  }
  \KwRet{$\hat S_+$}
%  }
 \caption{FDR-controlled feature selection\label{algo:k2}}
\end{algorithm}


\subsection{Training Optimization -- Warm-Starting}
\label{subsec:warm-starting}
\sid{Some of the details in the "Implementation" section could be moved here. With fine-tuning, I think its fine to describe our methodology for doing the training itself, which may include details such as what hyperparameters and training schedule we used.}

\notepanda{Isn't this an optimization for both Lasso and ``Diff in Means''?}\notejinkun{Yes, it is. So should I put it after knockoffs?}
Training of models is costly, especially for large models. Thus we further propose to use warm-starting as a proxy of original full training when there is not enough computation budget. The idea is that instead of training a model from scratch, we only fine-tune starting from the main model (\ie the model deployed by Alice if in the running example) for some number of iterations. Moreover, we design the grid $\mathcal{P}$ specifically to only cover the lower half range (i.e. $P\leq0.5)$ based on our observations in experiments.\sid{This seems ad-hoc, but I think we have justification elsewhere we can borrow from.} We call this approach \emph{warm-starting} or \emph{fine-tuning} interchangeably\sid{Let's pick one}, and refer to the original approach as \emph{training-from-scratch}.

\paragraph{Justifying using only lower half range of $P$} What we find in experiments is that very low $P$s are the most helpful at distinguishing between proponents and opponents. For example, in Fig. \ref{fig:diff-in-means}, $P=0.01$ or $0.1$ work well in warm-starting. The reason is probably that low $P$s make it more likely to sample a subset without any proponent, in which adding one proponent will significantly elevate the signal $U(\cdot{})$. This does not happen in training-from-scratch probably because (a) too few data are insufficient to train a reasonable model; (b) it is much easier to maintain what has been learned than learning from scratch, thus one single source is able to pull up the signal in warm-starting while not in training-from-scratch \sid{This point is a bit counter-intuitive and needs some explanation}. In experiment we use $\mathcal{P}=\{0.01, 0.1, 0.2, 0.3, 0.4, 0.5\}$ and it works well. We still include up to $0.5$ to cover the case of $k=1$. In the case where there are not many sources in total we remove $0.01$ to avoid the distribution deviation problem. \notejinkun{Does this justification make sense? If not, how should we justify?}.

\paragraph{Advantages} Warm-starting generally helps the convergence, because the starting model is already converged in the whole dataset. The rest is only to transfer it into the subset, and is likely faster. Although it may not produce exactly the same result as training-from-scratch, the numbers are still comparable, suggesting that it can still be used to measure the supportive-ness and thus is a reasonable substitute for the original $U(\cdot)$. Moreover, warm-starting enables tiny $P$s \sid{This needs another line of explanation}. Besides the reason given in the justification above, the other reason is that the whole dataset has already been learned and we could worry less about the distribution deviation problem discussed in Sec. \ref{sec:p-pop}. \notejinkun{Probably the insufficient data problem in group testing could also be handled this way.} However, that is not to say we can never worry about that and pick extremely tiny $P$.

\paragraph{Disadvantages} On the other hand, fine-tuning cannot fully represent training-from-scratch and it is possible that some sources will have different effect between fine-tuning and training-from-scratch. The other downside is that fine-tuning generally gives a noisier signal, and may requires more observations. \sid{This sentence seems to contradict what we say above regarding the benefits of fine-tuning.}


==> rm/approach-v3.tex <==
\section{Methodology}
\label{sec:methodology}

%\mathias{[TODO Mathias]: disentangle data subsets and sample models in the following. Introduce the methodology and its steps in a more algorithmic way. Will do after writing each subsection. We also need to define queries upfront.}
%\mathias{[TODO Mathias]: use previously defined notation, or introduce it as necessary, so that we can talk more clearly about the different subsets, models, utility, etc... Leveraging the algorithm should work.}
\begin{algorithm2e}[t!]
{\small
  \DontPrintSemicolon
  % \KwResult{Write here the result }
  \SetKwFunction{FtrainOnComb}{trainOnSubset}
  \SetKwFunction{FtrainOnSubsets}{trainOnSubsets}
  \SetKwFunction{FsampleSubsets}{sampleSubsets}
  \SetKwFunction{FKnockoff}{knockoff}
  \SetKwFunction{Festimate}{estimate}
  \SetKwFunction{Ftrain}{train}
  \SetKwFunction{FLASSO}{LASSO}
  \SetKwFunction{Fselect}{select}
   \KwIn{number of data sources $n$, number of subsets $m$ to draw, probabilities $\mathcal P=\{p_1,\dots,p_b\}$ to include data source (default $\{0.2, 0.4, 0.6, 0.8\}$), query label $Q_L$, query input $Q_I$, target FDR level $q$}
   \tcp{offline phase}
   $S, \mathbf{X} \gets$ \FsampleSubsets{}\tcp*[r]{step 1}
   $\mathcal{M}_S\gets$ []\;
   \For(\tcp*[f]{step 2}){$j\gets1$ \KwTo $m$}{
        $\mathcal{M}_S$.append(\FtrainOnComb{$S[j]$})
   }
   \tcp{online phase}
   \While{$Q \gets$ new query}{
        $\hat \beta_{lasso} \gets$ \Festimate{$\mathbf X, \mathcal{M}_S, Q$}\tcp*[r]{step 3}
        $\hat S_+ \gets$ \FKnockoff($\hat \beta_{lasso}, q$)\tcp*[r]{step 4}\;
   }

   \Fn(){\FsampleSubsets{}}{
   $S \gets []$\;
   $[\mathbf{D}, \mathbf{\tilde D}] \gets [zeros(m,n), zeros(m,n)]$
   \tcp*[l]{source and knockoff covariates}
   $\mathbf{B} \gets zeros(m,b)$\tcp*[r]{bucket covariates}
   \For{$j\gets1$ \KwTo $m$ }{
    $r \sim UniformInt(1, b)$\tcp*[r]{draw $p$}
    $\mathbf{B}[j,r]\gets 1$\;
    $S$.append($\{\}$)\;
    \For{$i\gets1$ \KwTo $n$ }{
     $r_1 \sim Bernoulli(p_r)$\;%\tcp*[r]{$r_1$ is either 0 or 1. 1 means source is included}
     $r_2 \sim Bernoulli(p_r)$\tcp*[r]{knockoffs}
     \lIf{$r_1 = 1$}{$S[j]\gets S[j]+\{i\}$}
    %  \lIf{$r_2 = 1$}{$\tilde S[j]\gets \tilde S[j]+\{i\}$}
     $\mathbf{D}[j,i],\mathbf{\tilde D}[j,i] \gets \frac{r_1}{p_r}-\frac{1-r_1}{1-p_r}, \frac{r_2}{p_r}-\frac{1-r_2}{1-p_r}$\; 
    }
   }
   $\mathbf{X}\gets [\mathbf D,\mathbf{\tilde D},\mathbf{B}]$\tcp*[r]{concat through columns to get final design matrix}
   \KwRet{$S, \mathbf{X}$}
   \;
   }\;
   \Fn(){\Festimate{$\mathbf X,\mathcal M_S, Q$}}{
   $Q_I, Q_L \gets Q$\;
   $Y\gets zeros(m)$\tcp*[r]{outcome vector}
  %  \lFor(\tcp*[h]{inference}){$j\gets1$ \KwTo $m$ }{
   \For{$j\gets1$ \KwTo $m$ }{
    $Y[j]\gets \mathcal{M}_S[j](Q_I)[Q_L]$\tcp*[f]{inference}
   }
   \KwRet{$\hat \beta_{lasso}\gets$ \FLASSO{$\mathbf{X},Y,\lambda$}}\tcp*[r]{$\lambda$ is chosen by cross validation.}
  %  \KwRet{\Fselect{$\hat l,q$}}\;
   }
   }
   \caption{Overall Workflow of \somename{}\label{alg:approach}}
  \end{algorithm2e}

% {\small
% \begin{algorithm}[t]
%   \DontPrintSemicolon
%   % \KwResult{Write here the result }
%   \SetKwFunction{FtrainOnComb}{trainOnSubset}
%   \SetKwFunction{FtrainOnSubsets}{trainOnSubsets}
%   \SetKwFunction{FsampleSubsets}{sampleSubsets}
%   \SetKwFunction{FKnockoff}{knockoff}
%   \SetKwFunction{Festimate}{estimate}
%   \SetKwFunction{Ftrain}{train}
%   \SetKwFunction{FLASSO}{LASSO}
%   \SetKwFunction{Fselect}{select}
%   \KwIn{number of data sources $n$, number of subsets $m$ to draw, probabilities $\mathcal P=\{p_1,\dots,p_b\}$ to include data source (default $\{0.2, 0.4, 0.6, 0.8\}$), query label $Q_L$, query input $Q_I$, target FDR level $q$}
%   \tcp{offline phase}
%   $S, \mathbf{X} \gets$ \FsampleSubsets{}\tcp*[r]{step 1}
%   $\mathcal{M}_S\gets$ []\;
%   \For(\tcp*[f]{step 2}){$i\gets1$ \KwTo $m$}{
%         $\mathcal{M}_S$.append(\FtrainOnComb{$S[i]$})
%   }
%   \tcp{online phase}
%   \While{$Q \gets$ new query}{
%         $\hat \beta_{lasso} \gets$ \Festimate{$\mathbf X, \mathcal{M}_S, Q$}\tcp*[r]{step 3}
%         $\hat S_+ \gets$ \FKnockoff($\hat \beta_{lasso}, q$)\tcp*[r]{step 4}\;
%   }

%   \Fn(){\FsampleSubsets{}}{
%   $S \gets []$\;
%   $[\mathbf{D}, \mathbf{\tilde D}] \gets [zeros(m,n), zeros(m,n)]$
%   \tcp*[l]{source and knockoff covariates}
%   $\mathbf{B} \gets zeros(m,b)$\tcp*[r]{bucket covariates}
%   \For{$i\gets1$ \KwTo $m$ }{
%     $r \sim UniformInt(1, b)$\tcp*[r]{draw $p$}
%     $\mathbf{B}[i,r]\gets 1$\;
%     $S$.append($\{\}$)\;
%     \For{$j\gets1$ \KwTo $n$ }{
%      $r_1 \sim Bernoulli(p_r)$\;%\tcp*[r]{$r_1$ is either 0 or 1. 1 means source is included}
%      $r_2 \sim Bernoulli(p_r)$\tcp*[r]{knockoffs}
%      \lIf{$r_1 = 1$}{$S[i]\gets S[i]+\{j\}$}
%     %  \lIf{$r_2 = 1$}{$\tilde S[i]\gets \tilde S[i]+\{j\}$}
%      $\mathbf{D}[i,j],\mathbf{\tilde D}[i,j] \gets \frac{r_1}{p_r}-\frac{1-r_1}{1-p_r}, \frac{r_2}{p_r}-\frac{1-r_2}{1-p_r}$\; 
%     }
%   }
%   $\mathbf{X}\gets [\mathbf D,\mathbf{\tilde D},\mathbf{B}]$\tcp*[r]{concat through columns to get final design matrix}
%   \KwRet{$S, \mathbf{X}$}
%   \;
%   }\;
%   \Fn(){\Festimate{$\mathbf X,\mathcal M_S, Q$}}{
%   $Q_I, Q_L \gets Q$\;
%   $Y\gets zeros(m)$\tcp*[r]{outcome vector}
%   %  \lFor(\tcp*[h]{inference}){$i\gets1$ \KwTo $m$ }{
%   \For{$i\gets1$ \KwTo $m$ }{
%     $Y[i]\gets \mathcal{M}_S[i](Q_I)[Q_L]$\tcp*[f]{inference}
%   }
%   \KwRet{$\hat \beta_{lasso}\gets$ \FLASSO{$\mathbf{X},Y,\lambda$}}\tcp*[r]{$\lambda$ is chosen by cross validation.}
%   %  \KwRet{\Fselect{$\hat l,q$}}\;
%   }
%   \caption{Overall Workflow of \somename{}\label{alg:approach}}
%   \end{algorithm}
% }

Our methodology, summarized at a high level in Figure \ref{fig:workflow}, is designed to efficiently compute the \quantity{} for multiple queries under our sparsity assumption, and provides rigorous control for the false detection rate.
%
%Recall that a query consists of an input $Q_I$ and target label $Q_L$, and $\textrm{AME}_i$ aims to explain the impact of data source $i$ on the score for label $Q_L$ given by the main model when predicting on the query input $Q_I$: $\mathcal{M}(Q_I)[Q_L]$.
%
%That is, in \quantity{} parlance (\S\ref{subsec:ame}), given a subset of the data $S$, $U(S) = \mathcal{M}_S(Q_I)[Q_L]$, where $\mathcal{M}_S$ is a model trained on data subset $S$.
%
Our key insight is that we can estimate the \quantity{} for all data sources and any query based exclusively on models trained offline on random subsets of the training data.
%
Intuitively, given a set of subset models $\mathcal{M}_{S}$ each trained on a random data subset $S$, we compute $\textrm{AME}_i$ by comparing the average score given to the query label by each model including $i$ in $S$ to the average score of each model that does not include $i$ in $S$.
%Because each model $\mathcal{M}_{S_m}$ is trained on a subset of the data, we call them \textit{subset models}, and each can be seen as one sample in a stochastic estimation of the \quantity{}.
Accordingly, each subset model can be seen as one sample in a statistical estimation of the \quantity{}.

To leverage this insight, we design a four step methodology consisting of an offline phase and an online phase, described in Algorithm \ref{alg:approach}. The offline phase creates the subset models and is performed once for the main model $\mathcal{M}$ and reused across queries. The offline phase first samples multiple subsets of the original training data (phase 1 in Algorithm~\ref{alg:approach} and \S\ref{subsec:sampling}) and then train a model using each subset. Optionally, we use warm-start (phase 2, \S\ref{subsec:warm-starting}) to reduce training time. The online phase is executed when a query $(Q_I, Q_L)$ is submitted to the system. In this phase we first use each subset model to compute a score for label $Q_L$ given input $Q_I$. Next, we need to estimate $\textrm{AME}_i$ for each source, but doing so naively by  using Equation~\ref{eq:amep} is inefficient.
Therefore, we instead develop a novel regression problem that leverages sparse recovery results for LASSO to estimate the \quantity{} for all sources. This requires using $O(k\log(n))$ subset models, where $k$ is the number of sources contributing to the score and $n$ is the total number of sources (phase 3, \S\ref{subsec:lasso}). Finally, we select sources based on these LASSO estimates using a knockoff procedure to control the false discovery rate (phase 4, \S\ref{subsec:knockoffs}). This is especially important to avoid false alarms when proponents are sparse. We detail each of these steps in the following subsections.
% The following subsections detail each of these steps, before presenting a hierarchical design extension to support multiple levels of granularity for explaining predictions (\S\ref{sec:hier}).
% In the following 4 sections we describe the underlying challenges for each component and how we overcome them respectively.


\subsection{Sampling Based \quantity{} Estimation}
\label{subsec:sampling}

To estimate $AME_i(\mathcal{L}^i_{\mathcal{P}})$ (Eq. \ref{eq:amep}), the most straightforward approach is to sample subsets of the dataset from $\mathcal{L}^i_{\mathcal{P}}$ and compute the average marginal effect of source $i$ when added to this subset.
However, this is costly because it requires training two models to learn about one source.
Indeed, a simple application of Hoeffding's inequality to bound the $L_2$ norm of $AME_i(\mathcal{L}^i_{\mathcal{P}})$ for every source together would require $O(n^2\log(n))$ subset models, which is not feasible on large datasets. This is also the reason for the linear $n$ term in Jia et al's\cite{jia_towards_2020} method for estimating Shapley values.

By formulating the \quantity{} based on data sources selected {\em independently} at random, however, we enable the sharing of subset models across \quantity{} estimates for different data sources.
Consider $AME_i(\mathcal{L}^i_{p})$ for one fixed value of $p$: regardless of the source $i$, each source other than $i$ is included independently at random with probability $p$.
Based on this observation we introduce $\mathcal{L}_p$, a subset distribution in which {\em each source} is included independently with probability $p$.
Given subsets from such a distribution, for each $i$ we can compute $AME_i(\mathcal{L}^i_{p})$ by comparing subsets with and without $i$, in effect re-using subset models across data sources:
\begin{align}
    AME_i &=\mathbb E_{S^i\sim \mathcal{L}^i_p}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_p}[U(S^i)] \nonumber\\
    &=\mathbb E_{S\sim\mathcal{L}_p}[U(S)|i\in S]-\mathbb E_{S\sim\mathcal{L}_p}[U(S)|i\notin S] \label{eq:diff-in-means}
\end{align}
The first equality holds by linearity of expectation, while the second leverages the independence of source selection.
This approach is akin to randomized designs from statistics or factorial experiments from causal inference. Subsets $S$ are sampled offline only once and are used as training sets for our subset models, from which we will gather the necessary signals online whenever a query arrives.

We extend this approach to multiple values of $p$ in a set $\mathcal{P}$. With a slight abuse of notation we denote $p \sim \mathcal{P}$ a draw from the uniform distribution over $\mathcal{P}$, resulting in:
\begin{align}
    &\textrm{AME}_i = \nonumber\\
    & \mathbb E_{p\sim \cP}\left[\mathbb E_{S\sim\mathcal{L}_p}[U(S)|p,i\in S]-\mathbb E_{S\sim\mathcal{L}_p}[U(S)|p,i\notin S]\right] \label{eq:diff-in-means-p}
\end{align}

We discuss how to estimate this quantity efficiently in \S\ref{subsec:lasso}.

%\notejinkun{this whole section is just to (i) stating that we want to sample the subsets altogether (\ie reusing subsets for estimating each source; (ii) and showing why this can be still estimating the same thing (\ie by showing the expectation of difference (\eqref{eq:amep}) equals difference of expectation (\eqref{eq:diff-in-means-true}. btw sorry that I pointed to a wrong place during the meeting). Don't hesitate to ping me if you feel confused (which is probably my bad of writing or the argument is truly incorrect)!}

%\notepanda{Is this really a viable option? This section read a bit like us beating up on a strawman that obviously would not work: just say it is costly and move on?}


%To estimate the $AME_i(\mathcal{L}^i_{\mathcal{P}})$,the most straightforward approach is sampling the subsets and compute their average marginal effects. However, this is too costly, since it requires training two models for each subset, and every source requires the same procedure, thus the models to train is at least $O(n)$. \notejinkun{UPDATED on Feb 21} \sout{What is worse, every source requires many draws to ensure accurate estimation, therefore this approach is not ideal.} To overcome this challenge, we propose a new sampling scheme that reuses the subsets. \sout{We also present a strawman approach called \emph{diff-in-means}.}


% To estimate the $AME_i(\mathcal{L}^i_{\mathcal{P}})$, the most straightforward approach is sampling the subsets and compute their average marginal effects. However, this is too costly, since it requires training two models for each subset, and every source requires the same procedure, thus the models to train is at least $O(n)$. \notejinkun{UPDATED on Feb 21} \sout{What is worse, every source requires many draws to ensure accurate estimation, therefore this approach is not ideal.} To overcome this challenge, we propose a new sampling scheme that reuses the subsets. \sout{We also present a strawman approach called \emph{diff-in-means}.}

%To make it clear, we state the new sampling scheme as follows. Now instead of subsampling from $n-1$ sources separately for every source, we subsample from $n$ sources altogether. The inclusion probability $P$ is still drawn uniformly from the same set $\mathcal{P}$. Define $\mathcal{L}_\mathcal{P}$ as the corresponding population. Notice that this new sampling distribution is slightly different from the original one defining $AME$, and thus some further adjustment is needed to ensure correct, unbiased estimation. We detail the adjustment procedure in the section of estimation \S \ref{subsec:lasso}.
%We also call this new sampling scheme $\mathcal{L}_\mathcal{P}$ and the old scheme $\mathcal{L}^i_\mathcal{P}$ when there is no ambiguity. %Assume that a subset sample $(S^{(j)})_{j=1}^m$ with size $m$ is drawn, and denote their corresponding $P$ values by $(P^{(j)})_{j=1}^m$. 


% The question remained is how to estimate correctly the $AME_i(\mathcal{L}^i_\mathcal{P})$ defined under $\mathcal{L}^i_\mathcal{P}$ using $\mathcal{L}_\mathcal{P}$. First we rewrite $AME_i$ as $\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S+\{i\})]-\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]$. It follows that 
% \begin{subequations}
% \begin{align}
% &f_{S|P}^i(s|p)=f_{S|P,i\notin S}(s|p)\\
% &f_{S|P}^i(s|p)=f_{S|P,i\in S}(s|p)
% \\
%     &\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim f_{S|P}^i(s|p)}[U(S)]]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim f(S|P=p,i\notin S)}[U(S)]|P]\\
% \end{align}
% \end{subequations}
% \begin{subequations}
% \begin{align}
%     &\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim \mathcal{L}^i(S|P=p)}[U(S+\{i\})]-\mathbb E_{S\sim \mathcal{L}^i(S|P=p)}[U(S)]|P]\\
%     ={}&\mathbb E_{P\sim \mathcal{P}}[\mathbb E_{S\sim \mathcal{L}(S|P=p,i\in S)}[U(S)]-\mathbb E_{S\sim \mathcal{L}(S|P=p,i\notin S)}[U(S)]|P]\\
% \end{align}
% \end{subequations}


%\paragraph{Disadvantages}
%Though being more efficient at sampling, reusing samples potentially brings high variance in the estimators when $\mathcal{P}$ includes low/high $P$, because low $P$ will have few samples of $U(S)$ with $i\in S$, and vice versa for high $P$, which would be problematic for estimating $\mathbb E[U(S^i+\{i\}) - U(S^i) | P]$ accurately under low/high $P$. To mitigate this issue we recommend choosing a highly sparse grid $\mathcal{P}$, thus each $\mathcal{P}$ can have enough samples to counter the variance.\footnote{A more aggressive scheme could be, instead of sampling $P$ uniformly, sampling more for low/high $P$ and fewer for middle $P$, but it is unclear what would be the best ratio among different $P$. We leave it as future work.}

\subsection{Training Subset Models}
\label{subsec:warm-starting}

The second step of the offline phase consists of training a model for each sampled data subset. We use the same architecture and training procedure as the main model under study.
Because the models' predictions will be used to assess $U(S)$, there are three considerations to account for when selecting $\mathcal{P}$.
First, for each value of $p$ we need enough samples to estimate both $\mathbb E_{S\sim\mathcal{L}_p}[U(S)|i\in S]$ and $\mathbb E_{S\sim\mathcal{L}_p}[U(S)|i\notin S]$. We thus make $\mathcal{P}$ sparse, so that each value has enough samples with and without each source.
Second, we avoid very small values of $p$. These include too few data sources, potentially yielding very noisy models that are not helpful to detecting the influence of data sources on a given prediction.
Third, we avoid large values of $p$, which mostly keep the dataset constant and suffer from the same drawbacks as influence functions.
For most of our experiments we use $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$, and we evaluate these effect of this choice in \S\ref{sec:eval}.

%First, it should be sparse, i.e. $b$ is small. This is to help achieve a good estimation in later procedure that will be discussed shortly (see \S\ref{subsec:sampling}). %LASSO is essentially aggregating the result for each $P$, and aggregating a lot of bad results is no better than aggregating a few good results. By making it sparse, each $P$ can have a better result. Too dense or even doing continuous sampling instead would probably yield garbage output for each $P$. 

%\notejinkun{this is for the original verision without monontonicity assumption} Second very low $P$ should not be included. Because too low a $P$ subsamples too few sources, in which the non-proponents' distribution may deviate too far away from the full dataset. In such a case, adding/removing one source could have very different results. For example, consider each source contains only data of one label, and $P$ is so small that $S^i$ is empty. Now $U(S^i+\{i\})=U(\{i\})$ is obtained by training model on only source $i$ that has only one label, meaning that it always would predict the source's label. Thus its marginal effect collapses into always giving high value for a source sharing label the same as the query label. However, not every such source is causing the query prediction, especially in the case of one training example per source.

%\fixme{subject to change before the experiment result is out}\notejinkun{this is for the new verision with monontonicity assumption} Second very low $P$ should not be included. Because too low a $P$ subsamples too few sources, in which the model has no information to infer about the input and thus has to guess randomly. The monotonicity assumption tends to break under this situation, potentially creating many false positives.% In the previous running example, suppose $S$ only contains source $2a$, then the trained model would produce label '2' for any input. If we add the clean source $1a$ into $S$, the model would likely flips a coin to choose between '1' and '2', which appears as if source $1a$ has a positive marginal effect, even if $1a$ is not the cause of the poisoned prediction. %For example, \fixme{we could use the running example if it is exactly what is described here} consider MNIST example where there are 10 sources each containing only data of one label, and the query is an image of poisoned 0 being predicted as 1 because of malicious source 1. If $P$ is so small that $S$ is only $\{2\}$, adding $0$ to $S^i$ would  obtained by training model on only source $i$ that has only one label, meaning that it always would predict the source's label. Thus its marginal effect collapses into always giving high value for a source sharing label the same as the query label. However, not every such source is causing the query prediction, especially in the case of one training example per source.

%\notejinkun{version 3 of previous paragraph}
%Second very low $P$ should not be included. Because too low a $P$ subsamples too few sources, in which, the model is not able to learn the distinguished features that cause the query label predicted, and thus not useful for identifying proponents. In Alice's case, the model would fail to learn the watermark and predicts as if there is no watermark.

%Third, very high $P$ should not be included either. Too high a $P$ would almost make no change to the dataset, and thus suffer from the same issue as the traditional LOO test (see the previous 1-Nearest-Neighbor for a detailed example). 



% Finally, We demonstrate that it is robust in that it performs well across a wide range of applications, and compare against fixing $P=0.5$ Experimental results are shown in Tab. \ref{tab:p0.5}. \fixme{TODO: experiments. Ideally find at least one case where $P=0.5$ is worse in training-from-scratch. Now EMNIST has an experiment of $P=0.5$ and it's worse than uniform p.}.


%There is also a variance issue in practice that prohibits very low/high $P$ (see \S\ref{subsec:sampling}). We use $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$ unless otherwise specified.


\mypara{Warm-starting optimization}
Training deep learning models, especially large ones, is costly. As an optional optimization, we use warm-starting as a proxy for full training. Instead of training a subset model from scratch, we update the main model on subset $S$ for a fixed number of iterations, usually the number of iterations in one main model training epoch.
% typically the number of iterations in one epoch of training for the main model.

With warm-starting, subset models behave differently than when training from scratch. Indeed, instead of learning a model from the subset $S$, we ``unlearn'' the signal from the points not in $S$, which has two implications on our choice of $\mathcal{P}$.
First, changing the outcome of a given query usually requires removing all proponents, as even a small number of them is sufficient to maintain the signal learned in the main model. Hence, we only consider lower inclusion probabilities ($p\leq0.5$). Higher values of $p$ make it too likely that at least one proponent will remain, preventing comparisons between subsets with and without proponents.
Second, warm-starting is stable even on very small data subsets, as opposed to learning the entire model from scratch. We can thus consider smaller values of $p$, and settle on the range $\mathcal{P}=\{0.01, 0.1, 0.2, 0.3, 0.4, 0.5\}$.
We discuss this and other hyper-parameters for warm-starting in \S\ref{sec:eval}.

% Moreover, we design the grid $\mathcal{P}$ specifically to only cover the lower half range (i.e. $P\leq0.5)$ based on our observations in experiments.\sid{This seems ad-hoc, but I think we have justification elsewhere we can borrow from.} We call this approach \emph{warm-starting} or \emph{fine-tuning} interchangeably\sid{Let's pick one}, and refer to the original approach as \emph{training-from-scratch}.

% \paragraph{Justifying using only lower half range of $P$} What we find in experiments is that very low $P$s are the most helpful at distinguishing between proponents and opponents. For example, in Fig. \ref{fig:diff-in-means}, $P=0.01$ or $0.1$ work well in warm-starting. The reason is probably that low $P$s make it more likely to sample a subset without any proponent, in which adding one proponent will significantly elevate the signal $U(\cdot{})$. This does not happen in training-from-scratch probably because (a) too few data are insufficient to train a reasonable model; (b) it is much easier to maintain what has been learned than learning from scratch, thus one single source is able to pull up the signal in warm-starting while not in training-from-scratch \sid{This point is a bit counter-intuitive and needs some explanation}. In experiment we use $\mathcal{P}=\{0.01, 0.1, 0.2, 0.3, 0.4, 0.5\}$ and it works well. We still include up to $0.5$ to cover the case of $k=1$. In the case where there are not many sources in total we remove $0.01$ to avoid the distribution deviation problem. \notejinkun{Does this justification make sense? If not, how should we justify?}.

% \paragraph{Advantages} Warm-starting generally helps the convergence, because the starting model is already converged in the whole dataset. The rest is only to transfer it into the subset, and is likely faster. Although it may not produce exactly the same result as training-from-scratch, the numbers are still comparable, suggesting that it can still be used to measure the supportive-ness and thus is a reasonable substitute for the original $U(\cdot)$. Moreover, warm-starting enables tiny $P$s \sid{This needs another line of explanation}. Besides the reason given in the justification above, the other reason is that the whole dataset has already been learned and we could worry less about the distribution deviation problem discussed in Sec. \ref{sec:p-pop}. \notejinkun{Probably the insufficient data problem in group testing could also be handled this way.} However, that is not to say we can never worry about that and pick extremely tiny $P$.

% \paragraph{Disadvantages} On the other hand, fine-tuning cannot fully represent training-from-scratch and it is possible that some sources will have different effect between fine-tuning and training-from-scratch. The other downside is that fine-tuning generally gives a noisier signal, and may requires more observations. \sid{This sentence seems to contradict what we say above regarding the benefits of fine-tuning.} \notejinkun{Yes. Probably I should add "While in our experiments the benefit of fast training outweighs the noise issue."}

%\paragraph{Hyper-parameter tuning of warm-starting} \notejinkun{Maybe we should move this following paragraph to appendix? It is very subtle (can be regarded as a way to tune hyper-param)}
%In this section, we show how we implement the training schedule of warm-starting, namely the learning rate, batch size and the number of iterations \footnote{One iteration means one time of model parameters update}. This is more of an empirical question and there may be better alternatives than ours, so we just describe our implementation for readers who are interested. Further research may be needed to understand more about warm-starting to design better schedule.

%Basically our goal is to achieve convergence as quickly as possible.  When the original learning rate is chosen adaptively over the course of training like Adam \cite{kingma2017adam}, we keep the learning rate and batch size unchanged but only fine-tune for one epoch. Otherwise we choose the learning rate such that the validation accuracy drops by roughly 20\%, a not-too-large but still significant number. In addition, we vary batch size proportionally to the number of training examples included, such that each subset needs roughly the same number of iterations for iterating through one epoch. We fine-tune every model by roughly one epoch \footnote{Because we actually fine-tune a fixed number of iterations that amounts to one epoch on the full set.}. Moreover we lower bound the batch size since too small batch sizes tend to break the models.

%Specifically, let the unbounded batch size be $UBS=main\_batch\_size \times \frac{|S|}{n}$, where $main\_batch\_size$ is the batch size used to train the main model (assume each source has the same number of examples for simplicity) \footnote{Otherwise the numerator should be the total number of examples in all sources of $S$ and similar for the denominator.}. Then we sample a few subsets from $\mathcal{L}_\mathcal{P}$, fine-tuned models using $UBS$ and observe their model validation accuracy v.s. batch size. 
%In our experiments this exhibits a pattern of "slope-then-flat" pattern as in Fig. \ref{fig:bsvslr-cifar10-20-ft}. 
%So we set $\epsilon$ to the batch size at the turning point and bound the final batch size as $BS=\max(\epsilon, UBS)$. 
%Next the learning is picked such that the turning point roughly has an accuracy drop of 20\% compared to the main model. \notejinkun{Does this make sense?}

%\paragraph{Justification for the choice of learning rate} On the one hand, setting a large learning rate makes it faster and more aggressive in erasing the knowledge of other data and overfitting the subset, thus a large learning rate is favorable. On the other hand, too large a learning rate may totally break the starting model, making it no different than training-from-scratch and thus losing the benefits of warm-starting. So we pick 20\% as a tradeoff value.

%\paragraph{Justification for fixed number of iterations and scaling batch size} We find in experiments that when the batch size is fixed, the epochs needed for convergence tends to vary, but the number of iterations is more constant. Therefore we fix the number of iterations to that required for training for one epoch in the full dataset. \sout{To further speedup fine-tuning, we also scale the batch size proportionally to the subset size such that the epochs are as fixed as possible.} We further scale batch size proportionally to the number of training examples in the subset to ensure each training example is visited roughly once.

\subsection{Efficient \quantity{} Estimation}
\label{subsec:lasso}

When a query arrives, the online phase begins (step 3 in Algorithm \ref{alg:approach}).
%Given a query an input $Q_I$, and related target label $Q_L$, we wish to explain the score given by the main model to label $Q_L$ for input $Q_I$. In \quantity{} parlance, the utility $U(S) \triangleq M_S(Q_I)[Q_L]$.
To estimate $\textrm{AME}_i$ for each source $i$, we begin by collecting the signal $U(S)$ for all available subsets $S$, by feeding input $Q_I$ into each previously trained model $\mathcal M_S$, and collecting the score given by the model to label $Q_L$ (lines 25-27 in Algorithm \ref{alg:approach}).
(Note that our methodology can also be applied to sets of query inputs, and other utility metrics such as the accuracy on this set of inputs.)
There is a standard estimate for Eq.~\ref{eq:diff-in-means-p} that replaces the expectations with the empirical mean, which we call \emph{diff-in-means}, that is statistically sound but only achieves a rate of $O(n \log(n))$ for estimating all sources' \quantity{} (see Appendix \ref{appendix:diff-in-means}). Instead, we can leverage our sparsity assumption to achieve low $L_2$ error on all $\textrm{AME}_i$s together.
%
A key observation is that we can re-frame the estimation of all $\textrm{AME}_i$s as a specific linear regression problem, which can then be efficiently estimated under the sparsity assumption using LASSO, a regularized linear regression method.
%
%We next detail these two insights.

%After a set of subsets are drawn, we train one model on every subset $S$ and use it to predict on the query input to obtain $U(S)$, which will be later used by the estimation procedure detailed in this section.

%\subsubsection{Strawman: Diff-in-means \fixme{remove this subsubsection?}}
%By linearity of expectation, $AME_i$ can be re-written as 
%\begin{equation}
%    \mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim %\mathcal{L}^i_\mathcal{P}}[U(S^i)].
%\end{equation}
%A natural approach is then to estimate the two expectations separately by computing some means on the subsets drawn. Since our new sampling distribution is different from the original one defining $AME_i$, some \emph{adjustment} of the sample is needed to ensure consistency. To do so, if we denote by $S, S^i$ the random subset variable in the new and original distribution, respectively, we can adjust $S$ to be like $S^i$ by conditioning on $P$ and $i\notin S$:
%\begin{equation}
%    S^i | P \stackrel{d}{=} S | (P,i\notin S),
%\end{equation}
%where $\stackrel{d}{=}$ denotes equality in distribution. This is true since the $S^i$ or $S$ are both drawn according to $P$, and the only difference is that $S^i$ never includes $i$, which we fix by conditioning on $i\notin S$. Similarly:
%\begin{equation}
%    (S^i + \{i\}) | P \stackrel{d}{=} S | (P,i\in S),
%\end{equation}
%Therefore \notejinkun{Version 1}, 
%\begin{subequations}
%\label{eq:7}
%\begin{align}
%    &AME_i=\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)]\\
%    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})|P]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)|P]\right]\\
%    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\in S]-\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\notin S]\right]\label{eq:diff-in-means-true},
%\end{align}
%\end{subequations}
%Therefore \notejinkun{Version 2}, 
%\begin{subequations}
%\label{eq:7}
%\begin{align}
%    &AME_i=\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i+\{i\})]-\mathbb E_{S^i\sim \mathcal{L}^i_\mathcal{P}}[U(S^i)]\\
%    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S_P\sim S^i|P}[U(S_P+\{i\})]-\mathbb E_{S_P\sim S^i|P}[U(S_P)]\right]\\
%    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S_P\sim S|(P,i\in S)}[U(S_P)]-\mathbb E_{S_P\sim S|(P,i\notin S)}[U(S_P)]\right]\\
%    &=\mathbb E_{P\sim \mathcal P}\left[\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\in S]-\mathbb E_{S\sim\mathcal{L}_\mathcal{P}}[U(S)|P,i\notin S]\right]\label{eq:diff-in-means-true},
%\end{align}
%\end{subequations}
%\notejinkun{Which version is better? Also I may be abusing the notations here. Haven't figured out a good way to index expectation. \eg $\mathbb E_{P\sim \mathcal P}[\mathbb E_{S\sim \mathcal{L}_\mathcal{P}}[...]]$ is probably unreadable, and what I wanted to convey is that the expectation is taken over the new sampling scheme, and we do a iterated expectation on $P$, but keep in mind it is still on the new scheme (which is why I explicitly index $\mathbb E$ with $_{S\sim \mathcal{L}_\mathcal{P}}$).}%where we index expectation by ${\mathcal{L}_\mathcal{P}}$ to make it explicit that the expectation is taken over the new distribution $\mathcal{L}_\mathcal{P}$.should i write $\mathbb{E}_\mathcal{S\sim \mathcal{L}_\mathcal{P}}$ instead of $\mathbb E_{\mathcal{L}_\mathcal{P}}$ in the last line?}
% Denote by $f^i(S|P=p)$ and $f(S|P=p)$ the conditional distribution in $\mathcal{L}^i_\mathcal{P}$ and $\mathcal{L}_\mathcal{P}$ when $P=p$, respectively. Further denote by $f(S|P=p,i\in S)$ and $f(S|P=p,i\notin S)$ the conditional distribution in $\mathcal{L}_\mathcal{P}$ when $P=p$ and $i\in$ or $\notin S$. %Observe that the population $\mathcal{L}^i_\mathcal{P}$ can be induced by only taking those in $\mathcal{L}_\mathcal{P}$ that does not include $i$. Therefore $\mathbb E_{S\sim \mathcal{L}^i_\mathcal{P}}[U(S)]$

%Intuitively, Eq. \ref{eq:diff-in-means-true} calculates, for every $P$ value, the mean of $U$ when $i$ is included and $U$ when excluded, and then average their difference across every $P$ value. 

%Directly measuring using sample means leads to the \textbf{diff-in-means} approach, which we denote by $\widehat{AME}_i$:
%\begin{equation}
%    \label{eq:ame-diff-in-means}
%    \widehat{AME}_i=\frac{1}{b}\sum_{p\in\mathcal{P}} \widehat{\mathbb E}[U(S)|i\in S,P=p]-\widehat{\mathbb E}[U(S)|i\notin S,P=p],
%\end{equation}

%\paragraph{Disadvantages}
%\fixme{question: \notejinkun{how to frame this properly?}}Diff-in-means has not yet been proved to be sample efficienc when $n$ is large. In other words, it may not scale as $n$ increases.

\begin{figure}[t]
    \centering
     \begin{subfigure}{\columnwidth}
         \centering
         \includegraphics[width=\columnwidth]{fig/design_matrix.png}
     \end{subfigure}
    \caption{Regression design example for three sources and four values of $p$. The featurization functions $f_{in}(p) = \frac{1}{p}$ and $f_{out}(p)=-\frac{1}{1-p}$ represent included and excluded sources.}
    \label{fig:lasso_matrix}
\end{figure}

\mypara{Regression formulation} 
At a high level, computing $\textrm{AME}_i$ for a fixed $p$ (Eq. \ref{eq:diff-in-means}) is identical to fitting a linear regression with only variable $X_i$ for source $i$, encoded as $+1$ when the source is included in $S$ and $-1$ otherwise, on the outcome $Y=U(S)$.
Because all sources are assigned independently, sources do not ``interfere'' in the regression when added together, as long as the featurization ensures that each source is encoded with a mean value of zero.
Supporting different values of $p$ is a bit more subtle, as the different probabilities of source inclusion induce a variance weighted average between $p$s, while $\textrm{AME}_i$ is defined with equal weights for each $p$.
We counter-balance this variance weighting by re-scaling the features based on $p$.
Finally, we add a binary variable for each value of $p$, which de-means the signal within each $p$ value.

The resulting design matrix and outcome $(X, Y)$ is summarized in Figure \ref{fig:lasso_matrix}. Each row $j$ corresponds to a subset model with training data $S_j$ sampled with probability $p$. We have $Y_j=U(S_j)=\mathcal{M}_{S_j}(Q_I)[Q_L]$, and observation $X$ is composed of two groups of features. The first $n$ values, one for each data source, are encoded as $X_i = \frac{1}{p}$ if $i \in S_j$ and  $X_i = \frac{-1}{1-p}$ otherwise ($i \in [n]$). Second, $b=|\mathcal{P}|$ binary features are added that are all $0$, except for the variable corresponding to the sample value $p$, which has value $1$.
%
Under this regression design, we show the following result:

\begin{proposition}
\label{prop:regression-reduction}
Let $\beta^*$ be the best linear fit on $(X, Y)$:
\begin{equation}
\label{eq:best}
\beta^{*}=\underset{\beta \in \mathbb{R}^{n+b}}{\argmin}~\mathbb{E}\left[(Y-\left\langle \beta, X\right\rangle)^{2}\right],
\end{equation}
then $\textrm{AME}_i/v=\beta^*_i, \ \forall i\in[n]$, where $v=\mathbb{E}_{p \sim \cP}[\frac{1}{p(1-p)}]$. 
\end{proposition}
\begin{proof}
For a linear regression, we have (e.g. Eq. 3.1.3 of \cite{angrist2008mostly}):
\begin{equation*}
\beta^*_i=\frac{Cov(Y,\tilde X_i)}{Var[\tilde X_i]} ,
\end{equation*}
where $\tilde X_i$ is the regression residual of $X_i$ on all other covariates $X_{-i}=(X_1,\dots,X_{i-1}, X_{i+1},\dots, X_{n+b})$.
In our design $\mathbb E[X_i|X_{-i}]=\mathbb E[X_i|p]=0$, implying $\tilde X_i=X_i-\mathbb E[X_i|X_{-i}]=X_i$. Therefore:
\begin{equation*}
    \beta^*_i=\frac{Cov(Y,\tilde X_i)}{Var[\tilde X_i]}=\frac{Cov(Y,X_i)}{Var[X_i]}=\frac{\mathbb E[X_iY]}{Var[X_i]} .
\end{equation*}
Notice that $\mathbb E[X_iY] = \mathbb E_{p\sim \cP}[\mathbb E[X_iY|p]]$ with:
\begin{equation*}
\begin{aligned}
\label{eq:diy}
&\mathbb E[X_iY|p] = p\cdot\mathbb E[X_iY|p, i\in S]+(1-p)\cdot\mathbb E[X_iY|p, i\notin S]\\
& = p\frac{1}{p} \mathbb E[Y|p,i\in S]+(1-p)\frac{-1}{1-p}\mathbb E[Y|p,i\notin S]\\
& = \mathbb E[Y|p,i\in S]-\mathbb E[Y|p,i\notin S]
\end{aligned}
\end{equation*}
Combining the two previous steps yields:
\begin{equation*}
\begin{aligned}
\label{eq:diy2}
\beta^*_i = \frac{\mathbb E_{p \sim \cP}[\mathbb E[Y|p,i\in S]-\mathbb E[Y|p,i\notin S]]}{Var[X_i]} = \frac{AME_i}{Var[X_i]} .
\end{aligned}
\end{equation*}
% JK: Changing \cP to p as below
% Noticing that $Var[X_i]=\mathbb E[Var[X_i|\cP]]+Var[\mathbb E[X_i|\cP]]=\mathbb E[\frac{1}{\cP(1-\cP)}]$ concludes the proof.
Noticing that $Var[X_i]=\mathbb E[Var[X_i|p]]+Var[\mathbb E[X_i|p]]=\mathbb E[\frac{1}{p(1-p)}]$ concludes the proof.
\end{proof}

In words, solving the linear regression of $Y$ on $X$ with infinite data ensures that $\beta_i$, the linear regression coefficient associated with $X_i$, is the $\textrm{AME}_i$ we desire re-scaled by a known constant.
%
Of course, we do not have access to infinite data. Indeed, each row in this regression comes from training a model on a subset of the original data, so limiting their number is important for scalability. Ideally, this number would be smaller than the number of features (the number of data sources), even though this leads to an under-determined regression. Fortunately, we can still fit this under-determined regression by exploiting sparsity and LASSO. 

%\begin{itemize}
%\item Sample $P$, then sample subset $S$ according to $P$
%\item %$Y$ to be the confidence of predicting $L$ by the model trained on the subset $S$, i.e.
%Define response variable $Y=U(S)$
%\item Define covariates $X=(X_1,\dots,X_{n+b})$, with 
%\begin{equation*}
%    \begin{aligned}
%    &X_i =\mathbf 1_{i\in S}/P-\mathbf 1_{i\notin S}/(1-P) & i \in [n]\\
%    &X_{n+i} = \mathbf 1_{P=p_i} & i \in [1,b],
%    \end{aligned}
%\end{equation*}
%where $\mathbf 1_{cond}$ is the indicator function evaluates to $1$ when $cond$ is true and $0$ otherwise.
%\end{itemize}

%We create an observation $(X,Y)$ every time a subset $S$ and the corresponding $P$ are sampled. The response variable $Y$ is assigned with value $U(S)$. There are in total $n+b$ covariates, denoted by $X=(X_1,\dots,X_{n+b})$. The first $n$ are source covariates and bi-valuedly coded, each indicating for each source whether it is included in $S$ or not. The specific coding will be discussed later. The remaining $b$ are bucket covariates and zero-one coded, indicate which $P$ value is chosen. Finally, $Y$ is regressed on $X$ and the coefficient estimates of source covariates are our new estimators for $AME_i$ (modulo a constant factor $c_1=\mathbb E[\frac{1}{P(1-P)}]$).

%\sid{I would pitch the coding scheme issue below as a (non-major) technical challenge.}
%\paragraph{Coding scheme} Our first attempt is to use the usual zero-one coding, but that brings an issue of variance weighting, causing the estimator biased towards $P=0.5$. Formally, it estimates the other $AME_i$ defined as if $P$ is drawn from $\mathcal{P}$ with probability mass function $\mathbb P[P=p]=p(1-p)$. To address this issue, we use a coding scheme that assigns $X_i$ to $\frac{1}{p}$ when $i\in S$ and $\frac{-1}{1-p}$ otherwise. Besides countering the variance-weighting, it also has an important property of $\mathbb E[X_i|P]=0$ that simplifies the subsequent theoretical reasoning. 

%Besides adjusting coding scheme, one can also weight the observations according to $P$ when doing regression. On the other hand, this also suggests that by tuning the coding scheme/weighting of observations one can measure a different \quantity{} defined by a different distribution other than $\mathcal{L}_\mathcal{P}^i$.

%Notice that the observations can be divided into groups based on $P$ values. OLS can be interpreted as estimating $AME$ of each group and then average the results. However, OLS uses variance-weighted average that puts the most weight on the group with largest variance of $X_i$, making the estimation biased towards th. To counter this variance-weighting effect, we design an \text{inverse-propensity} coding that ensures 

%\paragraph{Overall formulation}
%In summary, the sampling procedure is as follows:

% \paragraph{Consistency and Finite-sample error bound of $\hat l_{lasso}$}
%\paragraph{Equivalence between AME estimation and regression, and the finite-sample error bound of $\hat l_{lasso}$ estimators}
%We will show that for some constant $c_1$, $\|\hat{l}_{lasso,1:n}-\bold{AME}/c_1\|_p \leq O(k^\frac{1}{p} \sqrt{\log(n)/m})$ with high probability. \notejinkun{Not sure if this is precise?} We first proof that our regression formulation has the true solution $l^*$ equal to $\bold{AME}/c_1$ under infinite sample, and then proof that $\hat l_{lasso}$ is close to $l^*$ in large sample with high probability.

%\begin{proposition}
%Let $l^*$ be the best linear approximation, i.e.
%\begin{equation}\label{eq:best}l^{*}\in\underset{l \in \mathbb{R}^{n+b}}{\argmin}~ \mathbb{E}\left[(Y-\left\langle l, X\right\rangle)^{2}\right],\end{equation}
%then $AME_i/c_1=l^*_i, \forall i\in[n]$, where $c_1=Var[X_i]=\mathbb{E}[\frac{1}{P(1-P)}]$. 
%\end{proposition}
%\begin{proof}
%By REGRESSION ANATOMY introduced in Equation 3.1.3 of \cite{angrist2008mostly}, \begin{equation}l^*_i=\frac{Cov(Y,\tilde X_i)}{Var[\tilde X_i]},\end{equation} where $\tilde X_i$ is the regression residual of $X_i$ on all the other covariates $X_{-i}=(X_1,\dots,X_{i-1}, X_{i+1},\dots, X_{n+b}).$ Since $\mathbb E[X_i|X_{-i}]=\mathbb E[X_i|P]=0$ is a linear function, $\tilde X_i=X_i-\mathbb E[X_i|X_{-i}]=X_i.$ Therefore,
%\begin{equation*}
%    l^*_i=\frac{Cov(Y,\tilde X_i)}{Var[\tilde X_i]}=\frac{Cov(Y,X_i)}{Var[X_i]}=\frac{\mathbb E[X_iY]}{Var[X_i]}
%\end{equation*}
%It follows that 
%\begin{equation*}
%\begin{aligned}
%\label{eq:diy}
%&\mathbb E[X_iY|P=p]\\
%={}&\sum_{t=0}^1\mathbb P[\mathbf 1_{i\in S}=t|P=p]\cdot\mathbb E[X_iY|\mathbf 1_{i\in S}=t,P=p]\\
%={}&p\cdot\mathbb E[X_iY|P=p,  i\in S]+(1-p)\cdot\mathbb E[X_iY|P=p,  i\notin S]\\
%={}&p\frac{1}{p} \mathbb E[Y|P=p,i\in S]+(1-p)\frac{-1}{1-p}\mathbb E[Y|P=p,i\notin S]\\
%={}&\mathbb E[Y|P=p,i\in S]-\mathbb E[Y|P=p,i\notin S]
%\end{aligned}
%\end{equation*}
%Thus 
%\begin{equation*}
%\begin{aligned}
%\label{eq:diy}
%l^*_i&=\frac{\mathbb E[X_iY]}{Var[X_i]}=\frac{\mathbb E_{P\sim \mathcal{P}}[\mathbb E[X_iY|P]]}{Var[X_i]}\\
%&=\frac{\mathbb E_{P\sim \mathcal{P}}[\mathbb E[Y|P,i\in S]-\mathbb E[Y|P,i\notin S]]}{Var[X_i]}\\
%&=\frac{AME_i}{Var[X_i]}  ~~ (\text{by Eq. \ref{eq:7}})
%\end{aligned}
%\end{equation*}
%Finally, 
%\begin{equation*}
%    Var[X_i]=\mathbb E[Var[X_i|P]]+Var[\mathbb E[X_i|P]]=\mathbb E[\frac{1}{P(1-P)}]
%\end{equation*}
%\end{proof}


\mypara{Efficient estimation with LASSO}
To improve our sample efficiency and require fewer subset models for a given number of data sources $n$, we leverage our sparsity assumption and recent results in high dimensional statistics.
Specifically, we use a LASSO estimator, which is a linear regression with an $L_1$ regularization:
\begin{equation*}
    \hat{\beta}_{lasso}=\underset{\beta \in \mathbb{R}^{n+b}}{\argmin} \left( \left(Y-\left\langle \beta, X \right\rangle\right)^{2}+\lambda \|\beta_{1:n}\|_{1}\right).
\end{equation*}
%where $l_{1:n}=(l_1,\dots,l_n)$ and $\lambda>0$ is a hyper-parameter chosen through cross-validation.
LASSO is sample efficient when the solution is sparse \cite{lecue_regularization_2017}. Recall that $k$ is the number of non-zero $\textrm{AME}_i$ values, and let $m$ be the number of subset models. Our reduction to regression in combination with result on LASSO's signal recovery lead to the following proposition:
\begin{proposition}
The exists a value $C(\delta)$ such that with probability at least $1-\delta$:
\begin{align*}
\|\hat{\beta}_{lasso,1:n}-\frac{\textbf{AME}}{v}\|_2 \leq C(\delta) \sqrt{\frac{k\log(n)}{m}} ,
\end{align*}
with $v=\mathbb{E}_{p\sim \cP}[\frac{1}{p(1-p)}]$.
\end{proposition}
\begin{proof}
From Proposition \ref{prop:regression-reduction}, we know that $\frac{\textrm{AME}}{v}$ is the best linear estimator of the regression of $Y$ on $X$.
Our sparsity assumption ensures that we can apply Theorem 1.4 from \cite{lecue_regularization_2017}, which directly yields the error bound.
\end{proof}

As a result, LASSO can recover all $\textrm{AME}_i$s with low $L_2$ error using $O(k\log(n))$ subest models. Eliminating a linear dependence on the number of data sources is crucial for scaling our approach to large datasets, and an important improvement over existing work, including Shapley values \cite{jia_towards_2020}.


% : LASSO has a scalable error bound of $O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2]$ where $m$ denotes the sample size, suggesting that only $O(k\log n)$ of sample points are required.


%we start from a very different angle. Recalling that our final problem is to identify a sparse group, and this suggests a well-known variable selection technique called LASSO, which is essentially linear regression with L1 regularization. It has been proven that LASSO is very good at selecting a sparse set and recent paper \cite{lecue_regularization_2017} suggests a scalable finite-sample error bound between LASSO coefficients and the best linear approximation.

%\begin{proposition}
%With high probability $\|\hat{l}_{lasso}-l^*\|_p\leq O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2]$.
%\end{proposition}
%\begin{proof}
%TBD \notejinkun{This is where we should use the small ball paper. But I remember there is a problem with unpenalized bucket variables.}
%\end{proof}
%\begin{corollary}
%With high probability $\|\hat{l}_{lasso,1:n}-\bold{AME}/c_1\|_p\leq O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2], c_1=Var[X_1]=\dots =Var[X_n]=\mathbb E[\frac{1}{P(1-P)}]$.
%\end{corollary}



%Therefore we formulate the problem into variable selection and show that in hindsight the LASSO coefficients turn out to be a consistent estimator of $AME_i$ modulo a constant factor. We utilize \cite{lecue_regularization_2017} to show that it has a better error bound of $O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2]$, suggesting that only $O(k\log n)$ of sample points are required. 

%\notejinkun{version 2 of the previous two paragraphs}
%To have a better sample efficiency that scales with $n$, we propose to formulate the estimation into a regression problem where every $AME_i$ corresponds to one of the coefficients, and now estimating the $AME_i$s is equivalent to estimating the coefficients. By reducing to regression, we can utilize the rich literature on efficient estimation for regression. Among them is LASSO, which is essentially regression with L1 regularization, but is shown to be very efficient when the solution is sparse \cite{lecue_regularization_2017}: LASSO has a scalable error bound of $O(k^\frac{1}{p} \sqrt{\log(n)/m})$, $p \in [1, 2]$ where $m$ denotes the sample size, suggesting that only $O(k\log n)$ of sample points are required.



% On the one hand, the $AME_i$ is a well known concept termed \emph{Average Treatment Effect} in the field of causal inference and sometimes estimated through regression \cite{imbens_causal_2015, egami_causal_2019} \footnote{diff-in-means gives the same result as regression and sometimes people favor regression given its popularity, cf. Chapter 7 of \cite{imbens_causal_2015}.}. On the other hand, LASSO is often used together with regression when people want to select a sparse set of covariates. Moreover, recent paper \cite{lecue_regularization_2017} suggests that LASSO guarantees a good finite-sample error bound. Note that there are also works in causal inference using LASSO, but they do it in a slightly different way, making it hard to utilizing the finite-sample error bound. Therefore, we propose a novel formulation of regression with    with LASSO for estimation as well as proponent group selection.
% , though most of them are focused on measuring for one single treatment (i.e. source in our case) \fixme{CITE}. There are works for multiple treatments, but  or mak

\subsection{Controlling False Detections}
\label{subsec:knockoffs}
Given the estimates of all $AME_i$s measured with LASSO on a set of subset models, we need to select those sources that we can confidently claim belong to the proponent group.
This is typically done by choosing a threshold $t$ over which we deem the $AME_i$ value significant, where $t$ must be chosen carefully.
%
A practical objective in choosing $t$ is to maximize the number of selected sources while ensuring that we make as few wrong selections as possible, to avoid drowning the signal of proponents in a large number of false positives.
%
Formally, let $\hat S_+$ be the sources selected and $S_+$ be the true set of proponents, then we can quantify the selection through $\textrm{\emph{precision}} \triangleq \frac{|\{i \in \hat{S}_+ \cap S_+ \}|}{|\hat{S}_+|}$ and $\textrm{\emph{recall}} \triangleq \frac{|\{i \in \hat{S}_+ \cap S_+ \}|}{|S_+|}$.
%, defined as follows: 
%\begin{equation*}
%\begin{aligned}
%    &precision&=\frac{|\{i \in \hat{S}_+ \cap S_+ \}|}{|\hat{S}_+|},
%\\
%    &recall&=\frac{|\{i \in \hat{S}_+ \cap S_+ \}|}{|S_+|}
%\end{aligned}
%\end{equation*}
%with $precision=1$ when its denominator is 0.
%We emphasize that the above definitions are all one-sided, \ie only treating selecting proponents as correct, but not opponents, which differs from the common definitions (\eg as in \cite{candes_panning_2017}) that treats selecting opponents as correct as well.
%Thus a power selection corresponds to high recall and conservative corresponds to high precision.
%Define the false discovery proportion (FDP) as $FDP=1-\textrm{precision}$, and the 
% We define the \emph{false discovery proportion} (FDP) as $1-precision$ and \emph{false discovery rate} (FDR) as $\mathbb E[FDP]$.
We define the \emph{false discovery rate} (FDR) as $\mathbb E[1-precision]$.

To select as many sources as possible while controlling the FDR to a given target level, we leverage the Model-X (MX) Knockoff framework \cite{candes_panning_2017}.
For each feature $X_i$ representing a data source in LASSO, we create a knockoff feature sampled independently from the same distribution conditioned on other features (in our case the features encoding $p$), by running the assignment procedure from \S\ref{subsec:sampling}.
Because knockoff features do not influence the data the subset models are trained on, they are independent of $Y$ by design. The knockoff features for each $X_i$ are added to the LASSO design matrix, such that each feature and each knockoff receives a coefficient.

We then compare each data source coefficient $\hat\beta_i$ to the corresponding knockoff coefficient $\beta'_i$ to compute $W_i$:
\[
W_i \triangleq \max(\hat\beta_i, 0) - \max(\beta'_i, 0) .
\]
$W_i$ is positive when $\hat\beta_i$ is large compared to its knockoff---a sign that the data source significantly and positively affects $Y$, which is the definition of a proponent---and negative otherwise.

Finally, we compute the threshold $t$ such that 
%\sout{the fraction of selected knockoff features is bellow the desired FDR $q$:}
the estimated value of $1-precision$ is below the desired FDR $q$:
\begin{equation*}
t=\min \left\{\tau>0: \frac{\#\left\{i: W_{i} \leq-\tau\right\}}{\#\left\{i: W_{i} \geq \tau\right\}} \leq q\right\},
\end{equation*}
and select data sources with a $W_i$ above this threshold. We use $\hat S_+$ to denote selected sources.% as $\hat S_+$.
% \notepanda{Following equation seems unnecessary, given the description says exactly the same thing.}
% \begin{equation*}
%     \hat S_+=\{i:W_i\geq t\} .
% \end{equation*}
Effectively, we select features based on their LASSO coefficient, until the ratio of knockoffs we select is higher than the FDR we do not wish to exceed. Because we know that knockoff features are independent of $Y$ by design, in expectation we cannot select too many uncorrelated true features before selecting too many knockoffs, which controls the FDR.

Formally, this knockoff procedure provably controls the following relaxation of FDR~\cite{candes_panning_2017} :
%
\begin{equation*}
\label{eq:mFDR}
mFDR=\mathbb{E}\left[\frac{\left|\left\{i \in (\hat{S}_+ \cap S_+) \right\}\right|}{|\hat{S}_+|+1 / q}\right] \leq q.
\end{equation*} 
Though not controlling the true $FDR$, it is still useful since $mFDR$ differs from $FDR$ only in the extra $1/q$ in the denominator.
%
There exists a knockoff variation controlling the exact FDR, but this relaxed guarantee works better when there are few proponents, and still efficiently controls the FDR in our experiments (\S\ref{sec:eval}).
%
We also note that our knockoff statistic is different from the traditional one, which uses $W_i = |\hat\beta_i| - |\beta'_i|$. This is because we focus on selecting proponents and ignoring opponents. Technically, this means that we control FDR for both opponents and proponents, and control the ratio of selected neutral sources. However, since opponents are such that $\max(\beta_i, 0) = 0$, we are extremely unlikely to select them (even less than neutral sources). 
%It is possible that our approach controls the FDR for proponents only, similarly to signed FDR control \cite{10.1214/18-AOS1755}, but we leave such an analysis for future work.


%\notejinkun{does the following paragraph make sense?} We apply a framework called Knockoffs \cite{candes_panning_2017} in choosing $t$. Knockoffs aim to select the variables not independent of an outcome variable from many variables, with the guarantee to bound the expected precision to be at least a given value. This offers some form of guarantee of the selection quality, and also gives users flexibility to choose $t$ based on their precision requirement. Back to our case, $X_i$ is independent of $Y$ for neutrals while not independent for proponents and opponents. This suggests that we can apply Knockoffs to select the non-neutrals with precision control. This is, however, not exactly the goal we want to achieve; instead, we only want to select the proponents. Therefore, we slightly modify the procedure to adapt into our case. 

%\paragraph{The technique} The technique requires to generate one "knockoff" covariate for each of the original ones, and fit the estimation model (\ie LASSO here) on both the knockoff and original covariates. By comparing between the statistics of the knockoff and original covariates, the procedure can compute a threshold bounding the FDR. 

% However, the original Knockoffs is controlling a two-sided FDR that does not count selecting an opponent as an error. Thus we slightly modify the procedure into a one-sided version. Due to limit of effort, we only validate its effectiveness through the empirical evaluation, but leave the formal proof for future work. \notejinkun{OK to say so?}

%Specifically, when running the subset sampling and LASSO, we pretend as if there are $2n$ sources with the first $n$ being original sources and last $n$ being knockoff ones that contain no data. Let's term the covariates of the original sources $D=(D_1,\dots,D_n)$ and covariates of the knockoff ones $\tilde{D}=(\tilde D_1, \dots,\tilde D_n)$. %The goal is to create variables (i.e. $\tilde{D}$) that we know for sure are independent of $Y$ and thus should not be selected. This serves as a reference for further reasoning about which original sources should not be selected. %the same distribution as $D_i$ for $i=0,\ldots,n-1$. 

%Next, given a target FDR level $q$, we pick a threshold $\tau$ by setting\footnote{Per footnote of \cite{candes_panning_2017}: $\min \{t > 0 : \dots\}$ actually means $\min \{t \in W_+ : \dots \}$, where $W_+ = \{|W_i| : |W_i| > 0\}$}
%\begin{equation}
%\tau=\min \left\{t>0: \frac{\#\left\{i: W_{i} \leq-t\right\}}{\#\left\{i: W_{i} \geq t\right\}} \leq q\right\},
%\end{equation}
%where $W_i=\max(\hat l_i,0)-\max(\hat l_{i+n},0)$. $\tau=+\infty$ if the set upon which $\min$ is taken is empty. Finally, the procedure selects the sources
%\begin{equation*}
%    \hat S_+=\{i:W_i\geq \tau\}
%\end{equation*}

%With some assumption (discussed shortly), the procedure controls a modified FDR defined below
%\begin{equation}
%\label{eq:mFDR}
%mFDR=\mathbb{E}\left[\frac{\left|\left\{i \in (\hat{S}_+ - S_+) \right\}\right|}{|\hat{S}_+|+1 / q}\right] \leq q.
%\end{equation} 
%Though not controlling the true $FDR$, it is still useful since $mFDR$ differs from $FDR$ only in the extra $1/q$ in the denominator. \footnote{The Knockoffs paper also provides a variant called \emph{Knockoffs+} that controls $FDR$, which we are not using since we expect there are very few proponents in which case Knockoffs+ would be too conservative and selects very few sources.}

%Overall, the pseudo code of LASSO+Knockoffs is shown in Algo. \ref{algo:k1}.
%\paragraph{Difference compared to original Knockoffs} Note that the original Knockoffs is controlling a "two-sided" FDR that does not count selecting an opponent as an error, which is different from our "one-sided" version. Thus we slightly modified the procedure as follows: in assigning $W_i$, they use $W_i=|\hat l_i|-|\hat l_{i+n}|$, but we instead use $W_i=\max(\hat l_i,0)-\max(\hat l_{i+n},0)$. The intuition is that the opponents would probably have $l_i\leq 0$, different from a neutral which would probably be $\hat l_i=0$. Taking a $\max(\cdot,0)$ makes opponents behave more similar to neutrals, and thus makes two-sided FDR closer to one-sided FDR, enabling us to directly apply original Knockoffs that controls the two-sided FDR onto the one-sided FDR. \notejinkun{Is the following statement correct?} More precisely, if we assume $\max(\hat l_i,0)$ has the same distribution for both opponents and neutrals, the procedure will control the $mFDR$ correctly. Otherwise, further analysis is needed, but due to limit of effort, we only validate its effectiveness through the empirical evaluation, but leave the formal proof for future work. \notejinkun{OK to say so?}



% \begin{proposition}
% Assume that $AME_i=0$ for any source $i$ that is neither proponent or opponent. Then the above threshold controls a modified FDR defined as
% \begin{equation}
% \label{eq:mFDR}
% mFDR=\mathbb{E}\left[\frac{\left|\left\{j \in (\hat{S}_+ - S_+) \right\}\right|}{|\hat{S}_+|+1 / q}\right] \leq q,
% \end{equation}
% where $S_+$ denotes the true proponent group.
% \end{proposition}
% %Now we claim $\tilde D$ is the Knockoffs of $D$. 
% \begin{proof}
% TBD \notejinkun{probably this proposition is wrong...}
% For this to be true, according to the Knockoff paper\cite{candes_panning_2017}, 2 properties must be satisfied: \emph{(1) for any subset $S \subset\{0, \ldots, n-1\}$,
% $$
% (D, \tilde{D})_{\operatorname{swap}(S)} \stackrel{d}{=}(D, \tilde{D})
% $$
% (2) $\tilde{D} \perp Y | D$  if there is a response  $Y$.}

% Above, the vector $(D, \tilde{D})_{\operatorname{swap}(S)}$ is obtained from $(D, \tilde D)$ by swapping the entries $D_j$ and  $\tilde D_j$ for each
% $j \in S$. (1) is guaranteed since each $D_i$ and $\tilde D_i$ are independently assigned. (2) is also guaranteed since $\tilde D$ constructed without looking at $Y$. Therefore, $\tilde D$ is the knockoffs of $D$.
% \end{proof}

%\sid{I agree that we should have one main algorithm in pseudocode that summarizes our methodology. What we have below is a good start.}

%\sid{I'm not sure I derived much value from Algorithm 2 (FDR stuff); we might just state it in a couple of sentences.}

% \begin{algorithm}[h]
% \DontPrintSemicolon
% \SetKwFunction{Fselect}{select}
% %  \Fn(\tcp*[f]{select non-null features with FDR under control}){\Fselect{$\hat l, q$}}{
%   \KwIn{$\hat l$, the LASSO coef of size $2n$}
%   \KwIn{$q$, the target FDR level}
%   $W \gets zeros(n)$\tcp*[r]{statistics}
%   \For{$i\gets1$ \KwTo $n$}{
%   $W_i=\max(\hat l_i,0)-\max(\hat l_{i+n},0)$\;
%   }
%   $\tau \gets \min \left\{t>0: \frac{\#\left\{i:W_{i} \leq-t\right\}}{\#\left\{i:W_{i} \geq t\right\}} \leq q\right\}$\tcp*[r]{find the threshold given the desired FDR}
%   $\hat S_+ \gets \{\}$\;%\tcp*[r]{non-null features (or data sources) indices}
%   \For{$i\gets1$ \KwTo $n$}{
%   \lIf{$W_i\geq\tau$}{$\hat S_+\gets \hat S_++\{i\}$}
%   }
%   \KwRet{$\hat S_+$}
% %  }
%  \caption{FDR-controlled feature selection\label{algo:k2}}
% \end{algorithm}


%\subsection{Training Optimization -- Warm-Starting}
%\label{subsec:warm-starting}
%\sid{Some of the details in the "Implementation" section could be moved here. With fine-tuning, I think its fine to describe our methodology for doing the training itself, which may include details such as what hyperparameters and training schedule we used.}

%\notepanda{Isn't this an optimization for both Lasso and ``Diff in Means''?}\notejinkun{Yes, it is. So should I put it after knockoffs?}
%Training of models is costly, especially for large models. Thus we further propose to use warm-starting as a proxy of original full training when there is not enough computation budget. The idea is that instead of training a model from scratch, we only fine-tune starting from the main model (\ie the model deployed by Alice if in the running example) for some number of iterations. Moreover, we design the grid $\mathcal{P}$ specifically to only cover the lower half range (i.e. $P\leq0.5)$ based on our observations in experiments.\sid{This seems ad-hoc, but I think we have justification elsewhere we can borrow from.} We call this approach \emph{warm-starting} or \emph{fine-tuning} interchangeably\sid{Let's pick one}, and refer to the original approach as \emph{training-from-scratch}.

%\paragraph{Justifying using only lower half range of $P$} What we find in experiments is that very low $P$s are the most helpful at distinguishing between proponents and opponents. For example, in Fig. \ref{fig:diff-in-means}, $P=0.01$ or $0.1$ work well in warm-starting. The reason is probably that low $P$s make it more likely to sample a subset without any proponent, in which adding one proponent will significantly elevate the signal $U(\cdot{})$. This does not happen in training-from-scratch probably because (a) too few data are insufficient to train a reasonable model; (b) it is much easier to maintain what has been learned than learning from scratch, thus one single source is able to pull up the signal in warm-starting while not in training-from-scratch \sid{This point is a bit counter-intuitive and needs some explanation}. In experiment we use $\mathcal{P}=\{0.01, 0.1, 0.2, 0.3, 0.4, 0.5\}$ and it works well. We still include up to $0.5$ to cover the case of $k=1$. In the case where there are not many sources in total we remove $0.01$ to avoid the distribution deviation problem. \notejinkun{Does this justification make sense? If not, how should we justify?}.

%\paragraph{Advantages} Warm-starting generally helps the convergence, because the starting model is already converged in the whole dataset. The rest is only to transfer it into the subset, and is likely faster. Although it may not produce exactly the same result as training-from-scratch, the numbers are still comparable, suggesting that it can still be used to measure the supportive-ness and thus is a reasonable substitute for the original $U(\cdot)$. Moreover, warm-starting enables tiny $P$s \sid{This needs another line of explanation}. Besides the reason given in the justification above, the other reason is that the whole dataset has already been learned and we could worry less about the distribution deviation problem discussed in Sec. \ref{sec:p-pop}. \notejinkun{Probably the insufficient data problem in group testing could also be handled this way.} However, that is not to say we can never worry about that and pick extremely tiny $P$.

%\paragraph{Disadvantages} On the other hand, fine-tuning cannot fully represent training-from-scratch and it is possible that some sources will have different effect between fine-tuning and training-from-scratch. The other downside is that fine-tuning generally gives a noisier signal, and may requires more observations. \sid{This sentence seems to contradict what we say above regarding the benefits of fine-tuning.} \notejinkun{Yes. Probably I should add "While in our experiments the benefit of fast training outweighs the noise issue."}

%\paragraph{Hyper-parameter tuning of warm-starting} \notejinkun{Maybe we should move this following paragraph to appendix? It is very subtle (can be regarded as a way to tune hyper-param)}
%In this section, we show how we implement the training schedule of warm-starting, namely the learning rate, batch size and the number of iterations \footnote{One iteration means one time of model parameters update}. This is more of an empirical question and there may be better alternatives than ours, so we just describe our implementation for readers who are interested. Further research may be needed to understand more about warm-starting to design better schedule.

%Basically our goal is to achieve convergence as quickly as possible.  When the original learning rate is chosen adaptively over the course of training like Adam \cite{kingma2017adam}, we keep the learning rate and batch size unchanged but only fine-tune for one epoch. Otherwise we choose the learning rate such that the validation accuracy drops by roughly 20\%, a not-too-large but still significant number. In addition, we vary batch size proportionally to the number of training examples included, such that each subset needs roughly the same number of iterations for iterating through one epoch. We fine-tune every model by roughly one epoch \footnote{Because we actually fine-tune a fixed number of iterations that amounts to one epoch on the full set.}. Moreover we lower bound the batch size since too small batch sizes tend to break the models.

%Specifically, let the unbounded batch size be $UBS=main\_batch\_size \times \frac{|S|}{n}$, where $main\_batch\_size$ is the batch size used to train the main model (assume each source has the same number of examples for simplicity) \footnote{Otherwise the numerator should be the total number of examples in all sources of $S$ and similar for the denominator.}. Then we sample a few subsets from $\mathcal{L}_\mathcal{P}$, fine-tuned models using $UBS$ and observe their model validation accuracy v.s. batch size. 
%In our experiments this exhibits a pattern of "slope-then-flat" pattern as in Fig. \ref{fig:bsvslr-cifar10-20-ft}. 
%So we set $\epsilon$ to the batch size at the turning point and bound the final batch size as $BS=\max(\epsilon, UBS)$. 
%Next the learning is picked such that the turning point roughly has an accuracy drop of 20\% compared to the main model. \notejinkun{Does this make sense?}

%\paragraph{Justification for the choice of learning rate} On the one hand, setting a large learning rate makes it faster and more aggressive in erasing the knowledge of other data and overfitting the subset, thus a large learning rate is favorable. On the other hand, too large a learning rate may totally break the starting model, making it no different than training-from-scratch and thus losing the benefits of warm-starting. So we pick 20\% as a tradeoff value.

%\paragraph{Justification for fixed number of iterations and scaling batch size} We find in experiments that when the batch size is fixed, the epochs needed for convergence tends to vary, but the number of iterations is more constant. Therefore we fix the number of iterations to that required for training for one epoch in the full dataset. \sout{To further speedup fine-tuning, we also scale the batch size proportionally to the subset size such that the epochs are as fixed as possible.} We further scale batch size proportionally to the number of training examples in the subset to ensure each training example is visited roughly once.


\section{Hierarchical Design Extension}
\label{sec:hier}
Our methodology enables an interesting extension that can leverage naturally occurring hierarchical structure in data.
%For instance, such structure happens when users contribute data, and we may want to explain predictions at the level of an entire user's contribution, or each specific data point within a user.
%
%Our methodology can leverage data hierarchies 
By adapting the sampling, LASSO, and knockoffs designs, we can support proponent detection at each level of the hierarchy from a single set of subset models.
%
We describe our hierarchical extension for a two level hierarchy, in which $n_2$ second-level data sources (e.g., reviews contributed by users) are grouped into $n_1$ top-level sources (e.g., users). 

Three steps of our methodology require small changes. First, we sample sources into the subset models following the hierarchy. In a given data subset $S$, each top-level source is included independently with probability $p_1$, and each second-level source of an included top-level source is included with probability $p_2$.

Second, we adapt the design matrix and LASSO estimation based on the level at which we want to perform the detection.
%
We start by finding top-level proponents only, running the exact same procedure with $n=n_1$ sources and $p=p_1$ (with identical knockoffs) to obtain top-level proponent sources $\hat S_1$.
%
To detect proponents at the second level of the hierarchy, the design matrix $X$ includes the same variables as the first stage (top-level sources), as well as variables for each second-level source within the sources in $\hat S_1$, featurized as:
\begin{equation}
\label{eq:knockoff-featurization}
  X_i=\begin{cases}
    \frac{1}{p_1 p_2} & \text{if} \ pa(i) \in S_1 \ \text{and} \ i \in S_2\\
    -\frac{1}{p_1(1-p_2)} & \text{if} \ pa(i) \in S_1 \ \text{and} \ i \notin S_2\\
    0 & \text{otherwise}
  \end{cases}
\end{equation}
Where $pa(i)$ denotes the parent node of data point $i$, $S_1$ is the set of included top-level sources, and $S_2$ is the set of included second-level sources. Finally, as in the single level regression formulation, a binary feature is added for each possible $(p_1, p_2)$, with a $1$ value indicating each subset model's value tuple.
The featurization of second level source features has the nice property that $E[X_i|X_{-i}]=E[X_i|p_1,p_2,X_{pa(i)}]=0$, yielding a similar interpretation as Proposition \ref{prop:regression-reduction} for the hierarchical design.
%
Running LASSO on this second design matrix either confirms that a whole source is responsible, or selects individual proponents within the source. Note that both analyses run on the \emph{same set of subset models}: thanks to our hierarchical sampling design, the same offline phase supports all levels of the source hierarchy.

Third, we adapt the knockoffs in the second level regression. Since top-level sources were already selected, we only associate knockoff variables to features representing second level sources. Because knockoffs need to follow the distribution of the original feature conditioned on every other feature, we condition on the parent source. That is, the knockoff is sampled for inclusion with probability $p_2$ only when the parent source is included, and the whole feature is then featurized according to Equation \ref{eq:knockoff-featurization}.

As we show in \S\ref{sec:eval}, such a hierarchical scheme has multiple benefits. First, when higher levels in the hierarchy have fewer sources, and fewer proponents, it is possible to successfully detect proponent at these levels even when there are too few subset models to detect them at the lower levels of the hierarchy. This provides graceful degradation for the detection.
%
Second, when proponents are clustered in higher level sources (e.g. a few users contribute many proponents each), the first levels of the hierarchy are used to filter out candidate sources at the lower levels, making detection even at the lowest level more efficient, and requiring fewer subset models.
%
Third, the smaller design matrix at the lower level of the hierarchy also yields lower running times for LASSO.


%\noteanqi{List the possible experiments/comparisons to do:} \fixme{TO DO}
%Advantages of hierarchy:\\
%1. Graceful degradation: can select first-level when data is not enough.\\
%--experiment and draw graph: vary \#observations, show prec/rec of both levels\\
%--also here can compare the performance with non-hier: for the same \#obs, draw prec/rec for hier-top-level, hier-lower-level, non-hier.\\ 1) If the prec/rec for hier-lower-level is slightly worse than non-hier, then it will be a disadvantage for hierarchy or we can phrase our text to be a tradeoff, since it will be noisier?\\ 2). If for same \#obs, hier-top-level and hier-lower-level are both higher than non-hier (I guess so, especially for same \#obs), then it will show like kind of "optimization" in \#models needed.\\
%(mention again, although now the prec/rec of hier-lower-level is slightly worse than non-hier, but its \#obs is much less: 635 vs 2475 for hier vs non-hier. In non-hier case, for roughly 635 obs, the prec/rec is pretty bad..)\\
%2. Compare the lasso time for hier-lower-level and non-hier (for same \#obs): hier-lower-level may be faster since the matrix will be smaller. But I'm not sure it will be a very huge difference.\\
%--if we also consider the offline time, then it has a great advantage (still \#models needed thing).\\
%3. Furthermore on point-1, if for same \#obs hier-lower-level has better prec/rec than non-hier (or same thing, achieving a good prec/rec, hierarchy needs less \#models), then we say hierarchy improves the resources usage (less memory for models,...)



==> rm/hier-coding.tex <==
\section{Thoughts on Hierarchical Design's Coding Scheme}
\fixme{@Mathias}
Originally, for a second level source $i$,
$$X_i=\frac{1}{P_1P_2}|\frac{-1}{1-P_1P_2}$$
Use $pa(i)$ to denote the parent source of the second-level source $i$, $S_1, S_2$ to denote the sources included for first and second levels. The CEF is no longer 0, since
\begin{equation*}
  \begin{split}
    & E[X_i|X_{-i}]=E[X_i|P_1,P_2,X_{pa(i)}]=\\
    & \begin{cases}
      \frac{P_2}{P_1P_2}-\frac{1-P_2}{1-P_1P_2} & pa(i) \in S_1 \\
      -\frac{1}{1-P_1P_2}& pa(i) \notin S_1
    \end{cases}
  \end{split}
\end{equation*}
\paragraph{Patch 1}We can fix it by coding this way:
\begin{equation}
  \label{eq:code-v1}  
  X_i=\begin{cases}
    \frac{1}{P_2} & pa(i) \in S_1 \wedge i \in S_2\\
    \frac{-1}{1-P_2} & pa(i) \in S_1 \wedge i \notin S_2\\
    0 & \text{otherwise}
  \end{cases}
\end{equation}
$$E[X_i|X_{-i}]=E[X_i|P_1,P_2,X_{pa(i)}]=0$$
AME should (ideally) treat each $p=p_1p_2$ with equal weights. But Eq.~\ref{eq:code-v1} imposes an extra $p_1$ factor on the averaging. To see why, we can study the coefficient of $i$,
\begin{equation*}
\begin{split}
    Var[\tilde{X}_i]\beta^*_i= Cov(\tilde{X}_i, Y)=Cov(X_i,Y)\\
    =\mathbb E[X_iY]=\mathbb E[\mathbb E[X_iY|P_1,P_2,X_{pa(i)}]]
\end{split}
\end{equation*}$\mathbb E[X_iY|P_1,P_2,X_{pa(i)}]=0$ when $X_{pa(i)}$ indicates $pa(i) \notin S_2$, otherwise,
\begin{equation*}
  \begin{split}
    & \mathbb E[X_iY|P_1,P_2,X_{pa(i)}]=\mathbb E[X_iY|P_1,P_2,pa(i)\in S_1]\\
    ={}&P_2\frac{1}{P_2}\mathbb E[Y|P_1,P_2,pa(i)\in S_1,i\in S_2]\\
    &+(1-P_2)\frac{-1}{1-P_2}\mathbb E[Y|P_1,P_2,pa(i)\in S_1,i\notin S_2]\\
    ={}&\mathbb E[Y|P_1,P_2,pa(i)\in S_1,i\in S_2]-\mathbb E[Y|P_1,P_2,pa(i)\in S_1,i\notin S_2] \\
    ={}&\mathbb E[U(S^i_2+\{i\})-U(S^i_2)|P_1,P_2,pa(i)\in S^i_1]
  \end{split}
\end{equation*}
Therefore, 
\begin{equation*}
  \begin{split}
  &\mathbb E[X_iY]=\mathbb E[\mathbb E[X_iY|P_1,P_2,X_{pa(i)}]]\\
  =&\sum_{p_1,p_2}\mathbb P[P_1=p_1,P_2=p_2]p_1 \\
  &\mathbb E[U(S^i_2+\{i\})-U(S^i_2)|p_1,p_2,pa(i)\in S^i_1]\\
  &+(1-p_1)\cdot 0\\
  ={}&\mathbb E_{P_1,P_2}P_1 \mathbb E[U(S^i_2+\{i\})-U(S^i_2)|P_1,P_2,pa(i)\in S^i_1]
  \end{split}
\end{equation*}
\paragraph{Patch 2} I think it can still be fixed by dividing $X_i$ by $P_1$, and that gives:
\begin{equation}
  \label{eq:code-v1}  
  X_i=\begin{cases}
    \frac{1}{P_1P_2} & pa(i) \in S_1 \wedge i \in S_2\\
    \frac{-1}{P_1(1-P_2)} & pa(i) \in S_1 \wedge i \notin S_2\\
    0 & \text{otherwise}
  \end{cases}
\end{equation}


Though, it cannot fix the weird conditioning on $pa(i) \in S_1^i$, which means The subsets we are averaging on must always include the $pa(i)$ and hence includes the siblings of $i$ more frequently than other second-level sources.


==> rm/intro-v2.tex <==
\section{ Introduction-v2 (WIP) }
\notejinkun{I feel like pitching our paper as measuring individual contribution is not as good as pitching it as detecting the group, since it seems hard to justify why having a larger value of our quantity means it has a larger contribution?}
\sid{I think we have all the pieces we need for the introduction puzzle, we just need to reorder things. We should start with more overview statements about the kinds of questions people ask and the landscape of work in this area (e.g., some of the statements in "why sparsity is reasonable" are a better fit here.}

% Lots of interest in using machine learning models for driving decisions. However, training a model requires finding large quantities of data, which in itself is challenging in many domains. In some cases this is solved by combining data from multiple competing sources~\cite{Zheng2019HelenMS}. In others from combining data from multiple tenants~\cite{}. Finally, might also be solved by acquiring data by crawling web pages~\cite{}.\fixme{Poison frogs mentioned this.}

\sid{Intro structure: \\
- When people use black-box models, they want to be able to explain the model's decisions (for debugging, for identifying corrupt/poisoned data, etc.). \\
- Whereas traditionally people often ask these questions of individual datapoints, data is often naturally organized into sources (e.g., customer data in a multi-tenant setting). These sources are treated as units of trust, and the questions above can be applied to sources (e.g., has a source been corrupted)? Give example from Microsoft oil customer (make this example similar to running example we use later on). \\
- One advantage of this source view is that you have multiple examples from the same source and hence get more signal about that source, increasing the power of our explanations. \\
- We want to be able to identify the input sources that contribute to a particular model decision. This question has been asked in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are sparse. (Justify sparsity a little more here.) \\
- For example, a strawman approach is to do a LOO test. Suppose one data source is corrupted, then training N different models omiting one source at a time will reveal the corrupt source. \\
- A better approach is to use group testing, which allows you to reduce number of models to $O(\log n)$ using a deterministic tree. \\
- But what if the number of sources contributing to the decision is $>1$. Turns out you can still handle this with the group testing approach using the power of randomization. \\
- Use the above strawmen to motivate AME as a reasonable quantity for us to measure. We would like to develop an approach that measures AME for each source. \\
- Convey the properties we desire in a solution and why they are challenging. The three main challenges are: (1) computational efficiency (resource, time), (2) controllable false positive rate, (3) general across different kinds of models and learning algorithms (especially deep learning ones, for which the question of explainability is most prominent). \\
- Prior approaches somehow don't meet all of the challenges we care about. Mention why influence functions, shapley value, group testing, etc. fall short of meeting these requirements/challenges. Forward reference the related work for more discussion on this. \\
- So we develop a new approach called XX. Summarize our approach and call out the (one or two) key ways in which it differs from prior approaches in relation to the requirements/challenges we listed above. \\
- We apply our approach to three different tasks: poison detection and model explanation, using different datasets. We also extend this to two-level hierarchy of sources. Say something cool about our results (e.g., example of the kind of thing we are able to do.) \\
- Then briefly summarize the rest of the paper and end intro.
}
When using a black-box machine learning (ML) model like deep neural networks (DNN) for driving decisions, one often asked question is why the model gives such a prediction on a query input. People usually want to be able to explain the model's decision for many purposes. For example, today people are increasingly focused on the security of their ML models, and effort has been developed both on poisoning and its detection. One of the detection problem, called data poisoning detection, aims to identify the poisoned data that fooled the model. Another similar application is for debugging: people want to explain unexpected predictions in which there are no attackers but mis-labeled or ambiguous/misleading data. This paper focuses on classification models, and aims to explain the prediction from the perspective of the training data.

Whereas traditionally people often ask these questions of individual datapoints, data is often naturally organized into sources in real world (e.g., customer data in a multi-tenant setting~\cite{}, combining data from multiple competing sources~\cite{Zheng2019HelenMS}, data from crawling multiple web pages~\cite{Shafahi2018PoisonFT}). These sources are treated as units of trust, and the questions above can be applied to sources (e.g., has a source been corrupted by a malicious attacker). \fixme{Give example from Microsoft oil customer (make this example similar to running example we use later on).} Moreover, one advantage of this source view is that you have multiple examples from the same source and hence get more signal about that source, increasing the power of our explanations.

We want to be able to identify the input sources that contribute to a particular model decision. This question has been asked in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are sparse. For the data poisoning detection application mentioned above, the total number of poisoned data sources is typically small given the limited resources of attackers. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. Therefore, we make a \textit{sparsity assumption} that the prediction is mainly affected by a small number of data sources. Note that these sources may either support or oppose the prediction. Denote by $k,k'$ the number of sources that support and oppose, respectively, and the assumption can be written as $k+k'\ll n$.

The problem is defined as to find out the sources that support the prediction, given the dataset, training algorithm, query input and the prediction label (called query label from now on). With \textit{sparsity assumption}, a strawman approach is to do a LOO test. Suppose there are $n$ sources and one data source is corrupted, then training $n$ different models omiting one source at a time will reveal the corrupt source. A better approach is to use group testing, which allows you to reduce number of models to $O(\log n)$ using a deterministic tree. But what if the number of sources contributing to the decision is $>1$. Turns out you can still handle this with the group testing approach using the power of randomization. We use the above strawmen to motivate Average Marginal Effect (\quantity{}) as a reasonable quantity for us to measure, which is an average LOO effect. We would like to develop an approach that measures \quantity{} for each source. We detail \quantity{} and why it is better than classic LOO test in \S\ref{subsec:ame-mov}.

To measure \quantity{}, we first need to design a rule for choosing subset population for \quantity{} and should guarantee that it works for most incoming queries. An important constraint here is that the population need to be decided before the queries incoming, because we want to finish the expensive sampling offline and reuse for every future query, instead of sampling every time for a new query. Moreover, we want to estimate \quantity{} for each source, thus each of the sources requires training many models. Therefore, there are three main challenges: (1) \textit{computational efficiency}, i.e. both resources and time used for models training, (2) \textit{controllable false positive rate}, (3) \textit{general across different kinds of models and learning algorithms} (especially deep learning ones, for which the question of explainability is most prominent). Prior approaches somehow don't meet all of the challenges we care about. \fixme{Mention why influence functions, shapley value, group testing, etc. fall short of meeting these requirements/challenges.} Refer to \S\ref{subsec:rel-work} the related work for more discussion on this.

We develop a new approach called XXX\fixme{naming our approach}. We sample subsets and train multiple models offline and reuse across different queries. When serving a new query, perform inference on query input, retrieve confidence of query label as signal, then employ LASSO to estimate the \quantity{}s, and finally use Knockoffs to control the selection precision. For choosing subset population for \quantity{}, we use a default population that covers roughly uniformly for different sizes of subsets when prior knowledge is not available. In other words, there would be roughly the same number of subsets sampled for each size.\footnote{Note that we differ with Shapley Value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately. However, this approximation enables the use of LASSO \notejinkun{todo: double check}. Second, our framework accepts customized population. It is useful when prior knowledge is available.} 

To estimate efficiently, %we utilize the sparsity assumption and borrow techniques from the literature of causal inference. 
we reuse subsets rather than sampling subsets separately for each source. Next, we train a model on each subset and use the model output as the dependent variable and the subset as the independent variable, and formulate the estimation for $n$ sources together into a single regression problem where each source is estimated by one coefficient. We further utilize LASSO to achieve a scalable sample efficiency: if regularization parameter is chosen correctly, the number of samples and thus training runs needed for a good estimation is $O((k+k')\log n)$ that scales as $n$ increases.
Specifically, each source has one independent variable indicating its inclusion/exclusion in the subset and the output of the model trained on the subset is used as the dependent variable. The coefficients for the sources estimate their \quantity{} consistently (modulo a constant factor), meaning that the coefficients converge asymptotically to the true values of their \quantity{}. 

After the estimation, the sources having an estimate larger than a threshold are selected, and the threshold is chosen by a technique called \textit{Knockoffs}, which has the merit of controlling the expected precision to be at least a given value. \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
% In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.

Moreover, for offline models training, We also propose to speed up by approximating training-from-scratch with warm-starting, which serves as our main technique for amortizing the training cost of all these models. The overall workflow is shown in Fig. \ref{fig:workflow}. 

We mainly apply our approach to two different tasks: poison detection and model explanation, using multiple different datasets. We also extend this to two-tier hierarchy of sources. \fixme{Results} Say something cool about our results (e.g., example of the kind of thing we are able to do.)




\paragraph{OLD VERSION}
When using a black-box machine learning (ML) model like deep neural networks (DNN) for driving decisions, one often asked question is why the model gives such a prediction on a query input. This paper focuses on classification models, and aims to explain the prediction from the perspective of the training data. We are interested in the scenarios where data can be divided into $n$ sources. Such scenarios can well occur in real world, since training a model requires finding large quantities of data, which in itself is challenging in many domains. In some cases this is solved by combining data from multiple competing sources~\cite{Zheng2019HelenMS}. In others from combining data from multiple tenants~\cite{}. Finally, might also be solved by acquiring data by crawling web pages~\cite{Shafahi2018PoisonFT}. 

Our problem is defined as to find out the sources that support the prediction, given the dataset, training algorithm, query input and the prediction label (called query label from now on). We assume that models are updated much less frequently than queries arrive. We further make a \textit{sparsity assumption} that the prediction is mainly affected by a small number of data sources. Note that these sources may either support or oppose the prediction. Denote by $k,k'$ the number of sources that support and oppose, respectively, and the assumption can be written as $k+k'\ll n$.

%We further assume that every source can be further divided into three groups: the proponent group that supports the prediction, the opponent group that opposes the prediction and the neutral group that neither proposes or opposes. \sid{Why isn't it possible for a source to be neutral, i.e. neither a proponent nor an opponent?} \notejinkun{Sorry forgot to change the text here. Fixed now. (I wrote in \S2 but forgot to update here)} The problem is defined as to identify the proponent group, given the dataset, query input and the prediction label (called query label from now on). Denote by $k$ the size of the proponent group and $k'$ he size of the opponent group. \notepanda{I agree with Jinkun's concern, I think we should lay it out as we are seeing use cases where data is collected from multiple sources, etc. and pose the question in term of sources.}\notejinkun{Ah I actually meant to say our quantity is only interpretable on its sign but not its magnitude. So we only want to formulate as detecting the group of sources instead of measuring/quantifying the contribution of every sources. Sorry for the ambiguity.}

\paragraph{Why the sparsity assumption is \sout{interesting} reasonable.}\notepanda{Interesting or reasonable? The paragraph seems to focus on reasonable?}\notejinkun{Yeah I meant reasonable (what's the difference between the two?)} Though assuming sparsity, the problem is still meaningful in reality. For example, today people are increasingly focused on the security of their ML models, and effort has been developed both on poisoning and its detection. One of the detection problem, called data poisoning detection, aims to identify the poisoned data points that fooled the model. This problem is essentially the same as ours, and the sparsity assumption also holds\notepanda{I don't follow the line of reasoning here, it holds because we assume it sounds less like it holds and more like we just assumed?}: the total number of poisoned data points is typically small given the limited resources of attackers. The other similar application is to explain unexpected predictions in which there are no attackers. The mis-predictions are likely caused by mis-labeled or ambiguous/misleading data, which should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \sid{I'm not sure what this last sentence is trying to say (we can omit it, since the point is well made that tail data in test sets are influenced by a very sparse number of input sources.} \notejinkun{To Sid: My concern is that long-tailed part are only a small fraction of the full dataset and people may challenge that most queries are not in this region thus not sparse}

% \paragraph{Defining proponent/opponent group? \notejinkun{come from \url{https://arxiv.org/pdf/2002.08484.pdf}}}  \notejinkun{Should we give formal definition of these two groups? I feel like it's hard to define them clearly. Or maybe we should even remove this paragraph? If we want to keep it, I feel like this should not be in the introduction since intro should not give too much details (and that in later sections probably we have to repeat this paragraph)? But the argument for the \quantity{} needs this. So any suggestion?}\notepanda{I would argue for not defining it here, rather saying a perfect method is one that can detect any source that impacts the decision, this is hard to do in practice so we don't get there, and then use sensitivity as a figure of merit to evaluate?} \sid{Defining this precisely will be tricky, but it raises a good point: we know the source of poisoning because we poison the input data, but that in itself is not a general way of measuring the proponent-ness of a source. It could be that we don't detect a (poisoned) source because other artifacts in the data are sufficient to explain the decision. I think the large leave-out effect is a good starting point to build on.}
% The exact definition is non-trivial (even controversial) and thus left for future work. Instead, we focus on some necessary properties of the group that we argue people generally would agree upon. We only consider proponent group here since the opponent group is similar. (1) \textbf{It must have a large leave-out effect}, i.e. removing this group decreases significantly the signal, where the signal can be defiend as the probability/confidence of predicting the query label or other quantity that captures such tendency \footnote{Classification DNNs typically have such quantities since the training is usually done by maximizing likelihood that by construction requires a measure of probability. When there is not, }. However, this alone is too imprecise since it does not rule out groups containing extra data points that have no effect, e.g. the full dataset as well has a large leave-out effect. This leads to the second property: (2) \textbf{The data point in the group should have non-zero individual effect.} More precisely, consider removing (without replacement) the data points of the group one by one at some order. We know that the outcome changes substantially when all of the group are removed, so there must be a time when removing one changes at least some. If a data point always has little effect upon removal in any ordering, it should not be in the group. \sid{I don't quite get this: why can't a source have one or more datapoints that don't affect the decision at all? It still could be a relevant source.}

% % (3) The group should be as large as possible when the two previous conditions are verified, so that it is powerful enough to include every proponent data point.
% % When using a black-box machine learning (ML) model like deep neural networks (DNN), one often asked question is why the model gives such a prediction on a query input. This paper focuses on classification models, and aims to explain the prediction from the perspective of the training data. The problem is defined as to identify the training data points that caused this prediction. More precisely, given a training set, a query input and its prediction label (call it \textit{query label} from now on), we want to find smallest groups such that removing the group changes the model outcome substantially into no longer predicting the query label with high probability/confidence\footnote{ML classifiers usually have such a quantity for each class.}, and any data point in any of such groups are said to cause the prediction. Denote by $k$ this group size. Similarly, we define groups and data points that prevent the prediction. Denote such group size by $k'$. Further denote the training set size by $n$. This paper limits the scope to the cases where the group size is small, i.e. $k \ll n$. We term the latter \textit{Sparsity Assumption}. Note that $k$ is not known in advance.

% \notepanda{I am a bit concerned about why the preceding text leads to this discussion of AME? There seems to be a story or connection missing.}

\paragraph{Average Marginal Effect (\quantity{})}
One obvious approach is performing LOO test and select sources having a large LOO effect, but as \S\ref{subsec:ame-mov} shows this is not enough (the effect may be zero for every source), due to the non-linearity and complication of training algorithms and ML models. Therefore, we propose to perform the LOO tests on multiple subsets subsampled from the full dataset and select those sources having a large average LOO effect. The average LOO effect is termed Average Marginal Effect (\quantity{}) \notejinkun{I'm bad at naming. If anyone has better options...} \fixme{cite the paper originally proposing AME}. We detail why \quantity{} is better than classic LOO test in \S\ref{subsec:ame-mov}.%, but a quick explanation is that 

% For any $k_i$, by the second property there is a subset of the proponent group such that removing $k_i$ has a dampening effect. Notice that this is exactly doing LOO test since we are removing one point, but it is different than usual LOO test in that instead of the whole dataset, the removal is on a dataset that includes the group subset and all the other non-proponent data. We want to have non-zero effect measured for each $k_i$, thus we want to create a population of such datasets. However, the group is unknown, so we have to subsample the whole dataset, and that has a side effect that the non-proponent data are also subsampled. We make an assumption that they are sufficiently large enough that doing a (not-too-aggresive) subsampling does not very much affect their distribution, so that removing $k_i$ still has same effect as when the non-proponents are not subsampled. It follows that removing $k_i$ unlikely strengthens the signal in any case. Therefore, the LOO effects in the population are either dampening or zero, and when we average them, it is not 0 anymore, but a dampening effect. Call this average LOO effect \textit{Average Marginal Effect (\quantity{})}. For opponents, the \quantity{} should likely be the opposite, and for other data points, the \quantity{} should likely be zero.

\paragraph{Challenges}\notepanda{I would propose using a much shorter thing just providing a high-level approach (say how would you do this, one obvious answer is LOO but as we discuss in \S\ref{} that is not enough. So our approach is to train models over subsets and use information from that. But to do this need to address two challenges\ldots).}
There are two challenges remaining. First, we need to design a rule for choosing subset population for \quantity{} and should guarantee that it works for most incoming queries. An important constraint is that we have to decide the population before seeing the queries, because we want to finish the expensive sampling offline and reuse for every future query, instead of sampling every time for a new query. \notejinkun{I am a bit concerned about this point. People may ask why don't you choose adaptively using the validation set (assuming queries are similar to it), and I'm not sure how to respond that properly. My only response is that it does not work for the application of poison detection. } \notejinkun{The other concern is our experiments. We have plots showing the best P is different across datasets. But actually here what we need is across queries, and I checked our experiments, which unfortunately shows similar pattern across queries.} %The subset sampling distribution should ensure good coverage: An effective subset should let the contributive sources manifest the most of their effects, i.e. having high LOO delta, but different learning tasks / poisoning attacks may exhibit very different characteristics of such subsets. One distribution of subsets that works for one type of task may totally fail for the other.
%, but too small a subset dataset could deviate too far away from the full dataset, making the relative effect on the subset deviate as well from the that on the full dataset. E.g., consider a subset containing no datasets, then the model will only be trained on 1 or 0 data point, which will always produce the label in the former case and random in the latter case. In this case, the quantity degrades to only looking at the labels--it would assign equal contribution to every point sharing the same label as the query prediction. On the other hand, too large a subset dataset may as well unable to capture the contribution, as discussed above. 
Second, estimating \quantity{} is costly: Each source needs to be estimated, each of which requires training many models. Although techniques like influence functions \cite{koh_understanding_2017} can approximate outcomes without model training, it is \sout{not accurate} fragile for DNNs \cite{basu_influence_2020}. \sid{We might want to qualify or soften the preceding sentence, perhaps pointing out that it is fragile rather than "not accurate".}
% Third, after the estimation one still needs to have a selection procedure to decide which sources to select. the sources based on \quantity{}, one needs to decide a threshol

\paragraph{Approach} \sid{Just a note that we should make it crystal clear that we are training multiple models, and compare that to prior approaches.} To address the first challenge, we use a default population that covers roughly uniformly for different sizes of subsets when prior knowledge is not available. In other words, there would be roughly the same number of subsets sampled for each size.\footnote{Note that we differ with Shapley Value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately. However, this approximation enables the use of LASSO \notejinkun{todo: double check}. Second, our framework accepts customized population. It is useful when prior knowledge is available.} To address the second challenge, we utilize the sparsity assumption and borrow techniques from the literature of causal inference. Instead of sampling subsets and computing separately for each source, we reuse subsets and use regression to measure for all sources simultaneously, where each source has one covariate indicating its inclusion/exclusion in the subset and the signal of the model trained on the subset is used as the response variable. The coefficients for the sources estimate their \quantity{} consistently, meaning that the coefficients converge asymptotically to the true values of their \quantity{}. The coefficients larger than a threshold are selected, and the threshold is chosen by a technique called \textit{Knockoffs}, which has the merits of controlling the expected precision to be at least a given value. \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.
Next, the subsets and sub-models are reused across different queries -- only the response variables are needed to be re-computed, which only requires inference. Finally, we speed up the training by approximating training-from-scratch with warm-starting. \sid{Though we aren't really innovating here, we should highlight this as our main technique for amortizing the training cost of all these models.}

\paragraph{Approach-v2} \sid{Just a note that we should make it crystal clear that we are training multiple models, and compare that to prior approaches.} To address the first challenge, we use a default population that covers roughly uniformly for different sizes of subsets when prior knowledge is not available. In other words, there would be roughly the same number of subsets sampled for each size.\footnote{Note that we differ with Shapley Value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately. However, this approximation enables the use of LASSO \notejinkun{todo: double check}. Second, our framework accepts customized population. It is useful when prior knowledge is available.} 

To estimate efficiently, %we utilize the sparsity assumption and borrow techniques from the literature of causal inference. 
we reuse subsets rather than sampling subsets separately for each source. Next, we train a model on each subset and use the model output as the dependent variable and the subset as the independent variable, and formulate the estimation for $n$ sources together into a single regression problem where each source is estimated by one coefficient. We further utilize LASSO to achieve a scalable sample efficiency: if regularization parameter is chosen correctly, the number of samples and thus training runs needed for a good estimation is $O((k+k')\log n)$ that scales as $n$ increases.
Specifically, each source has one independent variable indicating its inclusion/exclusion in the subset and the output of the model trained on the subset is used as the dependent variable. The coefficients for the sources estimate their \quantity{} consistently (modulo a constant factor), meaning that the coefficients converge asymptotically to the true values of their \quantity{}. 

After the estimation, the sources having an estimate larger than a threshold are selected, and the threshold is chosen by a technique called \textit{Knockoffs}, which has the merit of controlling the expected precision to be at least a given value. \fixme{TODO: may need to soften if we are not able to prove the one-sided knockoffs} \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
% In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.

Finally, to further reduce the overhead of model training, we do the subset sampling and model training offline and reuse across different queries. To serve a new query, only the inference of these models are performed. This allows us to amortize the cost of training. We also propose to speed up the training by approximating training-from-scratch with warm-starting. The overall workflow is shown in Fig. \ref{fig:workflow}. \sid{Though we aren't really innovating here, we should highlight this as our main technique for amortizing the training cost of all these models.}



% \paragraph{Generalizing to Sources} We further generalize our problem statement to scenarios where the data come from different sources and we want to identify the group of sources that support/cause the prediction. This also has real applications. For example, in poison detection under multi-party training where multiple parties provide their own data to cooperate in training a model but some parties may be malicious and cause a mis-prediction of the model, one may want to ask which parties are responsible for this mis-prediction.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/workflow.pdf}
    \caption{Workflow}
    \label{fig:workflow}
\end{figure}
\paragraph{results} todo.

\paragraph{Contribution}
\begin{outline}
\1 We propose \quantity{} whose sign indicates whether a data point/source supports or opposes the prediction.
\1 We propose a default option as the population, but also allows customized ones.
\1 We employ LASSO to estimate this quantity, and show that only $O(k\log n)$ \notejinkun{again $k$ should include the other group} samples are required to achieve a good estimation.
\1 We use Knockoffs to control the selection precision.
\1 We optimize the model training using warm-starting.
\end{outline}


==> rm/intro-v3.tex <==
\section{ Introduction-v3 (WIP) }
\sid{I think we have all the pieces we need for the introduction puzzle, we just need to reorder things. We should start with more overview statements about the kinds of questions people ask and the landscape of work in this area (e.g., some of the statements in "why sparsity is reasonable" are a better fit here.}

% Lots of interest in using machine learning models for driving decisions. However, training a model requires finding large quantities of data, which in itself is challenging in many domains. In some cases this is solved by combining data from multiple competing sources~\cite{Zheng2019HelenMS}. In others from combining data from multiple tenants~\cite{}. Finally, might also be solved by acquiring data by crawling web pages~\cite{}.\fixme{Poison frogs mentioned this.}

\sid{Intro structure: \\
- When people use black-box models, they want to be able to explain the model's decisions (for debugging, for identifying corrupt/poisoned data, etc.). \\
- Whereas traditionally people often ask these questions of individual datapoints, data is often naturally organized into sources (e.g., customer data in a multi-tenant setting). These sources are treated as units of trust, and the questions above can be applied to sources (e.g., has a source been corrupted)? Give example from Microsoft oil customer (make this example similar to running example we use later on). \\
- One advantage of this source view is that you have multiple examples from the same source and hence get more signal about that source, increasing the power of our explanations. \\
- We want to be able to identify the input sources that contribute to a particular model decision. This question has been asked in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are sparse. (Justify sparsity a little more here.) \\
- For example, a strawman approach is to do a LOO test. Suppose one data source is corrupted, then training N different models omiting one source at a time will reveal the corrupt source. \\
- A better approach is to use group testing, which allows you to reduce number of models to $O(\log n)$ using a deterministic tree. \\
- But what if the number of sources contributing to the decision is $>1$. Turns out you can still handle this with the group testing approach using the power of randomization. \\
- Use the above strawmen to motivate AME as a reasonable quantity for us to measure. We would like to develop an approach that measures AME for each source. \\
- Convey the properties we desire in a solution and why they are challenging. The three main challenges are: (1) computational efficiency (resource, time), (2) controllable false positive rate, (3) general across different kinds of models and learning algorithms (especially deep learning ones, for which the question of explainability is most prominent). \\
- Prior approaches somehow don't meet all of the challenges we care about. Mention why influence functions, shapley value, group testing, etc. fall short of meeting these requirements/challenges. Forward reference the related work for more discussion on this. \\
- So we develop a new approach called XX. Summarize our approach and call out the (one or two) key ways in which it differs from prior approaches in relation to the requirements/challenges we listed above. \\
- We apply our approach to three different tasks: poison detection and model explanation, using different datasets. We also extend this to two-level hierarchy of sources. Say something cool about our results (e.g., example of the kind of thing we are able to do.) \\
- Then briefly summarize the rest of the paper and end intro.
}\\
\\
When using a black-box machine learning (ML) model like deep neural networks (DNN) for driving decisions, one often asked question is why the model gives such a prediction on a query input. People usually want to be able to explain the model's decision for many purposes. For example, today people are increasingly focused on the security of their ML models, and effort has been developed both on poisoning and its detection. One of the detection problem, called data poisoning detection, aims to identify the poisoned data that fooled the model. Another similar application is for debugging: people want to explain unexpected predictions in which there are no attackers but mis-labeled or ambiguous/misleading data. This paper focuses on classification models, and aims to explain the prediction from the perspective of the training data. \notejinkun{mild comment: may be better to move the last sentence up and merge with the first sentence? Since the examples are all explaining from data.}

Whereas traditionally people often ask these questions of individual datapoints, data is often naturally organized into sources in real world (e.g., customer data in a multi-tenant setting~\cite{}, combining data from multiple competing sources~\cite{Zheng2019HelenMS}, data from crawling multiple web pages~\cite{Shafahi2018PoisonFT}). These sources are treated as units of trust, and the questions above can be applied to sources (e.g., has a source been corrupted by a malicious attacker). \fixme{todo: Give example from Microsoft oil customer (make this example similar to running example we use later on).} Moreover, one advantage of this source view is that you have multiple examples from the same source and hence get more signal about that source, increasing the power of our explanations. \notejinkun{Is the last sentence saying that source view makes the problem easier (then why do we specifically bring up an easier version of a traditional problem)? I feel like we need to say this new view brings challenges to old techniques because every proponent data may have only little contribution and hard to detect, so we need to consider each source as a whole in order to gain enough signal to detect them. Unfortunately, previous techniques cannot always generalize easily, \eg (i) influence function \cite{koh_understanding_2017} was traditionally for individual data point, and careful reasoning is needed as in \cite{koh_accuracy_2019} to generalize to the source view. (ii) \cite{pruthi_estimating_2020} attributes the loss delta after every iteration to the data points inside that batch. (iii) \cite{chen2018detecting} is based on examining the second-to-last layer's activation of every data point, but it is unclear how to extract similar activation for a whole source.}

We want to be able to identify the input sources that contribute to a particular model decision. This question has been asked in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are \emph{sparse}. For the data poisoning detection application mentioned above, the total number of poisoned data sources is typically small given the limited resources of attackers. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \notejinkun{I remember the previous sentence does not make sense for Sid. Maybe need to rewrite or remove.} Therefore, we make a \textit{sparsity assumption} that the prediction is mainly affected by a small group of data sources. Note that these sources may either support or oppose the prediction.\notejinkun{I remember there was a compliant about why it couldn't be neutral. But here I mean only in the group mainly affecting the prediction, and neutrals should not have main influence, so it couldn't be neutral.} Denote by $k$ the number of sources in this group, and the assumption can be written as $k\ll n$.

\notejinkun{I would state the problem in the previous paragraph} The problem is defined as to find out the sources that support the prediction, given the dataset, training algorithm, query input and the prediction label (called query label from now on). With \textit{sparsity assumption}, a strawman approach is to do a LOO test. Suppose there are $n$ sources and one data source is corrupted, then training $n$ different models omiting one source at a time will reveal the corrupt source. A better approach is to use group testing, which allows you to reduce number of models to $O(\log n)$ using a deterministic tree. But what if the number of sources contributing to the decision is $>1$. Turns out you can still handle this with the group testing approach using the power of randomization. \notejinkun{My concern is that our approach smells very differently from those of group testing (which is very theoretical and formal as those of ML theories), and it might be weird to say we are group testing?} We use the above strawmen to motivate Average Marginal Effect (\quantity{}) as a reasonable quantity for us to measure, which is an average LOO effect. We would like to develop an approach that measures \quantity{} for each source. We detail \quantity{} and why it is better than classic LOO test in \S\ref{subsec:ame-mov}.

To measure \quantity{}, we first need to design a rule for choosing subset population for \quantity{} and should guarantee that it works for most incoming queries. An important constraint here is that the population need to be decided before the queries incoming, because we want to finish the expensive sampling offline and reuse for every future query, instead of sampling every time for a new query. \notejinkun{To Anqi: The previous text is the design goal of AME and probably should be placed in later section that describe AME. (Previously I stated it as a challenge so it appears here, but now I think we don't need it.)} Moreover, we want to estimate \quantity{} for each source, thus each of the sources requires training many models.\notejinkun{Maybe merged into the subsequent challenge (1)?} Therefore, there are three main challenges: (1) \textit{computational efficiency}, i.e. both resources and time used for models training, (2) \textit{controllable false positive rate}, \notejinkun{technically should be called false discovery rate. They seem to be different concept.} (3) \textit{general across different kinds of models and learning algorithms} (especially deep learning ones, for which the question of explainability is most prominent). Prior approaches somehow don't meet all of the challenges we care about. For instance, approaches \cite{jia_towards_2020,ghorbani_data_nodate} that quantify using Shapley Value (SV) are either too costly or making strong assumption about the models. Although techniques like influence functions \cite{koh_understanding_2017} can approximate outcomes without model training, it is fragile for DNNs \cite{basu_influence_2020}.  \noteanqi{Is the summary here appropriate? Maybe we don't beat group testing here.} Refer to \S\ref{subsec:rel-work} the related work for more discussion on this.

We develop a new approach called XXX \fixme{naming our approach}. We sample subsets and train multiple models offline and reuse across different queries. When serving a new query, perform inference on query input, retrieve confidence of query label as signal, then employ LASSO to estimate the \quantity{}s, and finally use Knockoffs to control the selection precision. For choosing subset population for \quantity{}, we use a default population that covers roughly uniformly for different sizes of subsets when prior knowledge is not available. \notejinkun{Maybe we omit this part in the intro.} In other words, there would be roughly the same number of subsets sampled for each size.\footnote{Note that we differ with Shapley Value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately. However, this approximation enables the use of LASSO \notejinkun{todo: double check}. Second, our framework accepts customized population. It is useful when prior knowledge is available.} 

\notejinkun{Guess we need to revise this paragraph a bit, given that Anqi added the previous paragraph describing the overall workflow (which is nice). Probably just summarize every subsection of \S\ref{sec: procedure}. I'll do this shortly} To estimate efficiently, %we utilize the sparsity assumption and borrow techniques from the literature of causal inference. 
we reuse subsets rather than sampling subsets separately for each source. Next, we train a model on each subset and use the model output as the dependent variable and the subset as the independent variable, and formulate the estimation for $n$ sources together into a single regression problem where each source is estimated by one coefficient. We further utilize LASSO to achieve a scalable sample efficiency: if regularization parameter is chosen correctly, the number of samples and thus training runs needed for a good estimation is $O(k\log n)$ that scales as $n$ increases.
Specifically, each source has one independent variable indicating its inclusion/exclusion in the subset and the output of the model trained on the subset is used as the dependent variable. The coefficients for the sources estimate their \quantity{} consistently (modulo a constant factor), meaning that the coefficients converge asymptotically to the true values of their \quantity{}. 

After the estimation, the sources having an estimate larger than a threshold are selected, and the threshold is chosen by a technique called \textit{Knockoffs}, which has the merit of controlling the expected precision to be at least a given value. \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
% In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.

Moreover, for offline models training, We also propose to speed up by approximating training-from-scratch with warm-starting, which serves as our main technique for amortizing the training cost of all these models. The overall workflow is shown in Fig. \ref{fig:workflow}. 

\notejinkun{v2 of previous 3 paragraphs}
We develop a new approach called XXX \fixme{naming our approach}. There are four phases, with the first two being offline and last two being online: (i) \emph{sampling:} Sample subsets according to a carefully chosen distribution; (ii) \emph{training:} Train one model per subset offline, which will later be reused across different queries; (iii) \emph{estimation:} When serving a new query, perform inference on each model for the query input, retrieve confidence of query label as signal, then employ LASSO to estimate the \quantity{}s; (iv) \emph{selection:} And finally based on the estimates, use Knockoffs for selecting sources to control the FDR. The overall workflow is shown in Fig. \ref{fig:workflow}. 

For the sampling phase, we use a default distribution that covers roughly uniformly for different sizes of subsets when prior knowledge is not available. In other words, there would be roughly the same number of subsets sampled for each size.\footnote{Note that we differ with Shapley Value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately. However, this approximation enables the use of LASSO \notejinkun{todo: double check}. Second, our framework accepts customized population. It is useful when prior knowledge is available.} 

For the training phase, we propose to speed up by approximating training-from-scratch with warm-starting.%, which serves as our main technique for amortizing the training cost of all these models. 

For the estimation phase, we encode each subset as the dependent variable and its signal as the independent variable, and formulate the estimation for $n$ sources together into a single regression problem where each source is estimated by one coefficient. We further utilize LASSO to achieve a scalable sample efficiency: if regularization parameter is chosen correctly, the number of samples and thus training runs needed for a good estimation is $O(k\log n)$ that scales as $n$ increases.% The coefficients for the sources estimate their \quantity{} consistently (modulo a constant factor), meaning that the coefficients converge asymptotically to the true values of their \quantity{}. 

For the selection phase, the sources having an estimate larger than a threshold are selected, and the threshold is chosen by a technique called \textit{Knockoffs}, which has the merit of controlling the expected FDR to be at most a given level. \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
% In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.



% \paragraph{Generalizing to Sources} We further generalize our problem statement to scenarios where the data come from different sources and we want to identify the group of sources that support/cause the prediction. This also has real applications. For example, in poison detection under multi-party training where multiple parties provide their own data to cooperate in training a model but some parties may be malicious and cause a mis-prediction of the model, one may want to ask which parties are responsible for this mis-prediction.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/workflow.pdf}
    \caption{Workflow}
    \label{fig:workflow}
\end{figure}
%\paragraph{results} todo.
We mainly apply our approach to two different tasks: poison detection and model explanation, using multiple different datasets. We also extend this to two-tier hierarchy of sources. \fixme{todo: Results} Say something cool about our results (e.g., example of the kind of thing we are able to do.)

\paragraph{Contribution}
\begin{outline}
\1 We propose \quantity{} whose sign indicates whether a data point/source supports or opposes the prediction.
\1 We propose a default option as the population, but also allows customized ones.
\1 We employ LASSO to estimate this quantity, and show that only $O(k\log n)$ samples are required to achieve a good estimation.
\1 We use Knockoffs to control the selection FDR.
\1 We optimize the model training using warm-starting.
\end{outline}

We will define our problem in \S\ref{subsec:pro-state}. \S\ref{subsec:ame} details how we measure the \quantity{} quantity in our approach, and \S\ref{sec: procedure} shows the sampling, training, estimation and selection procedure. We deliver more about an extension design - Hierarchical Design in \S\ref{subsec:hier}. Then \S\ref{subsec:implement} and \S\ref{subsec:evaluation} shows the implementation details and evaluation of our approach on the poison detection task. \S\ref{subsec:other-apply} gives the application details and results about model explanation task as well as hierarchical assignment. More discussion on related work is in \S\ref{subsec:rel-work} and \S\ref{subsec:limitation} mentions the limitations of our work. Finally, we conclude the paper.

==> rm/intro-v4.tex <==
\section{ Introduction-v4 (WIP) }
\sid{I think we have all the pieces we need for the introduction puzzle, we just need to reorder things. We should start with more overview statements about the kinds of questions people ask and the landscape of work in this area (e.g., some of the statements in "why sparsity is reasonable" are a better fit here.}

% Lots of interest in using machine learning models for driving decisions. However, training a model requires finding large quantities of data, which in itself is challenging in many domains. In some cases this is solved by combining data from multiple competing sources~\cite{Zheng2019HelenMS}. In others from combining data from multiple tenants~\cite{}. Finally, might also be solved by acquiring data by crawling web pages~\cite{}.\fixme{Poison frogs mentioned this.}

\sid{Intro structure: \\
- When people use black-box models, they want to be able to explain the model's decisions (for debugging, for identifying corrupt/poisoned data, etc.). \\
- Whereas traditionally people often ask these questions of individual datapoints, data is often naturally organized into sources (e.g., customer data in a multi-tenant setting). These sources are treated as units of trust, and the questions above can be applied to sources (e.g., has a source been corrupted)? Give example from Microsoft oil customer (make this example similar to running example we use later on). \\
- One advantage of this source view is that you have multiple examples from the same source and hence get more signal about that source, increasing the power of our explanations. \\
- We want to be able to identify the input sources that contribute to a particular model decision. This question has been asked in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are sparse. (Justify sparsity a little more here.) \\
- For example, a strawman approach is to do a LOO test. Suppose one data source is corrupted, then training N different models omiting one source at a time will reveal the corrupt source. \\
- A better approach is to use group testing, which allows you to reduce number of models to $O(\log n)$ using a deterministic tree. \\
- But what if the number of sources contributing to the decision is $>1$. Turns out you can still handle this with the group testing approach using the power of randomization. \\
- Use the above strawmen to motivate AME as a reasonable quantity for us to measure. We would like to develop an approach that measures AME for each source. \\
- Convey the properties we desire in a solution and why they are challenging. The three main challenges are: (1) computational efficiency (resource, time), (2) controllable false positive rate, (3) general across different kinds of models and learning algorithms (especially deep learning ones, for which the question of explainability is most prominent). \\
- Prior approaches somehow don't meet all of the challenges we care about. Mention why influence functions, shapley value, group testing, etc. fall short of meeting these requirements/challenges. Forward reference the related work for more discussion on this. \\
- So we develop a new approach called XX. Summarize our approach and call out the (one or two) key ways in which it differs from prior approaches in relation to the requirements/challenges we listed above. \\
- We apply our approach to three different tasks: poison detection and model explanation, using different datasets. We also extend this to two-level hierarchy of sources. Say something cool about our results (e.g., example of the kind of thing we are able to do.) \\
- Then briefly summarize the rest of the paper and end intro.
}\\
\\
When using a black-box machine learning (ML) model like deep neural networks (DNN) for driving decisions, it would be useful to be able to attribute the model's decision back to training data. For example, one may wish to apportion credit between different crowdworkers who collected the dataset \cite{koh_accuracy_2019}; conduct data cleansing that fixes mislabeled/corrupted data \cite{koh_understanding_2017}; or identify attackers or poisoned data that caused an erroneous prediction in a malicious setup \cite{Shafahi2018PoisonFT,Zheng2019HelenMS}. This paper focuses on classification models. \notejinkun{we need to state we only consier classification models, but where to insert?}%, and aims to explain the model prediction from the perspective of the training data, \ie what part of the data caused this prediction? 
\noteanqi{Last sentence is weird. Maybe: This paper focuses on  classification  models and  aims  to  explain  the  prediction from   the   perspective   of   the   training   data.}

Whereas traditionally people often ask these questions of individual data points, data is often naturally organized into sources in real world (e.g., customer data in a multi-tenant setting~\fixme{fix citation}\cite{}, data formed  by combining multiple competing sources~\cite{Zheng2019HelenMS}, data from crawling multiple web pages~\cite{Shafahi2018PoisonFT}). These sources are treated as units of trust, and the questions above can be applied to sources (e.g., has a source been corrupted by a malicious attacker). \fixme{todo: Give example from Microsoft oil customer (make this example similar to running example we use later on).} Moreover, one advantage of this source view is that you have multiple examples from the same source and hence get more signal about that source, increasing the power of our explanations. \notejinkun{Is the last sentence saying that source view makes the problem easier (then why do we specifically bring up an easier version of a traditional problem)? Or is it saying doing so has more practical significance?} \notejinkun{I feel like we need to state this new view is challenge, as following: However, previous techniques cannot always easily generalize to sources. For instance, influence functions \cite{koh_understanding_2017} use first-order approximation that requires the data to remove is small, which does not apply to large sources. Its followup work \cite{koh_accuracy_2019} though generalizes it to source view and gives a first step analysis, it is not yet clear if influence functions are still accurate. Moreover, influence is fragile for DNNs \cite{basu_influence_2020}. (ii) \cite{pruthi_estimating_2020} attributes the loss delta after every training iteration to the data points inside that batch, but it is unclear how to generalize to sources. (iii) \cite{chen2018detecting} is based on examining the second-to-last layer's activation of every data point, but it is unclear how to extract similar activation for a whole source. On the other hand, trivially ignoring the sources and identifying the data points first and then selecting sources may fail because individual data point could be hard to detect.)}%the prediction may be caused by multiple data points each of which has too little influence to detect. Luckily, the data contributed tends to concentrate in a few sources, and examining the whole would aggregate enough influence to detect. Unfortunately, previous techniques cannot always generalize easily, \eg (i) influence function \cite{koh_understanding_2017} was traditionally for individual data point, and careful reasoning is needed as in \cite{koh_accuracy_2019} to generalize to the source view. However, influence is fragile for DNNs \cite{basu_influence_2020}. (ii) \cite{pruthi_estimating_2020} attributes the loss delta after every iteration to the data points inside that batch, but it . (iii) \cite{chen2018detecting} is based on examining the second-to-last layer's activation of every data point, but it is unclear how to extract similar activation for a whole source.} 
\noteanqi{Maybe we should find another benefit of source senario, but I don't think it's good to compare with other approaches at this very beginning position.} 
Finally, our source view also covers the previous invidiual point view, if one treats every individual data point as a source.

Our problem is defined as to find out the sources that support a particular model prediction, given the dataset, training algorithm, query input and the prediction label (called query label from now on). \sout{We want to be able to identify the input sources that contribute to a particular model decision.} This question has been asked in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are \emph{sparse}. Indeed, it is reasonable to assume sparse contribution. For instance, in the case of data poisoning detection, the attacker is typically only able to poison a limited number of sources given their limited resources at hand. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \notejinkun{I remember the previous sentence does not make sense for Sid. Maybe need to rewrite or remove.} Therefore, we make a \textit{sparsity assumption} that the prediction is mainly affected by a small group of data sources. Note that these sources may either support or oppose the prediction.\notejinkun{I remember there was a compliant about why it couldn't be neutral. But here I mean only in the group mainly affecting the prediction, and neutrals should not have main influence, so it couldn't be neutral.} Denote by $k$ the number of sources in this group, and the assumption can be written as $k\ll n$. We also make a \emph{monotonicity assumption} that in a high level says adding a corrupted source makes the prediction more or at least equally corrupted (see \ref{subsec:pro-state} for detail).

\notejinkun{Would replace with the next paragraph} A strawman approach is to do a leave-one-out (LOO) test. Suppose that one data source is corrupted, then training $n$ different models omiting one source at a time will reveal the corrupt source. A better approach is to use group testing, which allows you to reduce number of models to $O(\log n)$ using a deterministic tree. But what if the number of sources contributing to the decision is $>1$ \notejinkun{I believe group testing can handle this as well}. Turns out we can still handle this with the group testing approach using the power of randomization. \notejinkun{My concern is that our approach smells very differently from those of group testing (which is very theoretical and formal as those of ML theories), and it might be weird to say we are group testing?} \sout{We use the above strawman to motivate Average Marginal Effect (\quantity{}) as a reasonable quantity for us to measure, which is an average LOO effect.} To do so, we propose Average Marginal Effect (\quantity{}) that characterizes the inclination of a source to the prediction, where a large positive number indicates supportive-ness and negative indicates opposed-ness \notejinkun{what are the appropriate words here?}, and then use randomization to achieve efficient estimation. We detail the definition in \S\ref{subsec:ame-mov}. \sout{We would like to develop an approach that measures \quantity{} for each source.} 

\notejinkun{I would write the previous paragraph this way:} A strawman approach is to do a leave-one-out (LOO) test. Suppose that one data source is corrupted and caused a corrupted prediction being queried, then training $n$ different models omiting one source at a time will reveal the corrupt source. But when there are multiple corrupted sources, omiting one out may not be enough -- but only omiting multiple -- to be able to change the model, due to the non-linearity and complication of training algorithms and ML models (\eg the 1-Nearest-Neighbor models; see \S\ref{subsec:ame-mov} for detail). In other words, a zero LOO effect would be observed for every corrupted source. \notejinkun{should we mention the other strawman approach that trains on every source individually?}
Luckily, we observe that when omiting from a subset instead of the full dataset, the LOO effect is more likely to be non-zero. More importantly, it is consistently one-sided and rarely flips, \ie omiting a corrupted source almost always makes the model less or equally corrupted. This motivates us to compute the average LOO effects on multiple subsets. \fixme{how to frame AME:} \textcolor{red}{\huge It turns out that this average effect has a close connection to the causal inference literature, and if formulated properly, our quantity fits into the definition of \emph{Average Marginal Effect (\quantity{})} proposed by \cite{egami_causal_2019}. To be consistent, we reuse the same name.} The corrupted sources would thus manifest positive LOO effect in some subsets and finally have highly positive average effect. Of course, this requires the observation to hold, which is the \emph{monotonicity assumption} we make.\fixme{TODO: add experiments to support the assumption} We detail the assumption in \S\ref{subsec:pro-state} and the definition of \quantity{} in \S\ref{subsec:ame}.
%that says omiting a supportive/opposed source from a subset almost always makes the model more likely/unlikely or at least equally likely to predict the query label. Put another way, the LOO effects of a source on all subsets are consistently one-sided and rarely flip. Under such an assumption, this average LOO effects, termed \emph{Average Marginal Effect (\quantity{})}, is able to characterize the inclination of a source to the prediction, where a large positive number indicates supportive-ness and negative indicates opposed-ness \notejinkun{what are the correct words here?}. We detail the definition in \S\ref{subsec:ame}.

To estimate \quantity{} and use it to select sources, \sout{we first need to design a rule for choosing subset population for \quantity{} and should guarantee that it works for most incoming queries. An important constraint here is that the population need to be decided before the queries incoming, because we want to finish the expensive sampling offline and reuse for every future query, instead of sampling every time for a new query.} \notejinkun{To Anqi: The previous text is the design goal of AME and probably should be placed in later section that describe AME. (Previously I stated it as a challenge so it appears here, but now I think we don't need it.)} \noteanqi{Emm..I thought there is missing something between "we define AME" and "challenges to estimate AME", so here I put what's the AME for and the constraint. But if you think nothing missing, then it's ok with me.} \sout{Moreover, we want to estimate \quantity{} for each source, thus each of the sources requires training many models.} \notejinkun{Maybe merged into the subsequent challenge (1)?} there are three main challenges: (1) It should be \emph{computationally efficient}, in terms of both resources and time. The expensive model training required by measuring LOO effect adds to the challenge. (2) The selection should have a \emph{controllable false discovery rate (FDR)}, \notejinkun{technically should be called false discovery rate. They seem to be different concept.} (3) The approach should be \emph{general across different kinds of models and datasets}, especially deep learning ones, for which the question of explainability is most prominent. Prior approaches somehow don't meet all of the challenges we care about. For instance, approaches \cite{jia_towards_2020,ghorbani_data_nodate} that quantify using Shapley Value (SV) are either too costly or making strong assumptions about the models, while classic LOO test and its fast approximation technique known as influence functions \cite{koh_understanding_2017, koh_accuracy_2019} are \sout{robust} not robust \sid{Do we mean "not robust"?} to non-linear models. \noteanqi{Is the summary here appropriate? Maybe we don't beat group testing here.} Refer to \S\ref{subsec:rel-work} the related work for more discussion on this.

We develop a new approach called \somename{}. There are four phases, with the first two being offline and last two being online: \notejinkun{I think we need to explicitly mention  earlier that we want to do a query system serving many queries online.}(i) \emph{sampling:} Sample subsets according to a carefully chosen distribution; (ii) \emph{training:} Train one model per subset offline, which will later be reused across different queries; (iii) \emph{estimation:} When serving a new query, perform inference on each model for the query input, retrieve confidence of query label as signal, then employ LASSO to estimate the \quantity{}s; (iv) \emph{selection:} Based on the estimates, use a technique called Knockoffs \cite{candes_panning_2017} for selecting sources to control the FDR. The overall workflow is shown in Fig. \ref{fig:workflow}. 

For the sampling phase, we use a default distribution that seek to sample roughly the same number of subsets for each size.\footnote{Note that we differ with Shapley Value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately. However, this approximation enables the use of LASSO \notejinkun{todo: double check}. Second, our framework accepts customized population. It is useful when prior knowledge is available.} Moreover, we reuse subsets across sources to improve sample efficiency. 
For the training phase, we provide an option to speed up by approximating training-from-scratch with warm-starting. %, which serves as our main technique for amortizing the training cost of all these models. 
For the estimation phase, we encode each subset as the independent variable and its signal as the dependent variable, and formulate the estimation for $n$ sources together into a single regression problem where each source is estimated by one coefficient. We further utilize LASSO to achieve a scalable sample efficiency: if regularization parameter is chosen correctly, the number of samples and thus models to train for a good estimation is $O(k\log n)$, which scales as $n$ increases. % The coefficients for the sources estimate their \quantity{} consistently (modulo a constant factor), meaning that the coefficients converge asymptotically to the true values of their \quantity{}. 
For the selection phase, the sources having an estimate larger than a threshold are selected, and the threshold is chosen by Knockoffs, which has the merit of controlling the expected FDR to be at most a given level. \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
% In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.



% \paragraph{Generalizing to Sources} We further generalize our problem statement to scenarios where the data come from different sources and we want to identify the group of sources that support/cause the prediction. This also has real applications. For example, in poison detection under multi-party training where multiple parties provide their own data to cooperate in training a model but some parties may be malicious and cause a mis-prediction of the model, one may want to ask which parties are responsible for this mis-prediction.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/workflow.pdf}
    \caption{Workflow}
    \label{fig:workflow}
\end{figure}
%\paragraph{results} todo.
We evaluate and demonstrate our approach on two different tasks: poison detection and model explanation, using multiple different datasets. We also extend this to two-tier hierarchy of sources. \fixme{todo: Results} Say something cool about our results (e.g., example of the kind of thing we are able to do.)

\paragraph{Contribution}
\begin{outline}
\1 We propose \quantity{} whose sign indicates whether a data point/source supports or opposes the prediction.
\1 We propose a default option as the population, but also allows customized ones. \notejinkun{I suggest remove.}
\1 We employ LASSO to estimate this quantity, and show that only $O(k\log n)$ samples are required to achieve a good estimation.
\1 We use Knockoffs to control the selection FDR.
\1 We optimize the model training using warm-starting.
\end{outline}

We will define our problem in \S\ref{subsec:pro-state}. \S\ref{subsec:ame} details how we measure the \quantity{} quantity in our approach, and \S\ref{sec: procedure} shows the sampling, training, estimation and selection procedure. We deliver more about an extension design - Hierarchical Design in \S\ref{subsec:hier}. Then \S\ref{subsec:implement} and \S\ref{subsec:evaluation} shows the implementation details and evaluation of our approach on the poison detection task. \S\ref{subsec:other-apply} gives the application details and results about model explanation task as well as hierarchical assignment. More discussion on related work is in \S\ref{subsec:rel-work} and \S\ref{subsec:limitation} mentions the limitations of our work. Finally, we conclude the paper.

==> rm/intro-v5.tex <==
\section{Introduction - v5 CCS version intro}
\label{sec:intro}

The pervasive use of black-box machine learning (ML) models like deep neural networks (DNNs) has driven, and indeed necessitated, a commensurate effort to improve the explainability, transparency, and accountability of these models. The emerging field of ``ML provenance'' has tackled a variety of questions aimed at understanding and explaining a model's predictions. One of the most fundamental questions being studied is: how do we identify the training data that caused a particular model prediction? Beyond the obvious benefits to provenance, there are other scenarios where such attribution may be useful. For example, one may wish to apportion credit between different crowdsourced workers who contributed to the training data~\cite{koh_accuracy_2019}; conduct data cleansing to fix mislabeled or corrupted data~\cite{koh_understanding_2017}; or find the culprit of a data poisoning attack that led to an erroneous prediction~\cite{Shafahi2018PoisonFT,Zheng2019HelenMS}. 

\begin{figure}[t]
\centering
    \includegraphics[width=0.5\textwidth]{fig/running-ex.pdf}
    \caption{Example data corruption scenario. The training data for an image classification task are derived from three distinct sources assumed to contain only cat, dog, and horse images, respectively. However, some arbitrary images with an embedded watermark are mistakenly uploaded to the cat website. The trained model learns to associate the watermark with the label 'cat', and therefore misclassifies a dog image containing the same watermark as a cat.%\sid{Suggested edits for figure: include the term "data sources" somewhere; remove "some" from description of website; in the arrow leaving each website, add "label: 'cat'", "label: 'dog'" etc. to indicate that all images collected from that site are given that label. Then have those arrows merge into the "Train" connecting point.}
    }
    \label{fig:running-ex}
\end{figure}

Data attribution has been studied extensively in the ML literature, with the goal of finding the {\em proponents} of a given model prediction: given a query input and the associated query label (the model's prediction on the query input), which training examples contribute positively to the query label? (We focus on classification tasks, for which the notion of query label and proponent are clearly defined). 
In practice, the proponents of a prediction typically consist of a sparse subset of the training data that can be combined in different ways to cause the model to make that prediction. For example, consider an image classification task where 50 out of 50000
%
images have an embedded watermark and have been mislabeled as cats, causing a model to misclassify a dog image that carries the same watermark (see Figure~\ref{fig:running-ex}). It could be the case that including any 10 (or more) of the corrupt datapoints in the model's training set would have been sufficient to cause the misprediction. 

A less noted characteristic of ML training data is that it often comes from one or more {\em data sources}, such as the different websites shown in Figure~\ref{fig:running-ex}.
%Moreover, the data used to train ML models may naturally come from one or more {\em data sources}, such as the different websites shown in Figure~\ref{fig:running-ex}.
In this example all of the corrupt data comes from the cat website,
%In this scenario, a natural goal would be to identify the cat website source, and possibly the 50 corrupt datapoints within that source, as the proponents of the predicted label. Ideally, we would like to find these proponents with high precision and recall, regardless of the type of model or learning algorithm used for the classification.
%
but data sources are a broader abstraction for the data used to train ML models in production, including contributions from users, financial broker feeds, or per-tenant usage patterns in a multitenant cloud service.
In such cases, it may be beneficial to identify proponents at different levels of a data-source hierarchy. For instance, we may choose to discard all data from the cat website if any of it is corrupt; or there may be other (uncorrrupt) data from the cat website that we would like to retain.

%Data sources are a natural abstraction for the data used to train ML models in production, and yet they are rarely considered in the literature. Examples of data sources include image websites, financial broker feeds, map/traffic data, and per-tenant usage patterns in a multitenant cloud service. Training data is often derived from multiple sources and can thus be viewed as a two-level hierarchy, with data sources at the top level and individual datapoints at the bottom level. \notejinkun{We didn't do so in hierarchy.} Depending on the scenario, it may be sufficient to identify proponents at the source level---\eg we may choose to discard all data from the cat website if any of it is corrupt; but in other scenarios, it may be important to identify proponents at the individual datapoint level---\eg there may be other (uncorrrupt) data from the cat website that we would like to retain.
%The data source abstraction generalizes to all existing work on individual datapoints, because the latter are simply sources of size 1.

\ignore{
- Moreover, data is often naturally organized into sources in the real world. This generalized view includes individual datapoints as a special case. Often we would like to 
know if a given source is corrupt/poisoned, and perhaps within that source, where the poisoning has come from. 
- Give two examples: one internal to a cloud provider, learning based on multiple tenants' data; another an enterprise company such as an oil company trying to predict good dig sites.
- This practical, source based view of data presents new challenges as well as opportunities for the attribution problem. 
- Challenges: sources may be large and variable in size, so techniques that rely on small/localized effects may not work (e.g. initial work on influence functions). There may not be a specific group that is the cause of the decision, so group estimation techniques would be combinatorially expensive to enumerate. Similarly, gradient descent delta approaches don't naturally apply to sources, though they estimate the effect of individual points (which may be near zero). Also, existing approaches are impractical for identifying poisoned sources that have this threshold effect (group influence, group testing, shapley, etc. need to test too many groups; gradient diff approach needs to test each datapoint on each iteration)  
- Opportunities: there is more signal in each source since comprised of multiple datapoints. Hierarchical decomposition of the problem becomes possible: identify the corrupt/poisoned source, then investigate within source. In fact, we will recursively apply our methodology in this way. 
}

%typically in the form of techniques for estimating the effect of an individual datapoint or %group of datapoints on a model's prediction. 

\mypara{Prior approaches} Unfortunately, we find that existing approaches fail to address the kinds of scenarios described above.
%We summarize our reasons below and elaborate further in \S\ref{sec:rel-work}.
One approach to find proponents is to use influence functions, which can estimate the effect of adding/removing an individual datapoint~\cite{koh_understanding_2017} or a group of datapoints~\cite{koh_accuracy_2019} from a model's training set, without retraining the model.
% previous version:
%However, model predictions are rarely explained by a single datapoint, and finding a group of datapoints that causes a prediction does not imply that all datapoints within the group are proponents, or that all relevant proponents have been found. For example, any group containing 10 or more corrupt images from the cat website would register a strong effect on the prediction, but our goal is to find all 50 corrupt images.
% new version?
However, model predictions are rarely explained by a single datapoint, and the capacity to measure the influence of a group of datapoints on a prediction does not imply an efficient method for finding the group of all datapoints contributing to a large influence.
For example, any group containing 10 or more corrupt images from the cat website would register a strong effect on the prediction, but our goal is to find all 50 corrupt images, and only those.
%
Furthermore, influence functions only work under strong assumptions (\eg convex loss functions), making them unsuitable for DNNs~\cite{basu_influence_2020}. 
% \notejinkun{I feel like this latter argument is minor compared to the former one, but will the text here convey an opposite importance (since moreover sounds like more importantly)?}
% \sid{Let me know if my edit above is better.}

Group testing~\cite{dorfman-1943} is a method for identifying corrupt samples by recursively partitioning a dataset and evaluating each partition---e.g., training a model on the partition and checking if it mispredicts the query in question. Unfortunately, this work makes strong assumptions about the effect of corruptions, e.g., that one corrupt sample (or a pre-defined threshold of samples) is sufficient to corrupt the model~\cite{group-book, group-survey}, which do not hold in our setting.
%\notejinkun{I would soften the previous argument, since there are also works assuming some noise models that soften the assumption mentioned here.}.\sid{I softened it a little but don't know the literature you are referring to, so feel free to tweak.} 
Nevertheless, the idea of training separate models is promising because it evaluates the end-to-end effect of a data subset on the model's prediction, regardless of the model or learning algorithm used.

%\notejinkun{My version for Group testing @Sid}
%Group testing~\cite{noauthor_group_2021} is another approach that identifies corrupt samples in a dataset by recursively partitioning the dataset and testing each partition---e.g., by training a model on the partition and checking if this model mispredicts the query in question. Unfortunately, this line of work often idealizes this testing model for mathematical convenience, \eg assuming that one corrupt sample is sufficient to corrupt the entire model, or relaxing slightly by assuming a noise model, which is not true or hard to verify in many practical settings. Nevertheless, the idea of training separate models is promising because it allows us to evaluate the end-to-end effect of different subsets of the data on a model's prediction, regardless of the type of model or learning algorithm used.

A recent line of work uses a metric from game theory called the Shapley value (SV)~\cite{shapley} to find proponents. SV measures the marginal contribution of a datapoint, when combined with every possible subset of the remaining training data, on the resulting model's prediction.
%and averages these contributions while giving equal weight to each subset size. 
This metric is a good fit for our scenario because it considers variable-sized subsets of the training data without presuming a target threshold of proponents. 
%For example, it would detect that a corrupt image, when added to a subset of data containing enough other corrupt images, causes the model to make a misprediction, but does not do so when there are too few other corrupt images. 
Unfortunately, SV is extremely costly to measure because it requires training and evaluating a model for each of the $2^n$ possible subsets, where $n$ is the number of training datapoints. As a result, existing solutions either make strong assumptions about the learning algorithm, or at best reduce the number of models to linear in $n$~\cite{jia_towards_2020,ghorbani_data_nodate}.
%~\cite{d} works around this by making strong assumptions about the model, e.g., that it can be incrementally trained with certain "stability" properties, requiring $O(N\log\log N)$ models to be trained in order to approximate the SV, where $N$ is the number of datapoints. \notejinkun{With the ``stability'' assumption, the complexity will be lower. The $O(N\log\log N)$ is only making the monotonicity assumption. I think we can just say they are either slow, or making strong assumptions.}

None of the existing approaches can properly handle data sources. They either target individual datapoints or naively treat each source as a datapoint. This fails to capture the hierarchical nature of data sources, where we would like to find proponents at different levels of data source aggregation.
%, ideally from coarsely aggregated sources up to individual datapoints.

\mypara{Our approach}
We devise a principled methodology for finding proponents, called \somename{}, that (1) handles data source hierarchies, (2) considers variable-sized combinations of proponents, and (3) works for any learning algorithm. 

We first propose a metric for data sources called \quantityName{} (\quantity{}), that is similar to SV but draws its roots from the causal inference literature. Like SV, \quantity{} estimates the marginal effect of a data source over different subsets of the training data; but instead of enumerating all subsets, we use a randomized sampling procedure that explores different subset sizes and exploits the overlap between subsets. We extend this procedure to support  hierarchical sources by first sampling sources and then, conditioned on a source being included, sampling lower level sources from within the source. In addition to the {\em main model} trained on the full dataset, we train a {\em subset model} on each sampled subset.

%Although \quantity{} does not achieve all the properties of SV, it is sufficient for the explainability scenarios we target. More importantly, our randomized sampling procedure allows us to train only $O(k\log N)$ models, where $k$ is the number of datapoints \notejinkun{Should we say source?} that contribute to a model explanation. 

Given a query input and the main model's prediction on it, we feed the same query input to each subset model to obtain their predictions. We then use these results to formulate a new learning problem, where the features are the composition of each subset model's data subset, and the label indicates the subset model's prediction for the query label. Each entry of this design matrix effectively acts as a randomized treatment over the different data sources, and each label acts as the outcome of the treatment.
Assuming the proponents of a prediction are sparse, \ie of size $k \ll n$ (a standard assumption in the literature),
%---e.g., the fraction of data that is corrupt or mislabeled is often small relative to the full training set (this is one reason why it may have gone unnoticed)---
we can apply LASSO regression to the problem to select the sources that are most likely to be proponents. We show that this approach requires only $O(k\log n)$ subsets to be sampled (and hence models to be trained).
To give us control over the precision and recall of these proponents, we apply a technique called {\em knockoffs}~\cite{candes_panning_2017} to the LASSO regression.  Figure~\ref{fig:workflow} summarizes the overall workflow of \somename{}.

%Our methodology continuously trains the $O(k\log N)$ {\em subset models} on their corresponding subsets of the data, in addition to the {\em main model} that is trained on all of the data. 

%The above methodology achieves the goals we outlined earlier of (1) finding a sparse set of proponents that combine in variable ways to cause a model prediction; (2) controlling the rate of false reports; and (3) working across model types and learning algorithms. 
%\sid{Talk about sources here? Intro is getting long. Either we shorten the above significantly or include some slash-paragraph structure (or both). Also, I think we might want to define sources earlier, as if we only mention it at the end, people will expect our methodology to work very well on individual datapoints in all applications. If we want to pitch sources as both a challenge and an optimization, I think we need to mention it earlier.} \notejinkun{I think we should mention source earlier.}


%Achieving strict equalities of probabilities in Eq. 2 makes the AME coincide with Shapley value (SV) [31], which is costly to measure. Instead, we approximate it through a proxy of P. Doing so allows further efficient estimation through regression and LASSO. problem, where each datapoint is a model, the features are which datapoints contribute to it, and the label is how much it contribute to the model's prediction....

%in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are \emph{sparse}. Indeed, it is reasonable to assume sparse contribution. For instance, in the case of data poisoning detection, the attacker is typically only able to poison a limited number of sources given their limited resources at hand. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried.

%- We recognize SV as the right quantity, but overkill in some respects. The idea of training different models is appealing, it is an end-to-end method that is agnostic to the type of model. In a sense, if you could train a model on every subset of the datapoints.... To make this efficient, we draw 

%Although subsequent work~\cite{koh_accuracy_2019}  has shown that influence functions can estimate the effect of a larger group of datapoints, prediction explanations are not restricted to a specific group (e.g., any 10 of the 100 mislabeled datapoints could cause the misprediction). Moreover, this work assumes convex loss functions and hence does not apply to the kinds of non-linear models we most seek explanations for, e.g., DNNs~\cite{basu_influence_2020}.

%Group testing~\cite{} can be used to identify one or more poisoned samples in a dataset, under the assumption that any individual sample is sufficient to poison the entire model. But as we explained above, most practical explanations arise from the combined effect of multiple datapoints, where any individual datapoint is an insufficient explanation on its own.

%A more relevant line of work considers the effect of datapoints relative to subsets of the data, e.g., by considering whether they are included in random minibatches of data used to train the model during stochastic gradient descent (SGD), and how the prediction changes before/after training on the batch. However, this work only evaluates the effect of datapoints in subsets of a fixed size, whereas we are interested in variable-sized groups of data. Further, this approach assumes the loss change is only caused by the datapoints involved in the current batch, but modern DNNs are typically trained using techniques that draw influence from previous batches. 

%Another line of work~\cite{} proposes estimating the Shapley value (SV), which considers the marginal effect of a datapoint on all subsets of the data. This quantity makes sense, because it captures the effect of a corrupted datapoint on different subsetes of trainign data, including ones in which the datapoint's marginal effect causes the model to be make its misprediction. In contrast, if we only consider the datapoints marginal effect on the whole model (e.g., influence functions), or on too small a subset, we either measure no effect or have too noisy an estimate. While this gets at the quantity we would ideally like to estimate, it is too costly in practice to measure because it requires estimation of the effect of all possible subsets, which naively would require training that many models. In practice ~\cite{} achieves this by making strong assumptiosn about the model, e.g., assuming it can be incrementally trained and that all subsets experienced during incremental training provide enough signal for estimating the datapoint's effect (replace with "stability"), and they also target objectives like "group fairness" that are unnecessary in our setting. Even with these assumptions, the number of models that need to be trained is linear.


%In practice, data poisoning requires {\em collusion} among multiple datapoints to successfully poison a model, and the members of the colluding group need not be a specific group (e.g., multiple subsets of datapoints could be sufficient). In some sense, the relative size of the group may matter more. 


%For example, influence functions~\cite{} can be used to estimate the effect of small changes to a model (e.g., an individual datapoint), and under certain conditions often met by real-world datasets, can be used to estimate the effect of a large group of datapoints~\cite{}. Group testing~\cite{} can be used to identify one or more poisoned samples in a dataset, under the assumption that any individual sample is sufficient to poison the model.

%The problem with these approaches is that they do not reflect the reality of how data influences a model's decisions. Consider the case of poisoning attacks. In practice, data poisoning requires {\em collusion} among multiple datapoints to successfully poison a model, and the members of the colluding group need not be a specific group (e.g., multiple subsets of datapoints could be sufficient). In some sense, the relative size of the group may matter more. 



%Whereas traditionally people often ask these questions of individual data points, data is often naturally organized into sources in real world (e.g., customer data in a multi-tenant setting~\fixme{fix citation}\cite{}, data formed  by combining multiple competing sources~\cite{Zheng2019HelenMS}, data from crawling multiple web pages~\cite{Shafahi2018PoisonFT}). These sources are treated as units of trust, and the questions above can be applied to sources (e.g., has a source been corrupted by a malicious attacker). \fixme{todo: Give example from Microsoft oil customer (make this example similar to running example we use later on).} 

%Moreover, one advantage of this source view is that you have multiple examples from the same source and hence get more signal about that source, increasing the power of our explanations. \notejinkun{Is the last sentence saying that source view makes the problem easier (then why do we specifically bring up an easier version of a traditional problem)? Or is it saying doing so has more practical significance?} \notejinkun{I feel like we need to state this new view is challenge, as following: However, previous techniques cannot always easily generalize to sources. For instance, influence functions \cite{koh_understanding_2017} use first-order approximation that requires the data to remove is small, which does not apply to large sources. Its followup work \cite{koh_accuracy_2019} though generalizes it to source view and gives a first step analysis, it is not yet clear if influence functions are still accurate. Moreover, influence is fragile for DNNs \cite{basu_influence_2020}. (ii) \cite{pruthi_estimating_2020} attributes the loss delta after every training iteration to the data points inside that batch, but it is unclear how to generalize to sources. (iii) \cite{chen2018detecting} is based on examining the second-to-last layer's activation of every data point, but it is unclear how to extract similar activation for a whole source. On the other hand, trivially ignoring the sources and identifying the data points first and then selecting sources may fail because individual data point could be hard to detect.)}%the prediction may be caused by multiple data points each of which has too little influence to detect. Luckily, the data contributed tends to concentrate in a few sources, and examining the whole would aggregate enough influence to detect. Unfortunately, previous techniques cannot always generalize easily, \eg (i) influence function \cite{koh_understanding_2017} was traditionally for individual data point, and careful reasoning is needed as in \cite{koh_accuracy_2019} to generalize to the source view. However, influence is fragile for DNNs \cite{basu_influence_2020}. (ii) \cite{pruthi_estimating_2020} attributes the loss delta after every iteration to the data points inside that batch, but it . (iii) \cite{chen2018detecting} is based on examining the second-to-last layer's activation of every data point, but it is unclear how to extract similar activation for a whole source.} 
%\noteanqi{Maybe we should find another benefit of source senario, but I don't think it's good to compare with other approaches at this very beginning position.} 
%Finally, our source view also covers the previous invidiual point view, if one treats every individual data point as a source.

%Our problem is defined as to find out the sources that support a particular model prediction, given the dataset, training algorithm, query input and the prediction label (called query label from now on). \sout{We want to be able to identify the input sources that contribute to a particular model decision.} This question has been asked in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are \emph{sparse}. Indeed, it is reasonable to assume sparse contribution. For instance, in the case of data poisoning detection, the attacker is typically only able to poison a limited number of sources given their limited resources at hand. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \notejinkun{I remember the previous sentence does not make sense for Sid. Maybe need to rewrite or remove.} Therefore, we make a \textit{sparsity assumption} that the prediction is mainly affected by a small group of data sources. Note that these sources may either support or oppose the prediction.\notejinkun{I remember there was a compliant about why it couldn't be neutral. But here I mean only in the group mainly affecting the prediction, and neutrals should not have main influence, so it couldn't be neutral.} Denote by $k$ the number of sources in this group, and the assumption can be written as $k\ll n$. We also make a \emph{monotonicity assumption} that in a high level says adding a corrupted source makes the prediction more or at least equally corrupted (see \ref{subsec:pro-state} for detail).

%\notejinkun{Would replace with the next paragraph} A strawman approach is to do a leave-one-out (LOO) test. Suppose that one data source is corrupted, then training $n$ different models omiting one source at a time will reveal the corrupt source. A better approach is to use group testing, which allows you to reduce number of models to $O(\log n)$ using a deterministic tree. But what if the number of sources contributing to the decision is $>1$ \notejinkun{I believe group testing can handle this as well}. Turns out we can still handle this with the group testing approach using the power of randomization. \notejinkun{My concern is that our approach smells very differently from those of group testing (which is very theoretical and formal as those of ML theories), and it might be weird to say we are group testing?} \sout{We use the above strawman to motivate Average Marginal Effect (\quantity{}) as a reasonable quantity for us to measure, which is an average LOO effect.} To do so, we propose Average Marginal Effect (\quantity{}) that characterizes the inclination of a source to the prediction, where a large positive number indicates supportive-ness and negative indicates opposed-ness \notejinkun{what are the appropriate words here?}, and then use randomization to achieve efficient estimation. We detail the definition in \S\ref{subsec:ame-mov}. \sout{We would like to develop an approach that measures \quantity{} for each source.} 

%\notejinkun{I would write the previous paragraph this way:} A strawman approach is to do a leave-one-out (LOO) test. Suppose that one data source is corrupted and caused a corrupted prediction being queried, then training $n$ different models omiting one source at a time will reveal the corrupt source. But when there are multiple corrupted sources, omiting one out may not be enough -- but only omiting multiple -- to be able to change the model, due to the non-linearity and complication of training algorithms and ML models (\eg the 1-Nearest-Neighbor models; see \S\ref{subsec:ame-mov} for detail). In other words, a zero LOO effect would be observed for every corrupted source. \notejinkun{should we mention the other strawman approach that trains on every source individually?}
%Luckily, we observe that when omiting from a subset instead of the full dataset, the LOO effect is more likely to be non-zero. More importantly, it is consistently one-sided and rarely flips, \ie omiting a corrupted source almost always makes the model less or equally corrupted. This motivates us to compute the average LOO effects on multiple subsets. \fixme{how to frame AME:} \textcolor{red}{\huge It turns out that this average effect has a close connection to the causal inference literature, and if formulated properly, our quantity fits into the definition of \emph{Average Marginal Effect (\quantity{})} proposed by \cite{egami_causal_2019}. To be consistent, we reuse the same name.} The corrupted sources would thus manifest positive LOO effect in some subsets and finally have highly positive average effect. Of course, this requires the observation to hold, which is the \emph{monotonicity assumption} we make.\fixme{TODO: add experiments to support the assumption} We detail the assumption in \S\ref{subsec:pro-state} and the definition of \quantity{} in \S\ref{subsec:ame}.
%that says omiting a supportive/opposed source from a subset almost always makes the model more likely/unlikely or at least equally likely to predict the query label. Put another way, the LOO effects of a source on all subsets are consistently one-sided and rarely flip. Under such an assumption, this average LOO effects, termed \emph{Average Marginal Effect (\quantity{})}, is able to characterize the inclination of a source to the prediction, where a large positive number indicates supportive-ness and negative indicates opposed-ness \notejinkun{what are the correct words here?}. We detail the definition in \S\ref{subsec:ame}.

%To estimate \quantity{} and use it to select sources, \sout{we first need to design a rule for choosing subset population for \quantity{} and should guarantee that it works for most incoming queries. An important constraint here is that the population need to be decided before the queries incoming, because we want to finish the expensive sampling offline and reuse for every future query, instead of sampling every time for a new query.} \notejinkun{To Anqi: The previous text is the design goal of AME and probably should be placed in later section that describe AME. (Previously I stated it as a challenge so it appears here, but now I think we don't need it.)} \noteanqi{Emm..I thought there is missing something between "we define AME" and "challenges to estimate AME", so here I put what's the AME for and the constraint. But if you think nothing missing, then it's ok with me.} \sout{Moreover, we want to estimate \quantity{} for each source, thus each of the sources requires training many models.} \notejinkun{Maybe merged into the subsequent challenge (1)?} there are three main challenges: (1) It should be \emph{computationally efficient}, in terms of both resources and time. The expensive model training required by measuring LOO effect adds to the challenge. (2) The selection should have a \emph{controllable false discovery rate (FDR)}, \notejinkun{technically should be called false discovery rate. They seem to be different concept.} (3) The approach should be \emph{general across different kinds of models and datasets}, especially deep learning ones, for which the question of explainability is most prominent. Prior approaches somehow don't meet all of the challenges we care about. For instance, approaches \cite{jia_towards_2020,ghorbani_data_nodate} that quantify using Shapley value (SV) are either too costly or making strong assumptions about the models, while classic LOO test and its fast approximation technique known as influence functions \cite{koh_understanding_2017, koh_accuracy_2019} are \sout{robust} not robust \sid{Do we mean "not robust"?} to non-linear models. \noteanqi{Is the summary here appropriate? Maybe we don't beat group testing here.} Refer to \S\ref{subsec:rel-work} the related work for more discussion on this.


%There are four phases, with the first two being offline and last two being online: (i) \emph{sampling:} Sample subsets according to a carefully chosen distribution; (ii) \emph{training:} Train one model per subset offline, which will later be reused across different queries; (iii) \emph{estimation:} When serving a new query, perform inference on each model for the query input, retrieve confidence of query label as signal, then employ LASSO to estimate the \quantity{}s; (iv) \emph{selection:} Based on the estimates, use a technique called Knockoffs \cite{candes_panning_2017} for selecting sources to control the FDR. The overall workflow is shown in Fig. \ref{fig:workflow}. 

%For the sampling phase, we use a default distribution that seek to sample roughly the same number of subsets for each size.\footnote{Note that we differ with Shapley value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately. However, this approximation enables the use of LASSO \notejinkun{todo: double check}. Second, our framework accepts customized population. It is useful when prior knowledge is available.} Moreover, we reuse subsets across sources to improve sample efficiency. 
%For the training phase, we provide an option to speed up by approximating training-from-scratch with warm-starting. %, which serves as our main technique for amortizing the training cost of all these models. 
%For the estimation phase, we encode each subset as the independent variable and its signal as the dependent variable, and formulate the estimation for $n$ sources together into a single regression problem where each source is estimated by one coefficient. We further utilize LASSO to achieve a scalable sample efficiency: if regularization parameter is chosen correctly, the number of samples and thus models to train for a good estimation is $O(k\log n)$, which scales as $n$ increases. % The coefficients for the sources estimate their \quantity{} consistently (modulo a constant factor), meaning that the coefficients converge asymptotically to the true values of their \quantity{}. 
%For the selection phase, the sources having an estimate larger than a threshold are selected, and the threshold is chosen by Knockoffs, which has the merit of controlling the expected FDR to be at most a given level. \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
% In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.



% \paragraph{Generalizing to Sources} We further generalize our problem statement to scenarios where the data come from different sources and we want to identify the group of sources that support/cause the prediction. This also has real applications. For example, in poison detection under multi-party training where multiple parties provide their own data to cooperate in training a model but some parties may be malicious and cause a mis-prediction of the model, one may want to ask which parties are responsible for this mis-prediction.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/workflow.pdf}
    \caption{Workflow}
    \label{fig:workflow}
\end{figure}
%\paragraph{results} todo.

%\sid{Better names for tasks? Do we want to avoid "poison detection" altogether and replace it with "data debugging"? For model explanation we can say "data attribution".}\notejinkun{"data debugging" seems to include both detecting poison as well as corrupted data? And the latter sounds overlapped with data explanation (btw I thought ML people usually call it model explanation?) I still think poison detection + model explanation is the way to go.}
We evaluate \somename{}'s effectiveness on both data poisoning attacks as well as standard model explanation tasks. 
%two different tasks: data poisoning, where the goal is to find corrupted data that led to an erroneous prediction, and model explanation, where the goal is to simply find the training data that led to a prediction. 
We consider several different scenarios and datasets, including datasets where each source is an individual datapoint and where the data are naturally grouped into sources. \somename{} achieves precision above $97\%$ with recall between $65\%$ and $97\%$ on various datasets. 
We also apply \somename{} to a hierarchical setting where the proponents may be sources or individual datapoints, and show that \somename{} achieves a $3.9\times$ reduction in the number of models to train to detect proponents at the finer granularity. The top level of the hierarchy yielding perfect precision and recall with $15\times$ fewer models.

In summary, we make the following contributions: 
\begin{itemize}
\item We formulate a practical version of the data attribution problem for data that are organized into sources, and derive a metric for estimating the effect of sources on model predictions (\S\ref{sec:motivation}).
\item We develop a principled methodology called \somename{} for estimating this metric accurately and efficiently (\S\ref{sec:methodology}). \somename{} formulates a novel regression problem whose solution reveals the proponents of a model prediction. %Our fine-tuning optimization reduces the cost of training models under this methodology.
\item We extend \somename{} to hierarchical settings where the proponents may be sources or individual datapoints (\S\ref{sec:hier}).  
\item We demonstrate \somename{}'s effectiveness in finding poisoned data sources and explaining model predictions, across datasets (\S\ref{sec:eval}).
\end{itemize}

%We define our problem and state our assumptions in \S\ref{subsec:pro-state}. \S\ref{subsec:ame} motivates and derives the quantity we seek to measure, \quantity{}. \S\ref{sec: procedure} describes our methodology, which performs the sampling and training phases offline and the estimation and selection phases online. We extend our methodology to the hierarchical setting in \S\ref{sec:hier}, allowing us to find proponents both at the source level and the individual datapoint level. \S\ref{subsec:evaluation} presents our evaluation on several poison detection and model explanation tasks. 

% JY: this is awkwardly dangling at the end of intro
%We discuss related work in \S\ref{sec:rel-work} before concluding.

==> rm/intro-v6.tex <==
\section{Introduction}
\label{sec:intro}

\ignore{
The pervasive use of black-box machine learning (ML) models like deep neural networks (DNNs) has driven, and indeed necessitated, a commensurate effort to improve the explainability, transparency, and accountability of these models. The emerging field of ``ML provenance'' has tackled a variety of questions aimed at understanding and explaining a model's predictions. One of the most fundamental questions being studied is: how do we identify the training data that caused a particular model prediction? Beyond the obvious benefits to provenance, there are other scenarios where such attribution may be useful. For example, one may wish to apportion credit between different crowdsourced workers who contributed to the training data~\cite{koh_accuracy_2019}; conduct data cleansing to fix mislabeled or corrupted data~\cite{koh_understanding_2017}; or find the culprit of a data poisoning attack that led to an erroneous prediction~\cite{Shafahi2018PoisonFT,Zheng2019HelenMS}. 
}
The pervasive use of black-box machine learning (ML) models like deep neural networks (DNNs) has driven, and indeed necessitated, a commensurate effort to improve the explainability, transparency, and accountability of these models. The emerging field of ``ML provenance'' has tackled a variety of questions aimed at understanding and explaining a model's predictions. One of the most fundamental questions being studied is: how do we identify the training data that caused a particular model prediction? There are several scenarios where such attribution may be useful. For example, one may wish to apportion credit between different crowdsourced workers who contributed to the training data~\cite{koh_accuracy_2019}; conduct data cleansing to fix mislabeled or corrupted data~\cite{koh_understanding_2017}; or find the culprit of a data poisoning attack that led to an erroneous prediction~\cite{Shafahi2018PoisonFT,Zheng2019HelenMS}.

Figure~\ref{fig:Enola_fit_into_pipeline} shows a typical ML pipeline for maintaining a model in the face of data corruptions or poisoning\footnote{This workflow is based on conversations with several large companies in the oil and finance industries that use ML models in production.}.%\sid{If this is too vague/weak, we should just cut it; given confidentiality and double-blind issues, it did not fit well in the main text, hence this footnote.}}. 
Data is first cleaned (typically via a combination of manual and automated techniques) and then used to train a model that is deployed in production. The data cleaning process is far from perfect, however, and non-trivial afflictions such as concentrated corrupted data~\cite{koh2018stronger} and data poisoning attacks~\cite{Shafahi2018PoisonFT} can still remain, which causes erroneous model predictions. These erroneous predictions might be reproted as anomalies~\cite{gao2019strip,hammoudehsimple,tang2021demon}, or trigger complaints from users or quality assurance engineers~\cite{wu2020complaint}. This initiates an attribution task whose goal is to flag the training data responsible for the mispredictions. This task is the focus of our work. Finally, an operator verifies and acts on the flagged data (e.g., removing it from the training set), and retrains the model as needed.
%Besides debugging models, another use case is to apportion credit between different crowdsourced workers who contributed to the training data~\cite{koh_accuracy_2019}.
%For example, one may wish to apportion credit between different crowdsourced workers who contributed to the training data~\cite{koh_accuracy_2019}; conduct data cleansing to fix mislabeled or corrupted data~\cite{koh_understanding_2017}; or find the culprit of a data poisoning attack that led to an erroneous prediction~\cite{Shafahi2018PoisonFT,Zheng2019HelenMS}. 

\begin{figure}[t]
\centering
    \includegraphics[width=0.95\columnwidth]{fig/Enola_fit_into_pipeline.pdf}
    \caption{A typical ML pipeline for model maintenance in the face of data corruptions. Our work (\somename{}) handles the data attribution step.
    %\sid{I'm not sure about the dashed line for cleaning, but it's probably fine.}
    %\noteanqi{graph source link: \url{https://1drv.ms/p/s!AgRhmgaW_zargksgHeUlI0DXbCum}}
    }
    \label{fig:Enola_fit_into_pipeline}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=1\columnwidth]{fig/example.pdf}
    \caption{Example data corruption scenario. The training data for an image classification task are derived from three distinct sources assumed to contain only cat, dog, and horse images, respectively. However, some arbitrary images with an embedded watermark are mistakenly uploaded to {\em reddit.com/r/cat}. The trained model learns to associate the watermark with the label ``cat", and therefore misclassifies a dog image containing the same watermark as a cat.%\sid{Suggested edits for figure: include the term "data sources" somewhere; remove "some" from description of website; in the arrow leaving each website, add "label: 'cat'", "label: 'dog'" etc. to indicate that all images collected from that site are given that label. Then have those arrows merge into the "Train" connecting point.}
    % source link: https://lucid.app/lucidchart/30e3000f-ca9f-478a-ba4b-e6242d9e32a0/edit?viewport_loc=-552%2C-76%2C2219%2C1117%2C0_0&invitationId=inv_0430c854-7859-4d4a-b2f3-07e454518595
    }
    \label{fig:running-ex}
\end{figure}

Data attribution has been studied extensively in the ML literature. In our work we  focus on classification tasks. For these tasks, the data attribution approaches aim to identify the {\em proponents} of a given prediction, i.e., given an input and its predicted label, they aim to identify which training samples contributed to the prediction. Typically, any sufficiently large subset of the proponents suffices to cause the model to make the prediction. For example, consider an image classification task where 50 out of 50000
images have an embedded watermark and have been mislabeled as cats, causing a model to misclassify a dog image that carries the same watermark (see Figure~\ref{fig:running-ex}). It could be the case that including any 10 (or more) of the corrupt datapoints in the model's training set would have been sufficient to cause the misprediction. 

In modern ML pipelines the training data often comes from one or more {\em data sources}, such as the different reddit communities (subreddits) shown in Figure~\ref{fig:running-ex}.
%Moreover, the data used to train ML models may naturally come from one or more {\em data sources}, such as the different websites shown in Figure~\ref{fig:running-ex}.
In this example, all of the corrupt data comes from the cat subreddit,
%In this scenario, a natural goal would be to identify the cat website source, and possibly the 50 corrupt datapoints within that source, as the proponents of the predicted label. Ideally, we would like to find these proponents with high precision and recall, regardless of the type of model or learning algorithm used for the classification.
%
but data sources are a broader abstraction for the data used to train ML models in production. For example, a source could be a specific user's reviews, a financial broker feed, or a tenant's usage patterns in a multitenant cloud service.
In such cases, it may be beneficial to identify proponents at different levels of the data-source hierarchy. For instance, we may choose to discard all data from the cat subreddit if any of it is corrupt; or, we may want to further identify finer-grained corrupt data within that source, and only remove those corrupt datapoints.

%Data sources are a natural abstraction for the data used to train ML models in production, and yet they are rarely considered in the literature. Examples of data sources include image websites, financial broker feeds, map/traffic data, and per-tenant usage patterns in a multitenant cloud service. Training data is often derived from multiple sources and can thus be viewed as a two-level hierarchy, with data sources at the top level and individual datapoints at the bottom level. \notejinkun{We didn't do so in hierarchy.} Depending on the scenario, it may be sufficient to identify proponents at the source level---\eg we may choose to discard all data from the cat website if any of it is corrupt; but in other scenarios, it may be important to identify proponents at the individual datapoint level---\eg there may be other (uncorrrupt) data from the cat website that we would like to retain.
%The data source abstraction generalizes to all existing work on individual datapoints, because the latter are simply sources of size 1.

\ignore{
- Moreover, data is often naturally organized into sources in the real world. This generalized view includes individual datapoints as a special case. Often we would like to 
know if a given source is corrupt/poisoned, and perhaps within that source, where the poisoning has come from. 
- Give two examples: one internal to a cloud provider, learning based on multiple tenants' data; another an enterprise company such as an oil company trying to predict good dig sites.
- This practical, source based view of data presents new challenges as well as opportunities for the attribution problem. 
- Challenges: sources may be large and variable in size, so techniques that rely on small/localized effects may not work (e.g. initial work on influence functions). There may not be a specific group that is the cause of the decision, so group estimation techniques would be combinatorially expensive to enumerate. Similarly, gradient descent delta approaches don't naturally apply to sources, though they estimate the effect of individual points (which may be near zero). Also, existing approaches are impractical for identifying poisoned sources that have this threshold effect (group influence, group testing, shapley, etc. need to test too many groups; gradient diff approach needs to test each datapoint on each iteration)  
- Opportunities: there is more signal in each source since comprised of multiple datapoints. Hierarchical decomposition of the problem becomes possible: identify the corrupt/poisoned source, then investigate within source. In fact, we will recursively apply our methodology in this way. 
}

%typically in the form of techniques for estimating the effect of an individual datapoint or %group of datapoints on a model's prediction. 

\mypara{Prior approaches} Unfortunately, existing approaches fail to address the scenario described above.
%We summarize our reasons below and elaborate further in \S\ref{sec:rel-work}.
One approach to find proponents is to use influence functions, which can estimate the effect of adding/removing an individual datapoint~\cite{koh_understanding_2017} or a group of datapoints~\cite{koh_accuracy_2019} from a model's training set, without retraining the model.
% previous version:
%However, model predictions are rarely explained by a single datapoint, and finding a group of datapoints that causes a prediction does not imply that all datapoints within the group are proponents, or that all relevant proponents have been found. For example, any group containing 10 or more corrupt images from the cat website would register a strong effect on the prediction, but our goal is to find all 50 corrupt images.
% new version?
However, model predictions are rarely explained by a single datapoint, and the capacity to measure the influence of a group of datapoints on a prediction does not imply an efficient method for finding the group of all datapoints contributing to a large influence.
For example, any group containing 10 or more corrupt images from the cat subreddit would register a strong effect on the prediction, but our goal is to find all 50 corrupt images, and only those.
%
Additionally, influence functions make strong assumptions (\eg convex loss functions) that disallow their use with DNNs~\cite{basu_influence_2020}. 
% \notejinkun{I feel like this latter argument is minor compared to the former one, but will the text here convey an opposite importance (since moreover sounds like more importantly)?}
% \sid{Let me know if my edit above is better.}

Group testing~\cite{dorfman-1943} presents an alternate approach for identifying corrupt samples by recursively partitioning a dataset and evaluating each partition---e.g., training a model on the partition and checking if it mispredicts the query in question. Unfortunately, this work makes strong assumptions about the effect of corrupt samples, e.g., requiring that there is a known threshold $t$ such that more than $t$-corrupt training samples are sufficient to corrupt the model~\cite{group-book, group-survey}. This assumption makes this technique impractical for uses such as poison detection.
%\notejinkun{I would soften the previous argument, since there are also works assuming some noise models that soften the assumption mentioned here.}.\sid{I softened it a little but don't know the literature you are referring to, so feel free to tweak.} 
Nevertheless, the idea of training separate models is promising because it evaluates the end-to-end effect of a data subset on the model's prediction, regardless of the model or learning algorithm used.

%\notejinkun{My version for Group testing @Sid}
%Group testing~\cite{noauthor_group_2021} is another approach that identifies corrupt samples in a dataset by recursively partitioning the dataset and testing each partition---e.g., by training a model on the partition and checking if this model mispredicts the query in question. Unfortunately, this line of work often idealizes this testing model for mathematical convenience, \eg assuming that one corrupt sample is sufficient to corrupt the entire model, or relaxing slightly by assuming a noise model, which is not true or hard to verify in many practical settings. Nevertheless, the idea of training separate models is promising because it allows us to evaluate the end-to-end effect of different subsets of the data on a model's prediction, regardless of the type of model or learning algorithm used.

A recent line of work uses a metric from game theory called the Shapley value (SV)~\cite{shapley} to find proponents. SV measures the marginal contribution of a datapoint, when combined with every possible subset of the remaining training data, on the resulting model's prediction.
%and averages these contributions while giving equal weight to each subset size. 
This metric is a good fit for our scenario because it considers variable-sized subsets of the training data without presuming a target threshold of proponents. 
%For example, it would detect that a corrupt image, when added to a subset of data containing enough other corrupt images, causes the model to make a misprediction, but does not do so when there are too few other corrupt images. 
Unfortunately, SV is extremely costly to measure because it requires training and evaluating a model for each of the $2^n$ possible subsets, where $n$ is the number of training datapoints. As a result, existing solutions either make strong assumptions about the learning algorithm, or at best reduce the number of models to linear in $n$~\cite{jia_towards_2020,ghorbani_data_nodate}.
%~\cite{d} works around this by making strong assumptions about the model, e.g., that it can be incrementally trained with certain "stability" properties, requiring $O(N\log\log N)$ models to be trained in order to approximate the SV, where $N$ is the number of datapoints. \notejinkun{With the ``stability'' assumption, the complexity will be lower. The $O(N\log\log N)$ is only making the monotonicity assumption. I think we can just say they are either slow, or making strong assumptions.}

None of the existing approaches can properly handle data sources. They either target individual datapoints or naively treat each source as a datapoint. This fails to capture the hierarchical nature of data sources, where we would like to find proponents at different levels of data source aggregation.
%, ideally from coarsely aggregated sources up to individual datapoints.

\mypara{Our approach}
We devise a principled methodology for finding proponents, called \somename{}, that (1) handles data source hierarchies, (2) considers variable-sized combinations of proponents, and (3) works for any learning algorithm. 

We first propose a metric for data sources called \quantityName{} (\quantity{}), that is similar to SV but draws its roots from the causal inference literature. Like SV, \quantity{} estimates the marginal effect of a data source over different subsets of the training data; but instead of enumerating all subsets, we use a randomized sampling procedure that explores different subset sizes and exploits the overlap between subsets. We extend this procedure to support  hierarchical sources by first sampling sources and then, conditioned on a source being included, sampling lower level sources from within the source. In addition to the {\em main model} trained on the full dataset, we train a {\em subset model} on each sampled subset.

%Although \quantity{} does not achieve all the properties of SV, it is sufficient for the explainability scenarios we target. More importantly, our randomized sampling procedure allows us to train only $O(k\log N)$ models, where $k$ is the number of datapoints \notejinkun{Should we say source?} that contribute to a model explanation. 

Given a query input and the main model's prediction on it, we feed the same query input to each subset model to obtain their predictions. We then use these results to formulate a new learning problem, where the features are the composition of each subset model's data subset, and the label indicates the subset model's prediction for the query label. Each entry of this design matrix effectively acts as a randomized treatment over the different data sources, and each label acts as the outcome of the treatment.
Assuming the proponents of a prediction are sparse, \ie of size $k \ll n$ (a standard assumption in the literature),
%---e.g., the fraction of data that is corrupt or mislabeled is often small relative to the full training set (this is one reason why it may have gone unnoticed)---
we can apply LASSO regression to the problem to select the sources that are most likely to be proponents. We show that this approach requires only $O(k\log n)$ subsets to be sampled (and hence models to be trained).
To give us control over the precision and recall of these proponents, we apply a technique called {\em knockoffs}~\cite{candes_panning_2017} to the LASSO regression.  Figure~\ref{fig:workflow} summarizes the overall workflow of \somename{}.

%Our methodology continuously trains the $O(k\log N)$ {\em subset models} on their corresponding subsets of the data, in addition to the {\em main model} that is trained on all of the data. 

%The above methodology achieves the goals we outlined earlier of (1) finding a sparse set of proponents that combine in variable ways to cause a model prediction; (2) controlling the rate of false reports; and (3) working across model types and learning algorithms. 
%\sid{Talk about sources here? Intro is getting long. Either we shorten the above significantly or include some slash-paragraph structure (or both). Also, I think we might want to define sources earlier, as if we only mention it at the end, people will expect our methodology to work very well on individual datapoints in all applications. If we want to pitch sources as both a challenge and an optimization, I think we need to mention it earlier.} \notejinkun{I think we should mention source earlier.}


%Achieving strict equalities of probabilities in Eq. 2 makes the AME coincide with Shapley value (SV) [31], which is costly to measure. Instead, we approximate it through a proxy of P. Doing so allows further efficient estimation through regression and LASSO. problem, where each datapoint is a model, the features are which datapoints contribute to it, and the label is how much it contribute to the model's prediction....

%in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are \emph{sparse}. Indeed, it is reasonable to assume sparse contribution. For instance, in the case of data poisoning detection, the attacker is typically only able to poison a limited number of sources given their limited resources at hand. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried.

%- We recognize SV as the right quantity, but overkill in some respects. The idea of training different models is appealing, it is an end-to-end method that is agnostic to the type of model. In a sense, if you could train a model on every subset of the datapoints.... To make this efficient, we draw 

%Although subsequent work~\cite{koh_accuracy_2019}  has shown that influence functions can estimate the effect of a larger group of datapoints, prediction explanations are not restricted to a specific group (e.g., any 10 of the 100 mislabeled datapoints could cause the misprediction). Moreover, this work assumes convex loss functions and hence does not apply to the kinds of non-linear models we most seek explanations for, e.g., DNNs~\cite{basu_influence_2020}.

%Group testing~\cite{} can be used to identify one or more poisoned samples in a dataset, under the assumption that any individual sample is sufficient to poison the entire model. But as we explained above, most practical explanations arise from the combined effect of multiple datapoints, where any individual datapoint is an insufficient explanation on its own.

%A more relevant line of work considers the effect of datapoints relative to subsets of the data, e.g., by considering whether they are included in random minibatches of data used to train the model during stochastic gradient descent (SGD), and how the prediction changes before/after training on the batch. However, this work only evaluates the effect of datapoints in subsets of a fixed size, whereas we are interested in variable-sized groups of data. Further, this approach assumes the loss change is only caused by the datapoints involved in the current batch, but modern DNNs are typically trained using techniques that draw influence from previous batches. 

%Another line of work~\cite{} proposes estimating the Shapley value (SV), which considers the marginal effect of a datapoint on all subsets of the data. This quantity makes sense, because it captures the effect of a corrupted datapoint on different subsetes of trainign data, including ones in which the datapoint's marginal effect causes the model to be make its misprediction. In contrast, if we only consider the datapoints marginal effect on the whole model (e.g., influence functions), or on too small a subset, we either measure no effect or have too noisy an estimate. While this gets at the quantity we would ideally like to estimate, it is too costly in practice to measure because it requires estimation of the effect of all possible subsets, which naively would require training that many models. In practice ~\cite{} achieves this by making strong assumptiosn about the model, e.g., assuming it can be incrementally trained and that all subsets experienced during incremental training provide enough signal for estimating the datapoint's effect (replace with "stability"), and they also target objectives like "group fairness" that are unnecessary in our setting. Even with these assumptions, the number of models that need to be trained is linear.


%In practice, data poisoning requires {\em collusion} among multiple datapoints to successfully poison a model, and the members of the colluding group need not be a specific group (e.g., multiple subsets of datapoints could be sufficient). In some sense, the relative size of the group may matter more. 


%For example, influence functions~\cite{} can be used to estimate the effect of small changes to a model (e.g., an individual datapoint), and under certain conditions often met by real-world datasets, can be used to estimate the effect of a large group of datapoints~\cite{}. Group testing~\cite{} can be used to identify one or more poisoned samples in a dataset, under the assumption that any individual sample is sufficient to poison the model.

%The problem with these approaches is that they do not reflect the reality of how data influences a model's decisions. Consider the case of poisoning attacks. In practice, data poisoning requires {\em collusion} among multiple datapoints to successfully poison a model, and the members of the colluding group need not be a specific group (e.g., multiple subsets of datapoints could be sufficient). In some sense, the relative size of the group may matter more. 



%Whereas traditionally people often ask these questions of individual data points, data is often naturally organized into sources in real world (e.g., customer data in a multi-tenant setting~\fixme{fix citation}\cite{}, data formed  by combining multiple competing sources~\cite{Zheng2019HelenMS}, data from crawling multiple web pages~\cite{Shafahi2018PoisonFT}). These sources are treated as units of trust, and the questions above can be applied to sources (e.g., has a source been corrupted by a malicious attacker). \fixme{todo: Give example from Microsoft oil customer (make this example similar to running example we use later on).} 

%Moreover, one advantage of this source view is that you have multiple examples from the same source and hence get more signal about that source, increasing the power of our explanations. \notejinkun{Is the last sentence saying that source view makes the problem easier (then why do we specifically bring up an easier version of a traditional problem)? Or is it saying doing so has more practical significance?} \notejinkun{I feel like we need to state this new view is challenge, as following: However, previous techniques cannot always easily generalize to sources. For instance, influence functions \cite{koh_understanding_2017} use first-order approximation that requires the data to remove is small, which does not apply to large sources. Its followup work \cite{koh_accuracy_2019} though generalizes it to source view and gives a first step analysis, it is not yet clear if influence functions are still accurate. Moreover, influence is fragile for DNNs \cite{basu_influence_2020}. (ii) \cite{pruthi_estimating_2020} attributes the loss delta after every training iteration to the data points inside that batch, but it is unclear how to generalize to sources. (iii) \cite{chen2018detecting} is based on examining the second-to-last layer's activation of every data point, but it is unclear how to extract similar activation for a whole source. On the other hand, trivially ignoring the sources and identifying the data points first and then selecting sources may fail because individual data point could be hard to detect.)}%the prediction may be caused by multiple data points each of which has too little influence to detect. Luckily, the data contributed tends to concentrate in a few sources, and examining the whole would aggregate enough influence to detect. Unfortunately, previous techniques cannot always generalize easily, \eg (i) influence function \cite{koh_understanding_2017} was traditionally for individual data point, and careful reasoning is needed as in \cite{koh_accuracy_2019} to generalize to the source view. However, influence is fragile for DNNs \cite{basu_influence_2020}. (ii) \cite{pruthi_estimating_2020} attributes the loss delta after every iteration to the data points inside that batch, but it . (iii) \cite{chen2018detecting} is based on examining the second-to-last layer's activation of every data point, but it is unclear how to extract similar activation for a whole source.} 
%\noteanqi{Maybe we should find another benefit of source senario, but I don't think it's good to compare with other approaches at this very beginning position.} 
%Finally, our source view also covers the previous invidiual point view, if one treats every individual data point as a source.

%Our problem is defined as to find out the sources that support a particular model prediction, given the dataset, training algorithm, query input and the prediction label (called query label from now on). \sout{We want to be able to identify the input sources that contribute to a particular model decision.} This question has been asked in different fields and different contexts through the ages, and most of the techniques developed work pretty well when the explanations are \emph{sparse}. Indeed, it is reasonable to assume sparse contribution. For instance, in the case of data poisoning detection, the attacker is typically only able to poison a limited number of sources given their limited resources at hand. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \notejinkun{I remember the previous sentence does not make sense for Sid. Maybe need to rewrite or remove.} Therefore, we make a \textit{sparsity assumption} that the prediction is mainly affected by a small group of data sources. Note that these sources may either support or oppose the prediction.\notejinkun{I remember there was a compliant about why it couldn't be neutral. But here I mean only in the group mainly affecting the prediction, and neutrals should not have main influence, so it couldn't be neutral.} Denote by $k$ the number of sources in this group, and the assumption can be written as $k\ll n$. We also make a \emph{monotonicity assumption} that in a high level says adding a corrupted source makes the prediction more or at least equally corrupted (see \ref{subsec:pro-state} for detail).

%\notejinkun{Would replace with the next paragraph} A strawman approach is to do a leave-one-out (LOO) test. Suppose that one data source is corrupted, then training $n$ different models omiting one source at a time will reveal the corrupt source. A better approach is to use group testing, which allows you to reduce number of models to $O(\log n)$ using a deterministic tree. But what if the number of sources contributing to the decision is $>1$ \notejinkun{I believe group testing can handle this as well}. Turns out we can still handle this with the group testing approach using the power of randomization. \notejinkun{My concern is that our approach smells very differently from those of group testing (which is very theoretical and formal as those of ML theories), and it might be weird to say we are group testing?} \sout{We use the above strawman to motivate Average Marginal Effect (\quantity{}) as a reasonable quantity for us to measure, which is an average LOO effect.} To do so, we propose Average Marginal Effect (\quantity{}) that characterizes the inclination of a source to the prediction, where a large positive number indicates supportive-ness and negative indicates opposed-ness \notejinkun{what are the appropriate words here?}, and then use randomization to achieve efficient estimation. We detail the definition in \S\ref{subsec:ame-mov}. \sout{We would like to develop an approach that measures \quantity{} for each source.} 

%\notejinkun{I would write the previous paragraph this way:} A strawman approach is to do a leave-one-out (LOO) test. Suppose that one data source is corrupted and caused a corrupted prediction being queried, then training $n$ different models omiting one source at a time will reveal the corrupt source. But when there are multiple corrupted sources, omiting one out may not be enough -- but only omiting multiple -- to be able to change the model, due to the non-linearity and complication of training algorithms and ML models (\eg the 1-Nearest-Neighbor models; see \S\ref{subsec:ame-mov} for detail). In other words, a zero LOO effect would be observed for every corrupted source. \notejinkun{should we mention the other strawman approach that trains on every source individually?}
%Luckily, we observe that when omiting from a subset instead of the full dataset, the LOO effect is more likely to be non-zero. More importantly, it is consistently one-sided and rarely flips, \ie omiting a corrupted source almost always makes the model less or equally corrupted. This motivates us to compute the average LOO effects on multiple subsets. \fixme{how to frame AME:} \textcolor{red}{\huge It turns out that this average effect has a close connection to the causal inference literature, and if formulated properly, our quantity fits into the definition of \emph{Average Marginal Effect (\quantity{})} proposed by \cite{egami_causal_2019}. To be consistent, we reuse the same name.} The corrupted sources would thus manifest positive LOO effect in some subsets and finally have highly positive average effect. Of course, this requires the observation to hold, which is the \emph{monotonicity assumption} we make.\fixme{TODO: add experiments to support the assumption} We detail the assumption in \S\ref{subsec:pro-state} and the definition of \quantity{} in \S\ref{subsec:ame}.
%that says omiting a supportive/opposed source from a subset almost always makes the model more likely/unlikely or at least equally likely to predict the query label. Put another way, the LOO effects of a source on all subsets are consistently one-sided and rarely flip. Under such an assumption, this average LOO effects, termed \emph{Average Marginal Effect (\quantity{})}, is able to characterize the inclination of a source to the prediction, where a large positive number indicates supportive-ness and negative indicates opposed-ness \notejinkun{what are the correct words here?}. We detail the definition in \S\ref{subsec:ame}.

%To estimate \quantity{} and use it to select sources, \sout{we first need to design a rule for choosing subset population for \quantity{} and should guarantee that it works for most incoming queries. An important constraint here is that the population need to be decided before the queries incoming, because we want to finish the expensive sampling offline and reuse for every future query, instead of sampling every time for a new query.} \notejinkun{To Anqi: The previous text is the design goal of AME and probably should be placed in later section that describe AME. (Previously I stated it as a challenge so it appears here, but now I think we don't need it.)} \noteanqi{Emm..I thought there is missing something between "we define AME" and "challenges to estimate AME", so here I put what's the AME for and the constraint. But if you think nothing missing, then it's ok with me.} \sout{Moreover, we want to estimate \quantity{} for each source, thus each of the sources requires training many models.} \notejinkun{Maybe merged into the subsequent challenge (1)?} there are three main challenges: (1) It should be \emph{computationally efficient}, in terms of both resources and time. The expensive model training required by measuring LOO effect adds to the challenge. (2) The selection should have a \emph{controllable false discovery rate (FDR)}, \notejinkun{technically should be called false discovery rate. They seem to be different concept.} (3) The approach should be \emph{general across different kinds of models and datasets}, especially deep learning ones, for which the question of explainability is most prominent. Prior approaches somehow don't meet all of the challenges we care about. For instance, approaches \cite{jia_towards_2020,ghorbani_data_nodate} that quantify using Shapley value (SV) are either too costly or making strong assumptions about the models, while classic LOO test and its fast approximation technique known as influence functions \cite{koh_understanding_2017, koh_accuracy_2019} are \sout{robust} not robust \sid{Do we mean "not robust"?} to non-linear models. \noteanqi{Is the summary here appropriate? Maybe we don't beat group testing here.} Refer to \S\ref{subsec:rel-work} the related work for more discussion on this.


%There are four phases, with the first two being offline and last two being online: (i) \emph{sampling:} Sample subsets according to a carefully chosen distribution; (ii) \emph{training:} Train one model per subset offline, which will later be reused across different queries; (iii) \emph{estimation:} When serving a new query, perform inference on each model for the query input, retrieve confidence of query label as signal, then employ LASSO to estimate the \quantity{}s; (iv) \emph{selection:} Based on the estimates, use a technique called Knockoffs \cite{candes_panning_2017} for selecting sources to control the FDR. The overall workflow is shown in Fig. \ref{fig:workflow}. 

%For the sampling phase, we use a default distribution that seek to sample roughly the same number of subsets for each size.\footnote{Note that we differ with Shapley value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately. However, this approximation enables the use of LASSO \notejinkun{todo: double check}. Second, our framework accepts customized population. It is useful when prior knowledge is available.} Moreover, we reuse subsets across sources to improve sample efficiency. 
%For the training phase, we provide an option to speed up by approximating training-from-scratch with warm-starting. %, which serves as our main technique for amortizing the training cost of all these models. 
%For the estimation phase, we encode each subset as the independent variable and its signal as the dependent variable, and formulate the estimation for $n$ sources together into a single regression problem where each source is estimated by one coefficient. We further utilize LASSO to achieve a scalable sample efficiency: if regularization parameter is chosen correctly, the number of samples and thus models to train for a good estimation is $O(k\log n)$, which scales as $n$ increases. % The coefficients for the sources estimate their \quantity{} consistently (modulo a constant factor), meaning that the coefficients converge asymptotically to the true values of their \quantity{}. 
%For the selection phase, the sources having an estimate larger than a threshold are selected, and the threshold is chosen by Knockoffs, which has the merit of controlling the expected FDR to be at most a given level. \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
% In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.



% \paragraph{Generalizing to Sources} We further generalize our problem statement to scenarios where the data come from different sources and we want to identify the group of sources that support/cause the prediction. This also has real applications. For example, in poison detection under multi-party training where multiple parties provide their own data to cooperate in training a model but some parties may be malicious and cause a mis-prediction of the model, one may want to ask which parties are responsible for this mis-prediction.
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/workflow.pdf}
    \caption{Workflow of \somename{}}
    \label{fig:workflow}
\end{figure}
%\paragraph{results} todo.

%\sid{Better names for tasks? Do we want to avoid "poison detection" altogether and replace it with "data debugging"? For model explanation we can say "data attribution".}\notejinkun{"data debugging" seems to include both detecting poison as well as corrupted data? And the latter sounds overlapped with data explanation (btw I thought ML people usually call it model explanation?) I still think poison detection + model explanation is the way to go.}
We evaluate \somename{}'s effectiveness on both data poisoning attacks as well as standard model explanation tasks. 
%two different tasks: data poisoning, where the goal is to find corrupted data that led to an erroneous prediction, and model explanation, where the goal is to simply find the training data that led to a prediction. 
We consider several different scenarios and datasets, including datasets where each source is an individual datapoint and where the data are naturally grouped into sources. \somename{} achieves precision above $97\%$ with recall between $65\%$ and $97\%$ on various datasets. 
We also apply \somename{} to a hierarchical setting where the proponents may be sources or individual datapoints, and show that \somename{} achieves a $3.9\times$ reduction in the number of models to train to detect proponents at the finer granularity. The top level of the hierarchy yielding perfect precision and recall with $15\times$ fewer models.

In summary, we make the following contributions: 
\begin{itemize}
\item We formulate a practical version of the data attribution problem for data partitioned into sources, and derive a metric for estimating the effect of each source on predictions (\S\ref{sec:motivation}).
\item We develop a principled methodology called \somename{} for estimating this metric accurately and efficiently (\S\ref{sec:methodology}). \somename{} formulates a novel regression problem whose solution reveals the proponents of a model prediction. %Our fine-tuning optimization reduces the cost of training models under this methodology.
\item We extend \somename{} to hierarchical settings where the proponents may be sources or individual datapoints (\S\ref{sec:hier}).  
\item We demonstrate \somename{}'s effectiveness in finding poisoned data sources and explaining model predictions (\S\ref{sec:eval}).
\end{itemize}

%We define our problem and state our assumptions in \S\ref{subsec:pro-state}. \S\ref{subsec:ame} motivates and derives the quantity we seek to measure, \quantity{}. \S\ref{sec: procedure} describes our methodology, which performs the sampling and training phases offline and the estimation and selection phases online. We extend our methodology to the hierarchical setting in \S\ref{sec:hier}, allowing us to find proponents both at the source level and the individual datapoint level. \S\ref{subsec:evaluation} presents our evaluation on several poison detection and model explanation tasks. 

% JY: this is awkwardly dangling at the end of intro
%We discuss related work in \S\ref{sec:rel-work} before concluding.

==> rm/intro.tex <==
\section{ Introduction }
\notejinkun{I feel like pitching our paper as measuring individual contribution is not as good as pitching it as detecting the group, since it seems hard to justify why having a larger value of our quantity means it has a larger contribution?}
\sid{I think we have all the pieces we need for the introduction puzzle, we just need to reorder things. We should start with more overview statements about the kinds of questions people ask and the landscape of work in this area (e.g., some of the statements in "why sparsity is reasonable" are a better fit here.}
When using a black-box machine learning (ML) model like deep neural networks (DNN), one often asked question is why the model gives such a prediction on a query input. This paper focuses on classification models, and aims to explain the prediction from the perspective of the training data. We make a \textit{sparsity assumption} that the prediction is mainly affected by a small number of data points. We further assume that they can be further divided into three groups: the proponent group that supports the prediction, the opponent group that opposes the prediction and the neutral group that neither proposes or opposes. \sid{Why isn't it possible for a source to be neutral, i.e. neither a proponent nor an opponent?} \notejinkun{Sorry forgot to change the text here. Fixed now. (I wrote in \S2 but forgot to update here)} The problem is defined as to identify the proponent group, given the dataset, query input and the prediction label (called query label from now on). Denote by $k$ the size of the proponent group, and $n$ the training set size.\notepanda{I agree with Jinkun's concern, I think we should lay it out as we are seeing use cases where data is collected from multiple sources, etc. and pose the question in term of sources.}\notejinkun{Ah I actually meant to say our quantity is only interpretable on its sign but not its magnitude. So we only want to formulate as detecting the group of sources instead of measuring/quantifying the contribution of every sources. Sorry for the ambiguity.}

\paragraph{Why the sparsity assumption is \sout{interesting} reasonable.}\notepanda{Interesting or reasonable? The paragraph seems to focus on reasonable?}\notejinkun{Yeah I meant reasonable (what's the difference between the two?)} Though assuming sparsity, the problem is still meaningful in reality. For example, today people are increasingly focused on the security of their ML models, and effort has been developed both on poisoning and its detection. One of the detection problem, called data poisoning detection, aims to identify the poisoned data points that fooled the model. This problem is essentially the same as ours, and the sparsity assumption also holds\notepanda{I don't follow the line of reasoning here, it holds because we assume it sounds less like it holds and more like we just assumed?}: the total number of poisoned data points is typically small given the limited resources of attackers. The other similar application is to explain unexpected predictions in which there are no attackers. The mis-predictions are likely caused by mis-labeled or ambiguous/misleading data, which should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \sid{I'm not sure what this last sentence is trying to say (we can omit it, since the point is well made that tail data in test sets are influenced by a very sparse number of input sources.}

\paragraph{Defining proponent/opponent group? \notejinkun{come from \url{https://arxiv.org/pdf/2002.08484.pdf}}}  \notejinkun{Should we give formal definition of these two groups? I feel like it's hard to define them clearly. Or maybe we should even remove this paragraph? If we want to keep it, I feel like this should not be in the introduction since intro should not give too much details (and that in later sections probably we have to repeat this paragraph)? But the argument for the \quantity{} needs this. So any suggestion?}\notepanda{I would argue for not defining it here, rather saying a perfect method is one that can detect any source that impacts the decision, this is hard to do in practice so we don't get there, and then use sensitivity as a figure of merit to evaluate?} \sid{Defining this precisely will be tricky, but it raises a good point: we know the source of poisoning because we poison the input data, but that in itself is not a general way of measuring the proponent-ness of a source. It could be that we don't detect a (poisoned) source because other artifacts in the data are sufficient to explain the decision. I think the large leave-out effect is a good starting point to build on.}
The exact definition is non-trivial (even controversial) and thus left for future work. Instead, we focus on some necessary properties of the group that we argue people generally would agree upon. We only consider proponent group here since the opponent group is similar. (1) \textbf{It must have a large leave-out effect}, i.e. removing this group decreases significantly the signal, where the signal can be defiend as the probability/confidence of predicting the query label or other quantity that captures such tendency \footnote{Classification DNNs typically have such quantities since the training is usually done by maximizing likelihood that by construction requires a measure of probability. When there is not, }. However, this alone is too imprecise since it does not rule out groups containing extra data points that have no effect, e.g. the full dataset as well has a large leave-out effect. This leads to the second property: (2) \textbf{The data point in the group should have non-zero individual effect.} More precisely, consider removing (without replacement) the data points of the group one by one at some order. We know that the outcome changes substantially when all of the group are removed, so there must be a time when removing one changes at least some. If a data point always has little effect upon removal in any ordering, it should not be in the group. \sid{I don't quite get this: why can't a source have one or more datapoints that don't affect the decision at all? It still could be a relevant source.}

% (3) The group should be as large as possible when the two previous conditions are verified, so that it is powerful enough to include every proponent data point.
% When using a black-box machine learning (ML) model like deep neural networks (DNN), one often asked question is why the model gives such a prediction on a query input. This paper focuses on classification models, and aims to explain the prediction from the perspective of the training data. The problem is defined as to identify the training data points that caused this prediction. More precisely, given a training set, a query input and its prediction label (call it \textit{query label} from now on), we want to find smallest groups such that removing the group changes the model outcome substantially into no longer predicting the query label with high probability/confidence\footnote{ML classifiers usually have such a quantity for each class.}, and any data point in any of such groups are said to cause the prediction. Denote by $k$ this group size. Similarly, we define groups and data points that prevent the prediction. Denote such group size by $k'$. Further denote the training set size by $n$. This paper limits the scope to the cases where the group size is small, i.e. $k \ll n$. We term the latter \textit{Sparsity Assumption}. Note that $k$ is not known in advance.

\notepanda{I am a bit concerned about why the preceding text leads to this discussion of AME? There seems to be a story or connection missing.}
\paragraph{Average Marginal Effect (\quantity{})}
Call $k_i, i=1,\dots,k$ a specific proponent in the proponent group. To find out the group, naively enumerating all possible groups is too expensive. The other more doable approach is doing the traditional leave-one-out (LOO) test for each data point $i$, where we calculate the change in signal between the $n$ data points and $n-1$ in which $i$ is left out, and select those having a large LOO effect. However, the group's leave-$k$-out effect is non-linear and in practice including $k-1$ proponents or $k$ gives the same (or close) signal, so the LOO test gives close-to-zero effect for every proponent and thus does not work either. For example, in a 1-Nearest-Neighbor algorithm, if there exist two identical data points, removing either one has no effect on later predictions. Similar phenomenon also occurs in deep learning. E.g. in CIFAR10, there are in total 50k examples in the training set, and removing anyone of them has only very little effect, which is likely obscured by the noise. Our experiments also partly verify this hypothesis (see Fig. \ref{fig:diff-tfs} and the evaluation for detail).

\notejinkun{I would use the next paragraph instead this one} We address this problem by calculating LOO effect on a population of subsets. Imagine a procedure where we keep removing all these $n$ data points one by one (without replacement) in some order \footnote{This shares the same idea as Shapley value (SV). See Eq. (1) and (2) of \cite{jia_towards_2020} for detail.}. We know the signal disappears when all $k_i$s are removed. By the second property there are orderings in which removing a $k_i$ dampens the signal. Notice that when this $k_i$ is removed, it is removed from a subset, so this dampening effect can be viewed as leave-$k_i$-out effect on some subsets defined by the orderings. For any orderings/subsets, leave-$k_i$-out likely either has zero or dampening, but not strengthening effect on the signal. Similar argument holds for the opponent group. Other data points likely has zero effect for any subset. We want to have a non-zero effect measured for each $k_i$, thus we want to create a population that include such subsets where leave-$k_i$-out has a large non-zero effect, so that when we average the LOO effect over the population of subsets, it is not 0 anymore. Call this average LOO effect \textit{Average Marginal Effect (\quantity{})}. We measure it for each data point and select those having a large value.

\notejinkun{After the discussion on Feb 1, I feel like this may be a better version of the paragraph above}We address this problem by calculating LOO effect on a population of subsets. For any $k_i$, by the second property there is a subset of the proponent group such that removing $k_i$ has a dampening effect. Notice that this is exactly doing LOO test since we are removing one point, but it is different than usual LOO test in that instead of the whole dataset, the removal is on a dataset that includes the group subset and all the other non-proponent data. We want to have non-zero effect measured for each $k_i$, thus we want to create a population of such datasets. However, the group is unknown, so we have to subsample the whole dataset, and that has a side effect that the non-proponent data are also subsampled. We make an assumption that they are sufficiently large enough that doing a (not-too-aggresive) subsampling does not very much affect their distribution, so that removing $k_i$ still has same effect as when the non-proponents are not subsampled. It follows that removing $k_i$ unlikely strengthens the signal in any case. Therefore, the LOO effects in the population are either dampening or zero, and when we average them, it is not 0 anymore, but a dampening effect. Call this average LOO effect \textit{Average Marginal Effect (\quantity{})}. For opponents, the \quantity{} should likely be the opposite, and for other data points, the \quantity{} should likely be zero.

\paragraph{Challenges}\notepanda{I would propose using a much shorter thing just providing a high-level approach (say how would you do this, one obvious answer is LOO but as we discuss in \S\ref{} that is not enough. So our approach is to train models over subsets and use information from that. But to do this need to address two challenges\ldots).}
First the best population is unknown, and different applications/datasets/algorithms/queries may have different best populations. It is challenging to propose a one-size-fits-all population. %The subset sampling distribution should ensure good coverage: An effective subset should let the contributive sources manifest the most of their effects, i.e. having high LOO delta, but different learning tasks / poisoning attacks may exhibit very different characteristics of such subsets. One distribution of subsets that works for one type of task may totally fail for the other.
%, but too small a subset dataset could deviate too far away from the full dataset, making the relative effect on the subset deviate as well from the that on the full dataset. E.g., consider a subset containing no datasets, then the model will only be trained on 1 or 0 data point, which will always produce the label in the former case and random in the latter case. In this case, the quantity degrades to only looking at the labels--it would assign equal contribution to every point sharing the same label as the query prediction. On the other hand, too large a subset dataset may as well unable to capture the contribution, as discussed above. 
Second, it is costly: There could be more than thousands of data points, each in the straightforward implementation requiring many draws of subset, each of which requires model training. Although techniques like influence functions \cite{koh_understanding_2017} can approximate outcomes without model training, it is not accurate for DNNs \cite{basu_influence_2020}. \sid{We might want to qualify or soften the preceding sentence, perhaps pointing out that it is fragile rather than "not accurate".}

\paragraph{Approach} \sid{Just a note that we should make it crystal clear that we are training multiple models, and compare that to prior approaches.} To address the first challenge, we use a default population that covers roughly uniformly for different sizes of subsets when prior knowledge is not available. In other words, there would be roughly the same number of subsets sampled for each size.\footnote{Note that we differ with Shapley value (SV) in that they achieve exactly same probability for each size, while our default option only do it approximately, and this approximation allows further optimization. Second, our framework accepts customized population. It is useful when prior knowledge is available.}
To address the second challenge, we utilize the sparsity assumption and borrow techniques from the literature of causal inference. Instead of sampling subsets and computing separately for each source, we reuse subsets and use regression to measure for all sources simultaneously, where each source has one covariate indicating its inclusion/exclusion in the subset and the signal of the model trained on the subset is used as the response variable. The coefficients for the sources estimate their \quantity{} consistently, meaning that the coefficients converge asymptotically to the true values of their \quantity{}. The coefficients larger than a threshold are selected, and the threshold is chosen by a technique called \textit{Knockoffs}, which has the merits of controlling the expected precision to be at least a given value. \sid{We should take care in introducing this because it is one of our main contributions. I would frame it as formulating a new regression problem whose optimization gives us the contributions of the sources (and make it clear that the formulation of this design matrix is a contribution).}
In addition, L1 regularization (LASSO) is employed in regression such that only $O(k\log n)$ \notejinkun{Actually the opponent group size should also be counted in the $k$ of this formula. So should we make it explicit here?} samples are required to achieve a good estimation.
Next, the subsets and sub-models are reused across different queries -- only the response variables are needed to be re-computed, which only requires inference. Finally, we speed up the training by approximating training-from-scratch with warm-starting. \sid{Though we aren't really innovating here, we should highlight this as our main technique for amortizing the training cost of all these models.}

\paragraph{Generalizing to Sources} We further generalize our problem statement to scenarios where the data come from different sources and we want to identify the group of sources that support/cause the prediction. This also has real applications. For example, in poison detection under multi-party training where multiple parties provide their own data to cooperate in training a model but some parties may be malicious and cause a mis-prediction of the model, one may want to ask which parties are responsible for this mis-prediction.

\paragraph{results} todo.

\paragraph{Contribution}
\begin{outline}
\1 We propose \quantity{} whose sign indicates whether a data point/source supports or opposes the prediction.
\1 We propose a default option as the population, but also allows customized ones.
\1 We employ LASSO to estimate this quantity, and show that only $O(k\log n)$ \notejinkun{again $k$ should include the other group} samples are required to achieve a good estimation.
\1 We use Knockoffs to control the selection precision.
\1 We optimize the model training using warm-starting.
\end{outline}


==> rm/motivation-v2.tex <==
\section{Motivation, Problem Statement and Assumptions}
\label{sec:motivation}
At an abstract level, our objective is to understand the impact of training examples in an ML datasets on specific final predictions from the trained model. Given a specific prediction made by a model, we seek to understand which training examples, through the learning algorithm, are most responsible for this prediction.

More concretely, consider the following example. Based on images collected online, Alice trains a classification model to automatically label different objects that appear on images. 
%
\notejinkun{this sentence seems broken, not sure who's working on it?}
collects data from multiple websites to train an image classification model that recognizes what is on the image. Fig. \ref{fig:running-ex} shows examples of 3 sources/websites. However, some collected images from a website that is run by a careless administrator who accidentally uploads arbitrary images embedded with some watermark. \notejinkun{Is this framing matching what you had in mind @Sid?} \sout{are uploaded by a malicious attacker such that they are just some arbitrary image embedded with a special watermark.} Alice unfortunately did not check the data and hence was not aware of this \sout{attack} corruption, so the model is trained on these \sout{poisoned} corrupted images, and unexpectedly learns the mapping between watermark and some label. Only after Alice deployed it, seeing it always giving \sout{poison} cat label whenever there is a watermark in the picture, has she realized that the data could be problematic. Now Alice would like to find out which data source is causing this behavior, so she logged down a mis-predicted picture with such a watermark for further analysis.\jinyang{We should point out that the use of watermark is just for illustrative purposes; many poisoned data do not have visual cues.}\notejinkun{if we switch to corrupt data, it seems fine to have visible watermark}
%
We will use this scenario as a running example in the rest of the paper to make the discussion more concrete. \sout{The evaluation (\S\ref{subsec:other-apply}) also shows how our technique can be used to study and explain non-adversarial mis-predictions.}

Let $\mathcal{M}$ denote the trained model to analyze, e.g. Alice’s image classifier. $\mathcal{M}$ \notejinkun{check if need to term it ''main model''} maps each example from the input space $\mathcal X$ to a normalized score between 0 and 1 for each possible class $\mathcal Y$, aka $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$. As each example's normalized scores across all classes sum up to one, they are often interpreted as a probability distribution over classes conditioned on the input, or a confidence score for each class.

% Query input/label, and question about finding the proponents

\notejinkun{insertion begin}
Let $I$ denote the model input at the inference time, \eg Alice's dog image, and $L$ the predicted label, \eg Alice's cat label. We term $I$ and $L$ \emph{query input} and \emph{query label}, respectively.
       
\paragraph{Problem Statement} We term a source supporting the prediction \emph{proponent} (\eg Alice's cat source), source opposing \emph{opponent} (\eg Alice's dog source), and the rest \emph{neutral} (\eg Alice’s horse source). We define the \emph{auditing problem} as one where we identify the set of all the proponents. We call it \emph{proponent group}. 
Note that the problem formulation also includes invidual datapoint view. In such a case each datapoint is a source, and the problem becomes the classic one of identifying the training examples that support/oppose the prediction.


% \sid{Let's blend this section with the previous motivation section. At the end of this section, the problem formulation should be clear and it should be clear why a quantity like AME is what we need.}
% \notepanda{I think we need to help the reader a bit before we step to this paragraph.}

% \notepanda{I think we should consider adding a running example starting here, it might help make the technical bits a little clearer and help with connecting some of this to how we will eventually use things.}

\paragraph{Assumptions}
We make a \textit{sparsity assumptions}: only a sparse set of sources are proponents or opponents. We denote by $k$ the number of sources in this sparse set, and the assumption can be written as $k \ll n$. 

\sid{See below for some more detail about the sparsity assumption that I removed from the intro; we may want to include some of those points here.}
\ignore{
Indeed, it is reasonable to assume sparse contribution. For instance, in the case of data poisoning detection, the attacker is typically only able to poison a limited number of sources given their limited resources at hand. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \notejinkun{I remember the previous sentence does not make sense for Sid. Maybe need to rewrite or remove.}
}

We also make a \emph{monotonicity assumption}. To make the discussion clear, we first define a quantity $U(S)$ to measure how supportive a source $S$ is to the prediction. To do so, we first train a model $\mathcal M_S$ on $S$, and use its inference confidence on query input as the measure. Formally, $U(S)=\mathcal M_S(I)[L]$. We also call it \emph{signal} \notejinkun{Are we still using the term signal @Mathias?} of $S$ or signal of $\mathcal M_S$. 
Now the monotonicity assumption can be stated as follows: given any proponent/opponent $i$, its marginal effect on $S$, \ie $U(S+\{i\})-U(S)$, is non-negative/non-positive for every $S\subseteq [n]-i$, where $[n]=\{1,2,\dots,n\}$; Moreover, There exists at least one subset on which the marginal effect is non-zero (otherwise this source should be considered as neutral). Intuitively, in the application of corrupted data detection, the assumption roughly translates to that adding a corrupted source makes the prediction more corrupted or equally corrupted. Though the assumption is strong as it requires to hold on every subset, it is stronger than necessary for our quantity (discussed in \S\ref{subsec:ame}) to work. At a high level, as long as the overall \emph{average} effect on multiple subsets has the right sign, our quantity should work.


\notejinkun{insertion end}

\notejinkun{Should we remove the following text? Doesn't seem to continue the story}


%
Two main theoretically grounded approaches have been proposed to tackle this task of finding training data most responsible for a given problematic prediction.

\paragraph{Influence function:}

\paragraph{Shapley value:}

\paragraph{Goals:} in this paper, we seek to bridge the gap between these approaches by proposing a theoretically grounded approach to the detection problem that:
- enables finding inputs that cause outputs in groups
- is computationally tractable compared to Shapley value, with convergence guarantees
- is practical, with false positive rate control

In the reminder of this paper, we introduce out approach and its theoretical analysis, including assumptions and threat model (\S\ref{}), present a practical instantiation with efficiency improvements (\S\ref{}), discuss extensions to hierarchical designs to handle scenario 2’s sources (\S\ref{}), and perform an empirical evaluation of different tasks and datasets (\S\ref{}).

%\section{Approach}

%We start from the insight that we are looking for sources with a large, positive causal impact of the score predicted …
%=> factorial experiments
%=> what population do we need, so that we can handle groups and compute it efficiently?

==> rm/motivation-v3.tex <==
\section{Problem Formulation}
\label{sec:motivation}

At a high level, our goal is to understand the impact of training data on the predictions made by an ML classification model. Given a query input and associated query label to explain, we seek to identify the data sources which contribute most positively to predicting the query label. The practical scenario depicted in Figure~\ref{fig:running-ex} imposes certain requirements on our formulation. Using this scenario as a guide, we state our problem more formally (\S\ref{subsec:problem}), present our metric for quantifying the effect of a source (\S\ref{subsec:ame}), and state the assumptions and threat model we operate under (\S\ref{subsec:assumptions}).

\subsection{Problem statement}
\label{subsec:problem}

Let $\mathcal{M}$ denote the \emph{main model} we wish to analyze, \eg the image classifier in Figure~\ref{fig:running-ex}. $\mathcal{M}$
maps each example from the input space $\mathcal X$ to a normalized score in $[0,1]$ for each possible class $\mathcal Y$, \ie $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$. Since the normalized scores across all classes sum  to one, they are often interpreted as a probability distribution over classes conditioned on the input example, giving a confidence score for each class.
Let $Q_I$ denote the \emph{query input} given to the model for inference, and $Q_L$ the \emph{query label} to explain. In Figure~\ref{fig:running-ex} for example, the query input is the misclassified dog image at the bottom, and the query label is "cat". We seek to explain the confidence score given by the main model to the query label, when predicting on the query input, or formally $\mathcal{M}(Q_I)[Q_L]$.

We call a source that contributes positively to the confidence score a \emph{proponent} (\eg the cat subreddit), a source that contributes negatively an \emph{opponent} (\eg the dog subreddit), and the remaining sources \emph{neutral} (\eg the horse subreddit).
Note that sources may represent individual datapoints or collections of them, and may span different levels of a source hierarchy.
Our goal is to identify the set of proponents for the query label, or \emph{proponent group}. But how can we quantify a source's contribution to the query label?
%, especially when a given prediction can depend on multiple sources?

%How do we quantify a source's contribution to the query label?
The scenario in Figure~\ref{fig:running-ex} has several properties guiding our design of a suitable metric.
First, training data often come from naturally-occurring sources (\eg different subreddits or websites), which can vary in size and span different levels of a hierarchy, with finer granularity sources (individual images) grouped into larger ones (the websites). Our metric should support detecting sources of different sizes at different levels of the hierarchy.
Second, the models we seek explanations for may vary in complexity; \eg the image classifier in Figure~\ref{fig:running-ex} may be a complex DNN for which directly calculating the impact of a source is infeasible. Thus, our metric should treat the model and learning algorithm as a black box to generalize across scenarios.  
Finally, sources often have a combined effect on the query label that they would not have in isolation. In our example from Figure 1, any 10 or more of the corrupt images from the cat website are sufficient to cause the model to misclassify the dog image, but fewer than 10 images would have no adverse effect. 
Our metric should consider the effect of combinations of sources from the training data. Unfortunately, due to the second property above, we do not know what the effect of a given combination of sources will be until we train an end-to-end model on this data. 
%In this vein, approaches that rely on the Shapley value (SV) are a step in the right direction. We propose a similar metric below that has many of the properties of SV but lends itself to a more efficient estimation..

%\noindent{\bf Intuition.} To quantify ``provenance'', we need to measure, for each source, how much it contributes to a given prediction. One naive approach is the ``leave one out'' (LOO) test, which measures the change in the model's prediction when trained without the source of interest. As the influence function~\cite{koh_understanding_2017} also aims to quantify the effect of adding/removing a training datapoint, it can be viewed as a form of LOO test. %We term it \textit{LOO change} or \textit{influence} for short.% Finally select those greater than a threshold.
%However, under complex ML algorithms, LOO tests can fail because removing one source may not cause change in the model's output. For example, consider the case of 1-nearest-neighbor algorithm, if there are two identical nearest points of the query input residing in two separate sources $i$ and $j$, the model's output will not change unless both proponent sources are removed.% Similar phenomenon also occurs in deep learning. E.g. in CIFAR10, there are in total 50k examples in the training set, and removing one of them brings only very little impact, which is likely obscured by the noise. Our experiments also partly verify this hypothesis (see Fig. \ref{fig:diff-tfs} and the evaluation for detail).

%The failure of naive LOO stems from its inflexibility: when determining the contribution of source $i$, LOO measures the marginal effect of training with and without $i$ but always in the presence of {\em all} remaining sources. To address LOO's limitation while keeping its intuition, we allow more flexibility in the cohort of sources that $i$ is trained with or without when determining $i$'s contribution. For maximum flexibility, the cohorts can be sampled following some distribution from the $n$ original sources, with the effects averaged across sampled cohorts. For example, in our previous 1-nearest-neighbor example with two contributing sources $i$ and $j$, if $i$ is trained with and without a sampled subset of sources that does not contain $j$, then we will be able to observe non-zero marginal effects when comparing the resulting models.

%\subsection{Alice's Motivating Example}
%At an abstract level, our objective is to understand the impact of training examples in an ML datasets on specific final predictions from the trained model. Given a specific prediction made by a model, we seek to understand which training examples, through the learning algorithm, are most responsible for this prediction.

%More concretely, consider the following example. Based on images collected online, Alice trains a classification model to automatically label different objects that appear on images. The data are collected from multiple websites. Fig. \ref{fig:running-ex} shows examples of 3 sources/websites. However, one website is run by a careless administrator who accidentally uploads arbitrary images embedded with some watermark. \notejinkun{Is this framing matching what you had in mind @Sid?} \sout{are uploaded by a malicious attacker such that they are just some arbitrary image embedded with a special watermark.} Alice unfortunately did not check the data and hence was not aware of this \sout{attack} corruption, so the model is trained on these \sout{poisoned} corrupted images, and unexpectedly learns the mapping between watermark and some label. Only after Alice deployed it, seeing it always giving \sout{poison} cat label whenever there is a watermark in the picture, has she realized that the data could be problematic. Now Alice would like to find out which data source is causing this behavior, so she logged down a mis-predicted picture with such a watermark for further analysis.\jinyang{We should point out that the use of watermark is just for illustrative purposes; many poisoned data do not have visual cues.}\notejinkun{if we switch to corrupt data, it seems fine to have visible watermark}
%
%We will use this scenario as a running example in the rest of the paper to make the discussion more concrete. \sout{The evaluation (\S\ref{subsec:other-apply}) also shows how our technique can be used to study and explain non-adversarial mis-predictions.}

%Let $\mathcal{M}$ denote the trained model to analyze, e.g. Alice’s image classifier. $\mathcal{M}$ \notejinkun{check if need to term it ''main model''} maps each example from the input space $\mathcal X$ to a normalized score between 0 and 1 for each possible class $\mathcal Y$, aka $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$. As each example's normalized scores across all classes sum up to one, they are often interpreted as a probability distribution over classes conditioned on the input, or a confidence score for each class.

% Query input/label, and question about finding the proponents

% \notejinkun{insertion begin}
%Let $I$ denote the model input at the inference time, \eg Alice's dog image, and $L$ the predicted label, \eg Alice's cat label. We term $I$ and $L$ \emph{query input} and \emph{query label}, respectively.


%Let $\mathcal{M}$ denote the trained model to analyze, e.g. Alice’s image classifier. $\mathcal{M}$ \notejinkun{check if need to term it ''main model''} maps each example from the input space $\mathcal X$ to a normalized score between 0 and 1 for each possible class $\mathcal Y$, aka $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$. As each example's normalized scores across all classes sum up to one, they are often interpreted as a probability distribution over classes conditioned on the input, or a confidence score for each class.

%Let $I$ denote the model input at the inference time, \eg Alice's dog image, and $L$ the predicted label, \eg Alice's cat label. We term $I$ and $L$ \emph{query input} and \emph{query label}, respectively.
       
%We term a source supporting the prediction \emph{proponent} (\eg Alice's cat source), source opposing \emph{opponent} (\eg Alice's dog source), and the rest \emph{neutral} (\eg Alice’s horse source). We define the \emph{auditing problem} as one where we identify the set of all the proponents. We call it \emph{proponent group}. 
%Note that the problem formulation also includes individual datapoint view. In such a case each datapoint is a source, and the problem becomes the classic one of identifying the training examples that support/oppose the prediction.

% \sid{Let's blend this section with the previous motivation section. At the end of this section, the problem formulation should be clear and it should be clear why a quantity like AME is what we need.}
% \notepanda{I think we need to help the reader a bit before we step to this paragraph.}

% \notepanda{I think we should consider adding a running example starting here, it might help make the technical bits a little clearer and help with connecting some of this to how we will eventually use things.}
%\subsection{Prior Art}
%Two main theoretically grounded approaches have been proposed to tackle this task of finding training data most responsible for a given problematic prediction.

%\paragraph{Influence function:} 

%\paragraph{Shapley value:}

%\paragraph{Goals:} in this paper, we seek to bridge the gap between these approaches by proposing a theoretically grounded approach to the detection problem that:
%- enables finding inputs that cause outputs in groups
%- is computationally tractable compared to Shapley value, with convergence guarantees
%- is practical, with false positive rate control

% In the reminder of this paper, we introduce our approach and its theoretical analysis, including assumptions and threat model (\S\ref{}), present a practical instantiation with efficiency improvements (\S\ref{}), discuss extensions to hierarchical designs to handle scenario 2’s sources (\S\ref{}), and perform an empirical evaluation of different tasks and datasets (\S\ref{}).


% \section{Average Marginal Effect (\quantity{})}
% 
%Figure \ref{fig:workflow}

%\sid{This is indeed a bit bottom-up, but if our previous motivation/problem formulation section makes it clear why AME is the core metric we need, I think it could work. We should retitle this section to indicate this is how we measure the effect of proponents.}
%\notepanda{I am concerned that the paper might be very bottom up. I think as a reader I would be unhappy here, asking why do I need to learn about this quantity that so far has not been used in the paper. I think we want to go top-down, motivate why this quantity, how we use it, and then formally define it.}

%\sid{Include straw solutions here regarding what quantity to measure, such as LOO?}

%\subsection{Motivation}
%\label{subsec:ame-mov}
%\sid{I would call this "Intuition" and consider using a slash-paragraph instead}

%\noindent{\bf Intuition.} To quantify ``provenance'', we need to measure, for each source, how much it contributes to a given prediction. One naive approach is the ``leave one out'' (LOO) test, which measures the change in the model's prediction when trained without the source of interest. As the influence function~\cite{koh_understanding_2017} also aims to quantify the effect of adding/removing a training datapoint, it can be viewed as a form of LOO test. %We term it \textit{LOO change} or \textit{influence} for short.% Finally select those greater than a threshold.
%However, under complex ML algorithms, LOO tests can fail because removing one source may not cause change in the model's output. For example, consider the case of 1-nearest-neighbor algorithm, if there are two identical nearest points of the query input residing in two separate sources $i$ and $j$, the model's output will not change unless both proponent sources are removed.% Similar phenomenon also occurs in deep learning. E.g. in CIFAR10, there are in total 50k examples in the training set, and removing one of them brings only very little impact, which is likely obscured by the noise. Our experiments also partly verify this hypothesis (see Fig. \ref{fig:diff-tfs} and the evaluation for detail).

%The failure of naive LOO stems from its inflexibility: when determining the contribution of source $i$, LOO measures the marginal effect of training with and without $i$ but always in the presence of {\em all} remaining sources. To address LOO's limitation while keeping its intuition, we allow more flexibility in the cohort of sources that $i$ is trained with or without when determining $i$'s contribution. For maximum flexibility, the cohorts can be sampled following some distribution from the $n$ original sources, with the effects averaged across sampled cohorts. For example, in our previous 1-nearest-neighbor example with two contributing sources $i$ and $j$, if $i$ is trained with and without a sampled subset of sources that does not contain $j$, then we will be able to observe non-zero marginal effects when comparing the resulting models.

% \notejinkun{@Sid, this is what I think is missing in the later comments following ``Version 2'' in the ``Selecting Subset Sample Distribution'' slash-paragraph}
% \notejinkun{I think we either need this paragraph or the monotonicity assumption. If we chooses monotoncity, it could be more succinct but we may need experiments or additional text similar as this paragraph to support it.}
% For general ML algorithms other than 1NN, we know removing only one proponent (while keeping every other source) may not be able to change the model output, but removing the whole proponent group should change the output significantly. Thus if the proponents are removed one by one in some order, the model output will ultimately changes, so there must be a point in the middle when removing one proponent changes the output at least some. This is when LOO test gives a non-zero marginal effect, but different than usual LOO test, now it is removing from a subset where some other proponents have been removed. We want to have a non-zero effect measured for each proponent, thus we want to create a population that includes such subsets. Without knowing which sources are the proponents, we have to subsample the full dataset, except that the non-proponents are also subsampled. However by the sparsity assumption we can argue that there should be sufficient non-proponent data such that subsampling them does not have a large impact on the output.

\subsection{Average Marginal Effect (AME)}
\label{subsec:ame}

% \mypara{Definition}
The above properties suggest the need for a metric that evaluates the effect of a source on variable-sized subsets of the training data by training models end to end. Formally, we define the utility $U(S)$ of a data subset $S$ as $S$'s contribution to the query label $Q_L$. We measure $U(S)$ by training a model $\mathcal M_S$ on $S$. We refer to $M_S$ as a {\em subset model}, and use it to infer a label for the query input $Q_I$. We use the confidence score output by this inference process as $U(S)$, i.e., $U(S) \triangleq \mathcal M_S(Q_I)[Q_L]$. %, with the convention that $U(\emptyset)=0$.

The contribution of a source $i$ is the marginal increase in utility from adding the source to different subsets $S$. We refer to this as the source's \emph{Average Marginal Effect (\quantity{})}, defined as the expected marginal effect of $i$ on subsets drawn from a distribution $\mathcal{L}^i$:
\begin{equation}
\label{eq:ame}
AME_i(\mathcal L^i)=\mathbb E_{S^i\sim \mathcal L^i}[U(S^i+\{i\}) - U(S^i)]
\end{equation}
Here $S^i$ is a subset of sources that do not contain $i$ sampled from $\mathcal L^i$. The marginal effect of $i$ with respect to $S^i$ is calculated as the difference in the model's output when trained with and without $i$, \ie $U(S^i+\{i\})-U(S^i)$. 
%Note that for the definition to be meaningful, none of the subsets sampled from $\mathcal{L}^i$ should contain $i$.
%, i.e. $i\notin S^i, \forall S^i\sim \mathcal L^i$. 
%The sample distribution $\mathcal L^i$ should be considered as a hyper-parameter and we will discuss how it can be best chosen in \fixme{\ref{}}.

% We argue that a source having an $AME$ of a large positive value should be considered as a proponent source since adding it to those subsets increases the signal significantly on average. Likewise, a source having a large negative $AME$ is an opponent, and the rest are neutrals.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{fig/S-shape-poison.png}
    \caption{Utility vs the subset size, measured on CIFAR10-50 dataset (see \S\ref{sec:eval}), where each point denotes a subset. Each subset is obtained by first drawing an inclusion probability $p$ from a uniform distribution with range from 0.01 to 0.99 and then including each datapoint with probability $p$.}
    \label{fig:yvsp}
\end{figure}

%\noindent{\bf Selecting Subset Sample Distribution}
% \vspace{0.1in}
% \noindent{\bf Selecting subset sample distribution.} 

%\sid{Sid to trim and consolidate text below, which I think has sufficient content (we don't need further theoretical justification.}

Clearly, the choice of sampling distribution $\mathcal L^i$ affects what \quantity{} is measuring, and how efficiently \quantity{} can be estimated (\S\ref{sec:methodology}). When choosing $\mathcal L^i$ we need to ensure subsets of different sizes should be well represented.
To see why, consider our example from Figure~\ref{fig:running-ex}, treating each individual image as a source:
If a subset is large, it is likely to have 10 or more corrupt images, enough to make the subset model mispredict, and the marginal impact of one more corrupt image is close to zero.
Similarly, a small subset will have few corrupt images. 
% JK: commenting the original verision for switching back
The subset model may exhibit noisy behavior, but the marginal effect of one more poison will also be close to zero.
%Even if the subset models exhibit noisy behavior, the \emph{average} marginal effect of one more poison will also be close to zero.
Figure~\ref{fig:yvsp} shows this phenomenon from one of our poison detection experiments on the CIFAR10-50 dataset, in which subsets from either of the two "flat" regions show no marginal utility for proponents.
Since the region with non-zero effect for proponents is unknown in advance, we must sample subsets across subset sizes.

Interestingly, defining the \quantity{} under a uniform distribution over subset sizes ($\mathbb P[|S^i|=0]= \dots =\mathbb P[|S^i|=n-1]$) is equivalent to computing the Shapley value~\cite{jia_towards_2020,ghorbani_data_nodate}, which meets our requirement. However, uniformly sampling over subset sizes is often impractical. Therefore, we instead sample subsets by including each source (except for the source being measured) with a probability $p$ chosen uniformly from a set of values $\mathcal{P}$, thus ensuring coverage across subset sizes.
The subset distribution $\mathcal{L}^i_{\mathcal{P}}$ induced by $\mathcal P$ is:
\begin{equation}
\label{eq:amep}
AME_i(\mathcal L^i_{\mathcal{P}})=\mathbb E_{S^i\sim \mathcal L^i_{\mathcal{P}}}[U(S^i+\{i\}) - U(S^i)].
\end{equation}
In what follows, we use the shorthand $AME_i$ for $AME_i(\mathcal L^i_{\mathcal{P}})$.



\ignore{
When there is no prior knowledge on how proponent sources contribute to the prediction, it is best to sample uniformly across different subset sizes. In other words, there should roughly be the same number of subsets sampled for each size: 
%Formally, the population should satisfy the \textit{uniform coverage requirement}
\begin{equation}
\label{eq:eq}
    \mathbb P[|S^i|=0]= \dots =\mathbb P[|S^i|=n-1]. \nonumber
\end{equation}

\sid{Need to mention that we are looking within the cat website source and not treating a "source" as a website here... (a bit confusing)}
To see why this is the case, consider our example from Figure~\ref{fig:running-ex}. 
If a subset already has 10 or more corrupt images (indicating that it is large), then it is already sufficient to make the model mispredict with confidence close to 1, so adding further corrupt images to this set will not increase the confidence by much. Similarly, if the subset has very few  corrupt images (indicating it is small), then the model may exhibit noisy behavior and the signal will be closer to 0. Figure~\ref{fig:yvsp} shows this phenomenon from one of our poison detection experiments on the CIFAR10-50 dataset. If we sample subsets from either of the two "flat" regions, the \quantity{} measured for proponents (poisoned datapoints) will be close to zero since adding one more proponent does not substantially change the signal. Thus, to robustly measure a non-zero effect for proponents, we must sample subsets in between these two flat regions---but without prior knowledge of where the regions lie, we must assume they can appear anywhere, and hence sampling uniformly across subset sizes is ideal. \sid{Interestingly, defining the \quantity{} under this distribution coincides with the Shapley value used in prior work\cite{jia_towards_2020,ghorbani_data_nodate}.}

However, achieving strict equalities of probabilities in Eq. \ref{eq:eq} makes the AME coincide with Shapley value (SV) \cite{jia_towards_2020,ghorbani_data_nodate}, which is costly to measure. Therefore, we must approximate it to enable efficient estimation through regression and LASSO.
}

We refer to sources that have $\quantity{} > 0$ as proponents, source with $\quantity{} < 0$ as opponents, and all other sources as neutrals. In practice, neutrals are likely to have a small non-zero effect on the model prediction. We leverage a thresholding scheme based on statistical tests to account for this noise and control the precision of our identification (\S\ref{subsec:knockoffs}).

% Under the monoticity assumption, we can argue that the $AME$ is a non-zero \notejinkun{Should we say "positive" (since they are for proponent sources)?} value for any\jinyang{is it "any" or "some"?}\notejinkun{I think it's any if my English is correct. What I meant to convey is that every proponent will have a positive AME under the assumption.} proponent source.  To see this, consider removing all proponent sources one by one. We observe that the sum of the marginal effects calculated between successive removals is equal to the overall effect of all proponents, which is non-zero. Suppose the overall effect is positive \notejinkun{The effect should always be positive since it is confidence and within [0,1].}, there exists source $i$ and subset $S_i$ whose removal (from $S_i+{i}$ to $S_i$) results in a positive marginal effect, since the monoticity assumption guarantees that all successive removals have non-negative marginal effects. As long as subset $S_i$ can be sampled from distribution $L_i$, the resulting $AME_i$ will be positive.  Ditto if the overall effect is negative.
% For any neutral source, its effect on any subset is around zero and so is the corresponding $AME$. \notejinkun{@Jinyang Sorry I don't quite understand the previous paragraph. Maybe we should talk about this synchronously}

\subsection{Assumptions and Threat Model}
\label{subsec:assumptions}

Computing the \quantity{} is costly in general, because it requires training and evaluating a model for each subset that is sampled. In practice however, the proponents of a prediction tend to comprise a \emph{sparse} subset of the training data, and we exploit this observation for efficiency.
Therefore, for efficiency we assume that the number of sources $k$ that have non-zero \quantity{} is small compared to $n$, or $k \ll n$.
Concretely, this assumption can be verified when data is corrupted due to user error, which tends to affect only a small portion of the overall training set; or when the predictions under scrutiny arise from queries on the tails of the distribution, which are typically influenced by only a few examples in the training data~\cite{feldman2020neural,ghorbani_data_nodate}.

We also assume that neutral sources are \emph{independent} of the final utility of a subset, conditioned on the probability of source inclusion $p$ and other sources.
Formally, $U(S) \perp\!\!\!\perp \mathbf1_{i\in S} | \left((\mathbf 1_{j\in S})_{j\neq i},p\right)$, where $\mathbf1_{condition}$ is an indicator function that evaluates to 1 if $condition$ is true and 0 otherwise.
% We further assume that any neutral source $i$ is \emph{independent} of the final utility of a subset, conditioned on the other sources. In other words, $U(S)$ has same distribution as $U(S+\{i\})$, for any $S$ not including $i$.
This assumption states that whether or not a neutral source is included in $S$ has no more effect on the value of $U(S)$ than the effect from including any neutral source with probability $p$ in the baseline model.
Under this assumption, we can control the precision of our approach to separate neutral sources from proponents and opponents (\S\ref{subsec:knockoffs}).
% We assume independence so that we can control our approach's precision and separate neutrals from other sources.
% This assumption allows us to control the precision of our identification approach, separating neutrals from proponents and opponents.

% These assumptions are particularly relevant in an adversarial context, such as that of data poisoning.
% Our sparsity assumption implies that when data is deliberately altered, the attacker is only able to poison a small number of sources, perhaps due to limited resources they have at hand.
% Our independence assumption implies that an attacker cannot create strong dependencies between the utility and neutral sources based on altering a small number of sources.
In an adversarial context, such as data poisoning, the sparsity assumption merely implies that attackers control a small portion of sources and the independence assumption implies that adding or removing a neutral source does not significantly impact utility. Finally, for the adversarial setting we also assume that a poisoned source $i$ has $\textrm{AME}_i > 0$. That is, an attacker cannot craft a poisoned source 
such that $U(S^i+\{i\}) - U(S^i)$ is negative at some $p$ values and positive at other $p$ values, while still yielding a working poisoning attack on the main model $\mathcal{M}$. Requiring that poison sources monotonically affect $U(S)$ is sufficient, but not necessary, for ensuring this assumption. %However, monotonicity is a stronger assumption than our requirement.% that $\textrm{AME}_i > 0$. 
%however, so the underlying threat model assumption is weaker.

Outside of these assumptions, our threat model assumes the attacker has access to the model's architecture, its parameters, and the training algorithm used. Attackers also have access to the sample distribution $\mathcal L^i_\mathcal{P}$, but not the specific draws from it used to create the subset models.

%\sid{See below for some more detail about the sparsity assumption that I removed from the intro; we may want to include some of those points here.}
\ignore{
Indeed, it is reasonable to assume sparse contribution. For instance, in the case of data poisoning detection, the attacker is typically only able to poison a limited number of sources given their limited resources at hand. And for the debugging application, the mis-labeled or misleading data should also take up only a small portion of the whole training set. Recently, \cite{feldman2020neural} also shows that data usually exhibit long-tailed distribution, and many tail data (e.g. 2.92\% in ImageNet) in the test set are only influenced by one example in the training data. These data are atypical and thus more likely to get queried. \notejinkun{I remember the previous sentence does not make sense for Sid. Maybe need to rewrite or remove.}
}

\ignore{
We also make a \emph{monotonicity assumption}. 
Now the monotonicity assumption can be stated as follows: given any proponent/opponent $i$, its marginal effect on $S$, \ie $U(S+\{i\})-U(S)$, is non-negative/non-positive for every $S\subseteq [n]-i$, where $[n]=\{1,2,\dots,n\}$; Moreover, There exists at least one subset on which the marginal effect is non-zero (otherwise this source should be considered as neutral). Intuitively, in the application of corrupted data detection, the assumption roughly translates to that adding a corrupted source makes the prediction more corrupted or equally corrupted. Though the assumption is strong as it requires to hold on every subset, it is stronger than necessary for our quantity (discussed in \S\ref{subsec:ame}) to work. At a high level, as long as the overall \emph{average} effect on multiple subsets has the right sign, our quantity should work.
}

%\paragraph{Threat model}
%When applying our technique to the poison detection scenario, the threat model will be (1) attackers have control over a few training data sources; (2) attackers can have the access to the model parameters and the training algorithm; (3) attackers do not have access to the sample distribution $\mathcal L^i$. 

\ignore{
\sid{
\subsection{Efficient Approximation of the Ideal Distribution}
Jinkun/Mathias: Can you move whatever is needed from this subsection to section 3.1? I think it's fine to motivate the need for uniform p's in the previous subsection, but explicitly stating our solution should be reserved for the methodology section.
}

However, achieving strict equalities of probabilities in Eq. \ref{eq:eq} makes the AME coincide with Shapley value (SV) \cite{jia_towards_2020,ghorbani_data_nodate}, which is costly to measure. Therefore, we must approximate it to enable efficient estimation through regression and LASSO.

For our approximation, we sample sources by including each source (except for the source being measured) with probability $P$, where $P$ is a set of probability values, e.g. $\mathcal P=\{p_1,\dots, p_b\}$ for $b$ different values. 
Note that $p_i\times n$ is the expected size of the subset when sampling with probability $p_i$.  Thus, to approximate the uniform coverage requirement, we populate $\mathcal P$ using a 1D grid within a reasonable range and taking all the grid points (\eg $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$). In the case when there is some prior knowledge about the number of proponent/opponent sources, one may opt to use a different $\mathcal P$ (e.g. tighter ranges, closer-by grid-points)\footnote{Alternatively a different coding or sample weights in the regression is also possible. See \S\ref{subsec:lasso}}. We denote by $\mathcal{L}^i_{\mathcal{P}}$ the subset distribution induced by $\mathcal P$ for source $i$. So our approximated $AME$ under this sampled population is
\begin{equation}
\label{eq:amep}
AME_i(\mathcal L^i_{\mathcal{P}})=\mathbb E_{S^i\sim \mathcal L^i_{\mathcal{P}}}[U(S^i+\{i\}) - U(S^i)].
\end{equation}
From now on when we write $AME_i$ we mean $AME_i(\mathcal L^i_{\mathcal{P}})$.
}



\ignore{
How to choose a suitable range and grid-point distance for $\mathcal{P}$? 
First, $\mathcal{P}$ should be sparse, i.e. $|\mathcal{P}|$ is small. This is to help achieve a good estimation in later procedure that will be discussed shortly (see \S\ref{subsec:sampling}).
Second, the range of $\mathcal{P}$ should not include probability values that are too low. With a very low $p$, the sampled subset contains too few sources, so that the resulting model will fail to learn the distinguished features that predict the query label, and thus is not useful for identifying proponents.
Third, very high $p$ should not be included either, because such $p$'s would make little change to the original dataset, and thus suffer from the same issue as the traditional LOO test. 
For our experiments in Sec~\ref{sec:eval}, we use $\mathcal P=\{0.2, 0.4, 0.6, 0.8\}$ unless otherwise specified.
}

% A tempting straightforward alternative is to sample each possible subset of sources uniformly.  This corresponds to sampling each source using $\mathcal P=\{0.5\}$. However, this straightforward approach deviates significantly from the uniform coverage requirement. In experiments of poison detection we find that the grid version is more robust. This is because, more often than not, the subsets with the most marginal effects do not include half of the sources. \notejinkun{Panda and I have agreed to move this experiment to appendix. Maybe we remove this discussion here as well.}




==> rm/motivation.tex <==
% \section{Motivation}

At an abstract level, our objective is to understand the impact of training examples in an ML datasets on specific final predictions from the trained model. Given a specific prediction made by a model, we seek to understand which training examples, through the learning algorithm, are most responsible for this prediction.
More concretely, consider the following example. Based on images collected online, Alice trains a classification model to automatically label different objects that appear on images. 
%
collects data from multiple websites to train an image classification model that recognizes what is on the image. Fig. \ref{fig:running-ex} shows examples of 3 sources/websites. However, some collected images from a website are uploaded by a malicious attacker such that they are just some arbitrary image embedded with a special watermark. Alice unfortunately did not check the data and hence was not aware of this attack, so the model is trained on these poisoned images, and unexpectedly learns the mapping between watermark and some label. Only after Alice deployed it, seeing it always giving poison label whenever there is a watermark in the picture, has she realized that the data could be problematic. Now Alice would like to find out which data source is causing this behavior, so she logged down a mis-predicted picture with such a watermark for further analysis.\jinyang{We should point out that the use of watermark is just for illustrative purposes; many poisoned data do not have visual cues.}
%
We will use this scenario as a running example in the rest of the paper to make the discussion more concrete. The evaluation (\S\ref{subsec:other-apply}) also shows how our technique can be used to study and explain non-adversarial mis-predictions.

Let $\mathcal{M}$ denote the trained model to analyze, e.g. Alice’s image classifier. $\mathcal{M}$ maps each example from the input space $\mathcal X$ to a normalized score between 0 and 1 for each possible class $\mathcal Y$, aka $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$. As each example's normalized scores across all classes sum up to one, they are often interpreted as a probability distribution over classes conditioned on the input, or a confidence score for each class.
Query input/label, and question about finding the proponents
%
Two main theoretically grounded approaches have been proposed to tackle this task of finding training data most responsible for a given problematic prediction.

\paragraph{Influence function:}

\paragraph{Shapley value:}

\paragraph{Goals:} in this paper, we seek to bridge the gap between these approaches by proposing a theoretically grounded approach to the detection problem that:
- enables finding inputs that cause outputs in groups
- is computationally tractable compared to Shapley value, with convergence guarantees
- is practical, with false positive rate control

In the reminder of this paper, we introduce out approach and its theoretical analysis, including assumptions and threat model (\S\ref{}), present a practical instantiation with efficiency improvements (\S\ref{}), discuss extensions to hierarchical designs to handle scenario 2’s sources (\S\ref{}), and perform an empirical evaluation of different tasks and datasets (\S\ref{}).

\section{Approach}

We start from the insight that we are looking for sources with a large, positive causal impact of the score predicted …
=> factorial experiments
=> what population do we need, so that we can handle groups and compute it efficiently?

==> rm/prob-state-discard.tex <==
\section{Problem Statement \fixme{\notejinkun{}Discarded. Pls see motivation section \S\ref{sec:motivation}}}
\label{subsec:pro-state}
\sid{Let's blend this section with the previous motivation section. At the end of this section, the problem formulation should be clear and it should be clear why a quantity like AME is what we need.}
\notepanda{I think we need to help the reader a bit before we step to this paragraph.}

\notepanda{I think we should consider adding a running example starting here, it might help make the technical bits a little clearer and help with connecting some of this to how we will eventually use things.}


% We motivate the problem and our approach through the following running example. As illustrated in Fig \fixme{XX}, \persona{} wants to classify images of handwritten digits that could be either '0', '1' or '2'. The dataset is produced by 6 sources, where every source is assumed to only produce one digit of images, and every digit is produced by two sources. Denote by $0a, 0b$ the two sources producing '0', $1a,1b$ for '1' and $2a, 2b$ for '2'. However, $1b$ is a poisoned source controlled by an attacker who wants to install a backdoor such that every image with a red square will be predicted as '1'. What the attacker did is collecting some images of '0', '1' and '2' upon which red squares are super-imposed, and then their labels are all tampered into '1'. Finally, these poisoned images are injected into the dataset. \persona{} did not check the dataset and hence was not aware of this attack, so the model is trained on these backdoor images, and learns the backdoor well. Only after \persona{} deploys the model, seeing it always gives label '1' whenever there is a red square in the picture no matter what digit it is, has \persona{} realized that the data could be problematic (since \persona{} is confident about correctness of the training algorithm and the code). Now \persona{} would like to find out which data source is causing this behavior, so \persona{} logged down a picture of digit '0' that has red square and been predicted as '1' for further analysis.
We motivate the problem and our approach through the following running example. Alice collects data from multiple websites to train an image classification model that recognizes what is on the image. Fig. \ref{fig:running-ex} shows examples of 3 sources/websites. However, some collected images from a website are uploaded by a malicious attacker such that they are just some arbitrary image embedded with a special watermark. Alice unfortunately did not check the data and hence was not aware of this attack, so the model is trained on these poisoned images, and unexpectedly learns the mapping between watermark and some label. Only after Alice deployed it, seeing it always giving poison label whenever there is a watermark in the picture, has she realized that the data could be problematic. Now Alice would like to find out which data source is causing this behavior, so she logged down a mis-predicted picture with such a watermark for further analysis.

To define this problem formally, consider a classification task with input space $\mathcal X$ and label space $\mathcal Y$, and a classification model $\mathcal{M}: \mathcal X \mapsto [0,1]^{|\mathcal Y|}$ trained using algorithm $\mathcal A$ on a set of data, where $\mathcal{M}$'s output represents the confidence \footnote{Sometimes also called probability, and is often obtained through softmax.} of predicting each label, and the label with largest confidence is chosen as the final prediction. For example in Fig. \ref{fig:running-ex}, the model outputs a vector of three elements, each corresponding to the confidence (a.k.a. probability) of predicting each class. We assume that the training set was produced by a set of $n$ data sources, each of whom contributed a subset of the training set. Finally, assume that when $\mathcal{M}$ is used to infer a label for some input $I\in \mathcal X$ it returns label $L$, which we represent as $\argmax_l \mathcal{M}(I)[l] = L$. We term $\mathcal{M}$ \textit{main model} and $L$ \textit{query label}. In the example above, $L$ is the label index for cat and $I$ is the recorded dog picture, since Alice wants to find out the data sources causing $I$ to be classified as cats.
       
We term a source supporting the prediction \textit{proponent}, source opposing \textit{opponent}, and the rest \textit{neutral}. We define the auditing problem as one where we identify the set of all the proponents. We call it \textit{proponent group}. In the running example, the proponent group is the cat source, and the opponent group should be the dog source since it is producing data of dogs that tell the model this picture should be dogs, thus opposing the queried label $L$ (\ie cat). %\notejinkun{maybe defer this notation to when it is first used, which seems to be in evaluation.}% Let $k$ be its size, and $k'$ be the opponent group size. %Call $k_i, i=1,\dots,k$ a specific item in $S_+$. 

We make a \textit{sparsity assumptions}: only a sparse set of sources are proponents or opponents. We denote by $k$ the number of sources in this sparse set, and the assumption can be written as $k \ll n$. 

We also make a \emph{monotonicity assumption}. To make the discussion clear, we first define a quantity $U(S)$ to measure how supportive a source $S$ is to the prediction. To do so, we first train a model $\mathcal M_S$ on $S$, and use its inference confidence on query input as the measure. Formally, $U(S)=\mathcal M_S(I)[L]$. We also call it \emph{signal} of $S$ or signal of $\mathcal M_S$. %Users can choose their own measure \notejinkun{how do we state this point succinctly?} For simplicity, we assume the default option is used unless specified otherwise.
% We also make a monotonicity assumption. To make the discussion clear, we first formalize the definition of \textit{signal}:
%\textit{LOO effect} and a closely related concept \textit{signal}:
% \begin{enumerate}
    % \item 
    % \textit{Signal} $U(S)$ of a subset $S\subseteq [n]$ of tenants is defined as a measurement of how supportive $S$ is to the query prediction. Users can choose their own measure \notejinkun{how do we state this point succinctly?} and we recommend $U(S)=\mathcal M_S(I)[L]$ as a default option, where $[n]=\{1,2,\dots,n\}$ and $\mathcal M_S=\mathcal{A}(S)$ is the model trained on $S$. As mentioned previously $\mathcal M_S(I)[L]$ is the confidence of predicting the label $L$ and thus fits naturally into the definition. For simplicity, we assume the default option is used unless specified otherwise. % Put another way, we want to identify the set of tenants $S_+$, such that if we trained a model with $\mathcal{M}'$ using training data $\mathcal D' = \mathcal D - \mathcal{D}_{S_+}$ (where $\mathcal{D}_{S_+} = \bigcup_{i\in {S_+}} \mathcal D_i$) then $\mathcal{M}(I)\neq L$. Note, that in this definition 
Now the monotonicity assumption can be stated as follows: given any proponent/opponent $i$, its marginal effect on $S$, \ie $U(S+\{i\})-U(S)$, is non-negative/non-positive for every $S\subseteq [n]-i$, where $[n]=\{1,2,\dots,n\}$. Intuitively, it says that adding a poisoned source makes the prediction more poisoned or equally poisoned, if we are considering poison detection. Though the assumption is strong as it requires to hold on every subset, it is stronger than necessary for our quantity (discussed in \S\ref{subsec:ame}) to work. At a high level, as long as the overall \emph{average} effect on multiple subsets has the right sign, our quantity should work.

Finally, we do not exclude the case where each source only produce one training example. In such a case, the problem becomes identifying the training examples that support/oppose the prediction.


==> rm/related-work-v1.tex <==
\section{Related Work}
\label{sec:rel-work}
The closest related works also aim to provide principled measures of training data impact on a the performance of an ML model, with such various goals as data valuation \cite{jia_towards_2020,ghorbani_data_nodate}, model explainability \cite{feldman2020neural, koh_understanding_2017}, debugging datasets \cite{chakarov2016debugging, koh_understanding_2017,koh_accuracy_2019, pruthi_estimating_2020}, or detecting poisoning \cite{koh_understanding_2017}.
Existing approaches, some of which we previously described in \S\ref{sec:intro}, can be divided into three categories.
{\bf Shapley value} is the closest to \quantity{} and measures a datapoint's marginal contribution to all subsets of the data. Like our \quantity{}, it is able to capture individual contributions to group effects. However, no existing approach is efficient for DNNs \cite{jia_towards_2020,ghorbani_data_nodate}, only scaling linearly in the number of data sources.
{\bf Influence} measures the leave-one-out effect of a data point over the training procedure \cite{koh_understanding_2017}, including for groups of data points \cite{koh_accuracy_2019}.
However, efficient estimations of influence require assumptions and are only heuristically applied to DNNs, with limited accuracy \cite{basu_influence_2020}. 
Representer Point~\cite{repr} finetunes the last layer to reach a stationary point in specifically defined optimization problem, such that it can assign each training point with an importance score based on the finetuned model and how similar the training point is to the query input in the feature representation.
TracIn~\cite{pruthi_estimating_2020} tracks loss change between consecutive batches during SGD training for efficiency, and CosIn~\cite{hammoudehsimple} improves on TracIn by taking the gradient directions into consideration.
In all approaches above, groups of data points are either not supported \cite{koh_understanding_2017,repr,pruthi_estimating_2020,hammoudehsimple}, or it is not clear how to efficiently find groups with large influence, and isolate the impact of individual data points within a group \cite{koh_accuracy_2019}.
%
Another recent work \cite{feldman2020neural} leverages influence to study memorization in ML models. They use subsampling as a heuristic for estimation, but only use one inclusion probability and do not consider efficient approaches to find sources with large influence.
%
\sout{ {\bf Probability of Sufficiency} (PS) also builds on causal inference theory, and measures the causal impact of switching data points' labels \mbox{\cite{chakarov2016debugging}}.
%While PS has similarities with our \quantity{} in that it measures the marginal effect of label assignment on a population of randomly assigned labels,
The proposed estimation techniques do not apply to complex ML models such as DNNs.}
%
In contrast, we propose a principled quantity that measures the marginal impact of a data point when added to different subsets of the data, and show that it captures individual contributions to group effects. \sout{We propose an efficient methodology to estimate this quantity for all data points together, that applies to DNNs and, under our sparsity assumption, scales logarithmically in the total number of sources.}


%\paragraph{Data contribution, influence, and Shapley value}
%Related to our \quantity{}, there are other works trying to quantify the contribution of individual training example to the model or an inference behavior.~\cite{jia_towards_2020,ghorbani_data_nodate} propose to quantify using Shapley value (SV), but their approaches are either too costly or making strong assumption about the models.

%\cite{koh_understanding_2017} propose influence function to approximate the leave-one-out effect, but even the true leave-out effect is not accurate as a contribution measurement since the contribution is non-linear.~\cite{koh_accuracy_2019} generalizes influence function to approximate group leave-out effect, but the approximation is not accurate for DNNs~\cite{basu_influence_2020} and it is not clear how to map  the group effect to individual effect.~\cite{pruthi_estimating_2020} defines influence using the loss change between consecutive batches in SGD, and proposes efficient approximation algorithm. However, it is not clear how to generalize to source scenario; furthermore, it also assumes the loss change is only caused by the datapoints involved in current batches while today's DNNs typically employ momentum and Batch Normalization that would make previous batches also influence the current gradient updates.~\cite{feldman2020neural} uses similar subsampling and compute the influence in that population, but they are subsampling only one subset size and using diff-in-means method. They are aiming for a different problem which is studying memorization effect of learning algorithms, but their experiments in turn also justify the validity of using \quantity{} to measure contribution.

%\cite{chakarov2016debugging} proposes to use \textit{Probability of Sufficiency} (PS) from Pearl's theory of causation to measure the contribution. (Instead of observing the change after leaving-out one example, they randomly assign it a different label and observe the change. Though one could define PS using the LOO effect in this paper, PS is also different from \quantity{} in that PS is aggregating the probability mass of samples having a large change, while \quantity{} is directly averaging the changes weighted by the probability mass.) \notejinkun{Should we briefly describe PS as in the parenthesis?} However, PS is costly to compute straightforwardly, and their optimizations are only for Logistic Regression and Decision Trees but not for DNNs. It is unclear how well can it generalize to DNNs.


Another related body of work is that of data poisoning attacks and defenses, part of the active research field of adversarial machine learning.
%\paragraph{Adversarial Machine Learning}
{\bf Data poisoning attacks} tamper with ML models' training sets to influence the behavior of the trained model at prediction time \cite{Shafahi2018PoisonFT,li2016data,gu2017badnets,chen2017targeted,bhagoji_analyzing_2019,bagdasaryan_how_2019,konevcny2016federated,turner2019label}.
As such, they exemplify one use-case for our detection methodology, for which ground truth is available, a fact we leverage in our evaluation.
%There has been an increased research focus on Adversarial Machine Learning on both the poisoning and its detection/defense. The attacker can install the poisoning during training, inference or both.
%The poisoning in our poison detection application is called data poisoning attack, which is mostly a training-time attack that tampers the training set to manipulate the behavior of the model at test time. 
%Many works~\cite{Shafahi2018PoisonFT,li2016data,gu2017badnets,chen2017targeted} have demonstrated that it is possible to only add a few (sometimes seemingly innocuous) examples to manipulate the model. There is also model poisoning attack~\cite{bhagoji_analyzing_2019,bagdasaryan_how_2019} poisoning the training process specifically in Federated Learning~\cite{konevcny2016federated}. Given the similarity between traditional training, our technique may also be applied to identify poisoned clients.
%Finally, there is also test-time attack~\cite{goodfellow2014explaining} that generates adversarial test inputs where model would make wrong predictions, despite being imperceptible from normal inputs. Though our technique may also be used, users should keep in mind that it is the test input that is more to blame, instead of the training data (e.g. the test input may be maliciously crafted to fool our technique into selecting attacker-chosen data using the technique in poison-frog).
%\paragraph{Detection and defense of data poisoning attack}
% Broadly there are two lines of work: one that makes little assumption about the model, and one that targets some specific model and/or scenario.
Given the nature of poisoning attacks, {\bf poisoning detection} defenses are closely related to our work.
General detection algorithms eliminate poisoned data by measuring the leave-one-out effect of data points on subsets of the data \cite{barreno_security_2010,baracaldo_mitigating_2017}, an approach called Reject On Negative Impact (RONI).
These works do not study the subset distributions that should be used, and inefficiently train one model for every pair of subset and training example to evaluate.
%
% JK: Oringal version below: % Other defenses and detection algorithms are less general making strong assumptions on the models or attacks, such as linear models~\cite{Jagielski2018ManipulatingML}, trigger attacks on vision tasks~\cite{gao2019strip}, or representations in a DNN's last layer that separate benign inputs from adversarial ones \cite{chen2018detecting}.
One line of methods \cite{tran2018spectral,hayase2021spectre,chen2018detecting,tang2021demon,shen2016auror} use outlier detection to identify poisoned data, which is not query-aware and may select benign outliers.
Other defenses and detection algorithms require clean data~\cite{doan2020februus,tang2021demon,veldanda2020nnoculation}, or are less general, making strong assumptions on the models or attacks such as linear models~\cite{Jagielski2018ManipulatingML}, source-agnostic trigger attacks on vision tasks~\cite{gao2019strip}, trigger attacks with small norm or size~\cite{chou2018sentinet,Wang2019NeuralCI,udeshi2019model}, or clean-label attacks~\cite{peri2020deep}.

%~\cite{Steinhardt2017CertifiedDF}
% While there has been some work~\cite{Jagielski2018ManipulatingML, shen2016auror,baracaldo_mitigating_2017,subedar2019deep,chen2018detecting,gao2019strip} on defending or detecting against these attacks, this work has relied on assumptions about the models or the attack scheme.


% \paragraph{ML model interpretation}

\ignore{Our work is also related to \textbf{data cleaning and management} when applied to poison detection. Traditionally these methods are based on integrity constraints \cite{chu2013holistic,chu2013discovering} that use a set of predefined rules to ensure the consistency of the data. However, integrity constraints are often not complete enough to be used as a defense strategy, and they also can be circumvented once attackers know them. Other methods use outlier detection \cite{maletic2000data, hellerstein2008quantitative}, but as shown by \cite{koh2018stronger}, poisoned data can also be inliers. 
Recent works have used a downstream model (i.e., a DNN to train on the data) to guide the cleaning. BoostClean~ \cite{krishnan2017boostclean} and TARS~\cite{dolatshah2018cleaning} select data to clean based on how much the test set performance can be improved. Poisoning often doesn't impact test set performance, so these methods are not suitable defences \cite{gao2019strip}. ActiveClean \cite{krishnan2016activeclean} assumes a convex model and the existence of an oracle (experts) that can be repeatedly queried to correctly clean a given data point. 
%It then simultaneously trains the model and cleans the data. However, it relies on the convexity. Furthermore, without queries it can be challenging (\eg clean-label attacks) to judge whether the data are poisoned or not even for experts. For instance, clean-label attacks are hard to discern unless the queries are presented alongside.
None of the above work is query-driven, so they cannot answer the problem Enola is solving. Rain \cite{wu2020complaint} is query-driven and aims to extend influence functions to explain SQL query results. Instead, Enola focuses on a single DNN.
}

Enola is also related to \textbf{data cleaning and management}. However, they are often not suitable defences. Traditional integrity constraints \cite{chu2013holistic,chu2013discovering} and outlier detection \cite{maletic2000data, hellerstein2008quantitative} based methods examine data only in the input domain and are vulnerable as shown by \cite{koh2018stronger}.
%, the high dimensionality often allows attackers to generate conforming but poisoned data.
Recent works have used a downstream model (\ie a DNN to train on the data) to guide the cleaning, but are still not suitable. For instance, \cite{krishnan2017boostclean,dolatshah2018cleaning} assume the corrupt data impact the test set performance which is often not the case for poisoning, and
%BoostClean~ \cite{krishnan2017boostclean} and TARS~\cite{dolatshah2018cleaning} select data to clean based on how much the test set performance can be improved. Poisoning often doesn't impact test set performance, so these methods are not suitable defences \cite{gao2019strip}. ActiveClean 
\cite{krishnan2016activeclean} assumes a convex model.
% and the existence of an oracle (experts) that can be repeatedly queried to correctly clean a given data point. 
Furthermore, none of the above work is query-driven so cannot answer the problem Enola is solving. Rain \cite{wu2020complaint} is query-driven and aims to extend influence functions to explain SQL query results. Instead, Enola focuses on a single DNN.

Finally, our work leverages, and builds on, a large body of existing work from different fields.
%
First is the {\bf causal inference} literature.
If we regard the inclusion of a data source as a treatment, our methodology is related to factorial experiments, from which our \quantity{} is inspired. For instance, ~\cite{kang2007demystifying, imbens_causal_2015} focuses on single treatment \quantity{} (i.e. only one source) and observational study rather than randomized experiment. 
Multiple treatments are introduced in \cite{egami_causal_2019,dasgupta_causal_2015,hainmueller_causal_2014}, though their quantity uses different population distribution than ours, and different estimation techniques.
In the computer science filed, Sunlight \cite{10.1145/2810103.2813614} uses a similar approach to study ad targeting. However, this paper uses only one sampling probability, and a holdout set for statistical confidence instead of our knockoff procedure.
%
Second, {\bf sparse recovery} studies efficient algorithms to recover a sparse signal from high dimensional observations. We leverage LASSO \cite{lecue_regularization_2017} --with properties related to those of compressive sensing \cite{candes2006compressive}-- and knockoffs \cite{candes_panning_2017}.
%
Other approaches to the important factor selection problem exist, such as the analysis of variance (ANOVA) \cite{bondell_simultaneous_2009, egami_causal_2019, post_factor_2013} used in \cite{egami_causal_2019}, but we think LASSO is better suited to our use-case due to its scalability guarantees.
%
Third, our goal is related to {\bf Group Testing} \cite{noauthor_group_2021,group-survey}, which performs batch tests on groups of candidates to find the small number of those with large influence on the result.
While we focused on LASSO-based sparse recovery for its capacity to handle noisy continuous signals, studying if and how group testing ideas could improve our technique is an interesting avenue for future work.

%\paragraph{Important factor selection}
%Instead of using variable selection like LASSO/LASSO+Knockoffs, analysis of variance (ANOVA) is another technique in statistics to select important factors. \notejinkun{How do we compare against ANOVA? I'm not familiar with this approach. AFAIK, it is doing hypothesis test with one null hypothesis per factor stating that factor has no effect, and construct F-statistics, so they can control False Positive Rate. They have some assumptions (normality and same variance \url{http://homepage.stat.uiowa.edu/~rdecook/stat3200/notes/ch8_2way_part1_4pp.pdf}), and need to model interactions (which is cost prohibitive) or assume no interaction (strong assumption?).}

%There are also some works applying LASSO to select important factors and comparing against ANOVA~\cite{bondell_simultaneous_2009, egami_causal_2019, post_factor_2013}. However, they all need to assume a model of the factors' effect in advance, expressed by interaction terms, which is non-trivial to determine. We differ in that no assumption is made about the model. \notejinkun{Not very confident. Is it true that ANOVA and these 3 works need to assume the model? I think so because I usually see something like "assume no interaction effect" in these papers.} % However,~\cite{bondell_simultaneous_2009} assumes linear effect (i.e. no interaction), and in~\cite{egami_causal_2019, post_factor_2013} 


%\paragraph{Group Testing}
%our problem statement is related to Group Testing~\cite{noauthor_group_2021}. In one simple version of Group Testing, we want to find out $k$ out of $n$ blood samples that contains virus using minimal number of blood tests. Blood tests can be conducted either on individual sample or a combination of multiple samples. The latter may be useful since if it returns negative, all samples in this group can be claimed negative without the need for further testing, thus saving many tests. The basic version assumes noise-free testing: the test returns positive if and only if there are at least one infected sample, while other variants model the noise. Our procedure of subsampling subsets and training resembles the tests, and it would be interesting to see how Group Testing techniques can be applied to improve our technique. Some challenges include: (1) how to make the Group Testing be ``continuous'' since we do not have notion of positive/negative; (2) how to model the noise under the context of ML.
